Masked prediction tasks: a parameter identifiability view

The vast majority of work in self-supervised learning, both theoretical and empirical (though mostly the latter), have largely focused on recovering good features for downstream tasks, with the definition of "good" often being intricately tied to the downstream task itself. This lens is undoubtedly very interesting, but suffers from the problem that there isn't a "canonical" set of downstream tasks to focus on -- in practice, this problem is usually resolved by competing on the benchmark dataset du jour. In this paper, we present an alternative lens: one of parameter identifiability. More precisely, we consider data coming from a parametric probabilistic model, and train a self-supervised learning predictor with a suitably chosen parametric form. Then, we ask whether we can read off the ground truth parameters of the probabilistic model from the optimal predictor. We focus on the widely used self-supervised learning method of predicting masked tokens, which is popular for both natural languages and visual data. While incarnations of this approach have already been successfully used for simpler probabilistic models (e.g. learning fully-observed undirected graphical models), we focus instead on latent-variable models capturing sequential structures -- namely Hidden Markov Models with both discrete and conditionally Gaussian observations. We show that there is a rich landscape of possibilities, out of which some prediction tasks yield identifiability, while others do not. Our results, borne of a theoretical grounding of self-supervised learning, could thus potentially beneficially inform practice. Moreover, we uncover close connections with uniqueness of tensor rank decompositions -- a widely used tool in studying identifiability through the lens of the method of moments.

==> COLT2022/3.discrete.tex <==
\section{Learning with discrete hidden Markov models}

Our goal is to characterize the types of prediction task that enables parameter recovery.
For sufficient conditions, prior work by \cite{kruskal77}
% and \cite{anandkumar2014tensor}
and \cite{allman2009identifiability}
have shown that third-order moments suffice for parameter identifiability.
%  we only need to focus on tasks involving tensors of order no more than 3.
Regarding necessary conditions, it is well-known in the factor analysis literature that matrices (i.e. second-order moments) are insufficient for identifiability in general, unless under additional conditions such as sparsity~\citep{donoho2003optimally,candes2006stable,spielman2012exact,arora2014new}, low-rankness~\citep{georgiev2005sparse,aharon2006uniqueness,cohen2019identifiability}, or orthogonality.
% \textcolor{Orange}{(todo: other citations?)}

Given results in prior work, it seems natural to use tasks which predict 3 masked out tokens.
It turns out that we can do better: predicting only 1 or 2 tokens can suffice for identifiability, provided that the task involves three tokens when counting also the conditioned tokens:
\vspace{-1em}
\begin{theorem}[Identifiability of masked prediction \textcolor{Orange}{on three tokens}, HMM]
% \label{lem:discrete_two_given_one}
\label{thm:discrete}
    Let the ground truth parameters $\mEmiss, \mTrans$ satisfy Assumption \ref{assump:latent}, \ref{assump:discrete_rowNE}, \ref{assump:discrete_full_rank}.
    % Let the prediction task be $x_{\tTwo} \otimes x_\tThr | x_\tOne$ for $(\tOne, \tTwo, \tThr)$ being any permutation of $(1,2,3)$.
    Let the prediction task be $x_{\tTwo} \otimes x_\tThr | x_\tOne$ for $(\tOne, \tTwo, \tThr)$ being any permutation of $(1,2,3)$.
    If $\tilde\mEmiss, \tilde\mTrans$ forms an optimal predictor,
    then $\tilde\mEmiss = \mEmiss$, $\tilde\mTrans = \mTrans$ up to a permutation of labeling.
    % \vspace{-0.8em}
    % \begin{enumerate}
        % \item the task of predicting $x_{t_2} \otimes x_{t_3}$ given $x_{t_1}$;
        % \item the task of predicting $x_{t_3}$ given $x_{t_1} \otimes x_{t_2}$ (\textcolor{Orange}{todo}).
    % \end{enumerate}
\end{theorem}
The proof of Theorem \ref{thm:discrete} works by constructing a third-order tensor from the conditional second-order tensors given by the masked prediction task, for which Kruskal's theorem gives identifiability up to column-wise permutation and scaling.
The indeterminacy in scaling can be further removed by the fact that columns of $\mTrans$ sum up to 1.

As a remark, the choice of time step $1,2,3$ can be generalized to $\tOne, \tTwo, \tThr$ provided that they contain at least one pair of adjacent time steps.
We cannot generalize beyond adjacent time steps though.
The intuition is that the conditional distribution of one token given another is defined with the transition matrix raised to the power of the difference in time.
When the time steps are at least 2 steps apart, matching the predictors only matches the matrix power, which however does not imply the transition matrices themselves are the same as shown by the following result:
\vspace{-1em}
\begin{lemma}
\label{lem:transPower_nonId}
      For any positive integer $t$, there exist stochastic matrices $\mTrans, \tilde\mTrans$ satisfying Assumption \ref{assump:latent}, \ref{assump:discrete_full_rank},
      such that $\mTrans \neq \tilde{\mTrans}$ and $\mTrans^t = \tilde\mTrans^{t}$. 
      \textcolor{Orange}{(note: changed from the previous theorem to this lemma)}
\end{lemma}

% \vspace{-1em}
% \begin{theorem}[Nonidentifiability from large time gaps]
% \label{thm:power_nonId}
%     Let $\tOne, \tTwo, \tThr$ be distinct time steps such that any pair of time steps are at least 2 steps apart.
%     Then, there exist parameters $\mMeans,\mTrans$ and $\tilde\mMeans, \tilde\mTrans$ following Assumption \ref{assump:latent}, \ref{assump:discrete_rowNE}, \ref{assump:discrete_full_rank},
%     such that $\tilde{\mTrans} \neq \mPerm\mTrans$ for any permutation $\mPerm$, yet $\tilde\mMeans, \tilde\mTrans$ form an optimal predictor for the prediction task of $x_{\tTwo} \otimes x_{\tOne}|x_{\tOne}$.
%     % one of the following is satisfied:
%     % \vspace{-0.4em}
%     % \begin{itemize}[leftmargin=*]
%         % 1) $f_{\mMeans,\mTrans}^{\tTwo, \tThr|\tOne}(x_\tOne) = f_{\tilde\mMeans,\tilde\mTrans}^{\tTwo, \tThr|\tOne}(x_\tOne)$, $\forall x_\tOne$;
%         % or 2) $f_{\mMeans,\mTrans}^{\tThr|\tOne, \tTwo}(x_\tOne, x_\tTwo) = f_{\tilde\mMeans,\tilde\mTrans}^{\tThr|\tOne, \tTwo}(x_\tOne, x_\tTwo)$.
%     % \end{itemize}
%     \textcolor{red}{matching two powers together?}
% \end{theorem}
% \vspace{-0.5em}


Moreover, we note that it is indeed necessary for the prediction task to involve three tokens.
The following result show that if each task involves only two tokens, then the parameters are not identifiable even when considering multiple tasks together:
\vspace{-1em}
\begin{theorem}[Nonidentifiability of pairwise masked prediction]
\label{thm:discrete_nonId}
    Let the ground truth parameters $\mEmiss, \mTrans$ of a HMM satisfy Assumption \ref{assump:latent}, \ref{assump:discrete_rowNE} and \ref{assump:discrete_full_rank}.
    % \ref{assump:discrete_distinct_diag},
    There exist $\tilde\mEmiss, \tilde\mTrans$ satisfying the same assumptions. such that $\tilde\mEmiss, \tilde\mTrans$ form optimal predictors for the tasks of $x_2|x_1$, $x_1|x_2$, $x_3|x_1$, and $x_1|x_3$,
    yet $\tilde\mEmiss \neq \mEmiss$.
\end{theorem}
\vspace{-1em}
\textcolor{draftGray}{\textcolor{Orange}{todo} (low priority): the non-identifiability result can generalize to generic timesteps as well? e.g. we know that $\mTrans^2 = \tilde\mTrans^2$ doesn't imply $\mTrans = \tilde\mTrans$; the same likely applies to other powers as well.}

% \subsection{Identifiability from predicting a single token}
% Next, we show that with proper conditioning, predicting a single token also suffices for parameter recovery:
% \vspace{-1em}
% \begin{theorem}[Identifiability of predicting a single token, conditioned on two]
% \label{lem:discrete_one_given_two}
%     Consider the task of \textcolor{peach}{predicting $x_{t_3}$ given $x_{t_1} \otimes x_{t_2}$},
%     where $t_1, t_2,t_3$ are distinct time steps.
%     Under Assumption \ref{assump:discrete_uniform_latent}, \ref{assump:discrete_full_rank}, \ref{assump:discrete_distinct_diag}, if the predictor has \emph{\textcolor{Orange}{the correct parametric form}}, then
%     $f^{t_3|t_1,t_2}(\cdot; \mTrans, \mEmiss) = f^{t_3|t_1, t_2}(\cdot; \tilde\mTrans, \tilde\mEmiss)$ implies $\tilde\mTrans = \mTrans$, $\tilde\mEmiss = \mEmiss$.
% \end{theorem}
% \textcolor{Orange}{todo: merge the two lemmas into 1 theorem}


% We note that it is important to predict the two tokens jointly.
% Learning both the task of $x_{t_2} | x_{t_1}$ and $x_{t_3} | x_{t_1}$ also gives identifiability.
% For this negative result, let's consider a more restricted set of parameters, where the emission matrix is also row normalized.
% \vspace{-1em}
% \begin{assumption}[Row normalization]
% \label{assump:discrete_row_normed}
%     $\forall i \in [d]$, $\sum_{j \in [k]}B_{ij} = 1$.
% \end{assumption}
% The following lemma states that a pair of single-token prediction tasks cannot guarantee identifiability even under the additional assumption of row normalization:
% \vspace{-1em}
% \begin{lemma}[\textcolor{Orange}{Identifiability} of predicting a pair of single tokens, conditioned on one]
% \label{lem:discrete_pair_single}
%     Let $\mTrans, \tilde\mTrans \in \R^{d \times k}$, $\mEmiss, \tilde\mEmiss \in \R^{k \times k}$ satisfy Assumption \ref{assump:discrete_uniform_latent}, \ref{assump:discrete_full_rank}, and \ref{assump:discrete_distinct_diag}.
%     %  and \ref{assump:discrete_row_normed}.
%     For any distinct time steps $t_1, t_2, t_3$, if the predictor has \emph{\textcolor{Orange}{the correct parametric form}}
%     then having $f^{t_2|t_1}(\cdot; \mTrans, \mEmiss) = f^{t_2|t_1}(\cdot; \tilde\mTrans, \tilde\mEmiss)$ and $f^{t_3|t_1}(\cdot; \mTrans, \mEmiss) = f^{t_3|t_1}(\cdot; \tilde\mTrans, \tilde\mEmiss)$ implies $\tilde\mTrans = \mTrans$, $\tilde\mEmiss = \mEmiss$.
%     % Then, there exist an infinite number of $\tilde\mTrans \in \R^{d \times k}, \tilde\mEmiss \in \R^{k \times k}$ satisfying the same assumptions, such that $f^{2|1}(\cdot ; \mTrans,\mEmiss) = f^{2|1}(\cdot ; \tilde\mTrans, \tilde\mEmiss)$ and $f^{3|1}(\cdot ; \mTrans,\mEmiss) = f^{3|1}(\cdot ; \tilde\mTrans, \tilde\mEmiss)$.
% \end{lemma}





==> COLT2022/4.gmm.tex <==
\section{Learning with conditionally-Gaussian HMMs}
% \section{Learning with Gaussian mixture hidden Markov models}

First, we have the identifiability result from predicting three-tokens, similar to the discrete case:
\vspace{-1em}
\begin{theorem}[Identifiability of masked prediction \textcolor{Orange}{on three tokens}, \GHMM]
\label{thm:gmm}
    Let the ground truth parameters $\mMeans, \mTrans$ satisfy Assumption \ref{assump:latent}, \ref{assump:gmm_full_rank},and \ref{assump:gmm_equal_norms}.
    % Let the prediction task be $x_{\tTwo} \otimes x_\tThr | x_\tOne$ for $(\tOne, \tTwo, \tThr)$ being any permutation of $(1,2,3)$.
    If $\tilde\mMeans, \tilde\mTrans$ forms an optimal predictor,
    then 
    \vspace{-0.8em}
    \begin{enumerate}[leftmargin=*]
    \item when the task is predicting $x_2 \otimes x_3$ given $x_1$ (or predicting $x_1 \otimes x_2$ given $x_3$),
        then $\tilde\mMeans = \mMeans$, $\tilde\mTrans = \mTrans$ up to a permutation of labeling; 
    
    \item when the task is predicting $x_1 \otimes x_3$ given $x_2$,
        then $\tilde\mMeans = \mH\mMeans$, $\tilde\mTrans = \mTrans$ up to a permutation of labeling, where \textcolor{peach}{$\mH \in \R^{d \times d}$} is a Householder transformation that is uniquely determined by $\mMeans$.
    \end{enumerate}
\end{theorem}
% 
The proof is similar to that of Theorem \ref{thm:discrete} using the Kruskal's theorem.
The difference between the discrete and the Gaussian case is that the posterior function $\phi(x)$ takes up different forms, which will affect the identifiability of parameters.
As a result, while the pairwise prediction task is not identifiable for HMM,
it does suffice for identifiability for \GHMM:
\vspace{-0.8em}
\begin{theorem}[Identifiability of \GHMM~ from predicting $x_2$ given $x_1$]
\label{thm:gmm_2_1_id}
    Under Assumption \ref{assump:latent}, \ref{assump:gmm_full_rank}, and \ref{assump:gmm_equal_norms},
    if $\mMeans, \mTrans$ and $\tilde\mMeans, \tilde\mTrans$ give the same predictor for $x_2$ given $x_1$,
    then up to a permutation of labeling, $\tilde\mMeans \in \{\mMeans, \mH\mMeans\}$ where $\mH$ is a Householder reflection uniquely determined by $\mMeans$.
\end{theorem}
\vspace{-1em}
The proof idea is that matching the predictors implies matching the posterior function, which requires $\tilde{\mMeans}$ to be a translation of $\mMeans$.
It turns out that this translation is given by Householder transformation $\mH = (\mI_d - 2\hat{v}\hat{v}^\top)\mMeans$, for $\hat{v}$ being the unit vector normal to the affine hull of $\gA := \{\mu_i: i \in [k]\}$.
Intuitively, the set of $\{\tilde\mu_i\}_{i\in[k]}$ are obtained by translating $\gA$ to the other side of the origin, and intersecting this shifted affine hull with the hypersphere on which $\{\mu_i\}_{i\in[k]}$ lie.
Since the direction of translation is normal to the affine hull, this translation is also the reflection of $\{\mu_i\}_{i\in[k]}$ with respect to the subspace parallel to $\gA$.
\footnote{
Such subspace is a hyperplane when $d=k$.
When $d>k$, we only need to consider the $k$-dimensional subspace that is the span of $\{\mu_i\}_{i \in [k]}$
(since $\tilde\mMeans$ parameterizing an optimal predictor means the column span of $\tilde\mMeans$ is the same as that of $\mMeans$), hence the reflection is still well defined.
% Reflection should be defined with respect to hyperplanes rather than other subspaces of lower dimensions.
}

The non-determinacy of $\mR$ can be further eliminated if we consider the full conditional \textit{distribution} rather than the conditional \textit{expectation}:
\vspace{-0.8em}
\begin{theorem}[Identifiability of conditional distribution]
\label{thm:gmm_conditional}
    % If $p(x_2|x_1; \mMeans,\mTrans) = p(x_2|x_1; \tilde\mMeans,\tilde{\mTrans})$, $\forall x_1,x_2 \in \R^d$,
    Let $\mMeans, \mTrans$ and $\tilde\mMeans, \tilde\mTrans$ be two set of parameters satisfying Assumption \ref{assump:latent} and \ref{assump:gmm_full_rank}.
    If $p(x_2|x_1; \mMeans,\mTrans) = p(x_2|x_1; \tilde\mMeans,\tilde{\mTrans})$, $\forall x_1,x_2 \in \R^d$,
    then $\mMeans = \tilde\mMeans$, $\mTrans = \tilde\mTrans$ up to a permutation of labeling. 
\end{theorem}
\vspace{-1em}
Contrasting Theorem \ref{thm:gmm_2_1_id} and \ref{thm:gmm_conditional} highlights that unlike discrete HMMs, the non-identifiability of pairwise prediction task in \GHMM~is not because there is not enough information in pairs, but that masked prediction only utilizes the conditional expectation, which is too weak a task.
Moreover, while there likely exist self-supervised tasks whose objectives correspond to matching the conditional distribution, our goal is not to propose specific algorithms, and thus Theorem \ref{thm:gmm_conditional} should be treated only as a characterization for identifiability.

\textcolor{gray}{\textcolor{Orange}{note}: we can also remove $\mH$ by predicting both $x_2|x_1$ and $x_3|x_1$, as stated in Theorem \ref{thm:gmm_21_31} in the appendix.}

%% Commenting out previous theorem statements
% \input{COLT2022/not_used/gmm_previous_statements}


==> COLT2022/bak/Feb6th_4pm/1.intro.tex <==
\section{Introduction}


% \textcolor{gray}{// Self-supervised learning: initially tool for distribution learning (e.g. NCE, etc. as cheaper alternatives to MLE). Progressively, goal of learning a distribution got abandoned in favor of learning a ``good'' representation. }
\textcolor{gray}{// self-supervised learning and masked prediction}

Self-supervised learning refers to the type of learning where the training signals come from inherent properties of the data, without  requiring explicitly curated labels.
As a generic learning paradigm, self-supervision is extremely versatile and can be applied to a range of tasks.
A good-performing method is the masked prediction task, where the model is trained to predict the missing part of a sample given the rest of it.
This strategy has been widely adopted in empirical works.
Notable early works include word2vec~\citep{word2vec}, which uses continuous bag-of-word and skip-gram for learning word embeddings.
More recently, large-scale experiments enabled by architectural progress such as the invention of Transformers~\citep{vaswani2017attention} have shown great progress in processing both natural languages and visual data, where the models are able to produce decent representations that can perform well on a wide range of downstream tasks~\citep{bert,GPT2,MAE21}


% \textcolor{gray}{// It isn't clear what a ``good'' representation is when detached from a model of data --- in practice, this is evaluated through a suite of downstream tasks. Unclear what tasks are ``canonical''. }

% \textcolor{gray}{// When data comes from a generative model (particular a latent-variable one), it makes sense to ask when the learned predictors (if parametrized correctly), recover the ground truth parameters. This is actually a classical approach to learning probabilistic models (e.g. learning MRFs via pseudo-likelihood, which involves predicting a node from it's neighbors), but the question hasn't been tackled in more complicated (e.g. latent-variable) models.}

\textcolor{gray}{// representation learning relies on downstream tasks; this work focuses on parameter recovery}

The majority of the current self-supervised learning research have been focusing on representation learning, where the progress is measured by the performance of downstream tasks.
However, using downstream performance as a quality measure can be suboptimal, since different downstream tasks may favor different properties of the representation \textcolor{grass}{(cite?)}, and it is unclear which task should be chosen.
We argue that a better alternative is to focus on learning the data distribution itself.
Note that using self-supervised learning for distribution learning is not unreasonable;
for instance, early work by \cite{nce} has proposed to contrast the data distribution with a known noise distribution as a less computationally intensive alternative of the classical maximum likelihood estimation.

% \textcolor{gray}{// This question is in spirit similar to other ``ML alternatives'' --- e.g. method of moments and tensor decomposition-based algorithms. We tackle this question in models with time-series structure: HMMs (discrete latents, observables) and state-space models (discrete latents, continuous observables). In the latter case, we focus on the case of $x_t|z_t$ being a Gaussian distribution (i.e. the marginal $p(x_t)$ is a mixture of Gaussians). }

\textcolor{gray}{// parameter recovery for latent-variable sequence models}

In this work, we focus on the \emph{masked prediction task} and its application to parameter recovery of latent-variable generative models.
One advantage of using a generative model is that there is readily a notion of ground truth,
and it makes sense to ask whether and when the learned models are able to recover these ground truth parameters.
Masked prediction fits naturally to this objective and has in fact been a classical approach to learning probabilistic models.
For instance, \cite{ravikumar2010high} used pseudo-likelihood to learn Markov random fields via regularized prediction of a node given its neighbors \textcolor{grass}{(more cites)}.
In contrast to prior works which mostly focus on fully observed models,
we tackle this question for the more complicated latent-variable models with time-series structure.
We study parameter recovery under two setups, one being the standard hidden Markov model with discrete latent and observables, and the other being a model also with a hidden Markov structure but the observables are conditionally Gaussian given the latent.

% \paragraph{Contributions}
The contributions of this work are two-fold.
First, as a conceptual contribution, we identify a close connection between identifiability via self-supervised learning, and identifiability of model parameters from low-rank tensor decomposition~\citep{kruskal77,allman2009identifiability}.
The latter is a classical topic in theoretical computer science, and the basis of many efficient algorithms for latent-variable model learning~\citep{anandkumar2012multiview,anandkumar2014tensor}.
As a second contribution, we provide a complete characterization of the type of prediction tasks sufficient for identifiability. In particular, we analyze tasks involving up to three tokens, in any order and configuration.
Specifically, we show that: \textcolor{Orange}{(to be updated)}
\vspace{-1em}
\begin{itemize}[leftmargin=*]
\item In both HMMs and state space models, tasks involving only 2 tokens (i.e. predicting $x_t | x_{t-1}$ and/or $x_t|x_{t+1}$) are insufficient to identify the parameters of the model.

\item In both HMMs and state space models, tasks involving 3 tokens (i.e. 
$x_S | x_{\{t-1,t,t+1\} \setminus S}$ or $ x_{\{t-1,t,t+1\} \setminus S} | x_S$
for any $S \subseteq \{t-1,t,t+1\}, |S| = 2$)   
\end{itemize} 
We emphasize that the identifiability results require the predictor to have a correct parametric form.
\textcolor{gray}{todo: take into account the structure of data, contrasting this with merely treating them as sufficient statistics.}


\subsection{Related works}

\paragraph{Self-supervised applications}

Concurrent to the advances in NLP, there has also been a flourishing line of work in visual representation learning.
Pioneering works include designing tasks to utilize spatial relations \citep{relPos15,jigsaw16}, image inpainting \citep{inpaint16}, and leveraging global properties such as colorization \cite{color16} or image orientation \citep{rotation18}.
Classic ideas such as contrast or masked prediction also prove helpful in their modern realizations~\citep{CPC,CPCv2,simclr,iGPT,MAE21}, constantly pushing the state of the art performance and even surpassing supervised pretraining in various aspects \textcolor{grass}{(cite)}.

\paragraph{Evaluating self-supervised models}
The most common quality measure for self-supervised representation learning is the performance of downstream tasks.
Empirically, it is common to evaluate representations on their transfer performance, such as evaluating visual representations on objection detection and segmentation~\citep{inpaint16,simclr}, or evaluating language embeddings on various semantic and syntactic tasks such as question answering~\citep{bert,GPT2} \textcolor{grass}{(cite more)}.
On the theoretical front, analyses are available both on masked predictions~\citep{predictLee20,promptWei21} and contrastive methods~\citep{arora2019theoretical,multiViewTosh20,topicTosh21,WangIsola20,Zixin20}.
In contrast, few work has analyzed using self-supervised methods for parameter recovery.
While the learned representations in \cite{Zixin20} also reveal the model parameters, they used a sparse-coding model for the data and a contrastive objective as the self-supervised task, both of which are very different from our setting.

\paragraph{Latent variable models and tensor methods}
\textcolor{gray}{\textcolor{Orange}{todo}: nonlinear ICA (Hyvarinen); Daniel's works; Geoff Gordon's paper.}


==> COLT2022/bak/Feb6th_4pm/2.setup.tex <==
\section{Setup}
\label{sec:setup}

This work considers two latent-variable sequence models, the first is the fully discrete hidden Markov models (HMM), and the second is HMMs whose observables marginally follow a mixtures of Gaussians with identity covariance.
We will denote the observations and hidden states by $\{x_t\}_{t\geq 1}$ and $\{h_t\}_{t \geq 1}$, respectively.

\subsection{Discrete Hidden Markov Model}

For the discrete case, let $\Obs$ denote the observation space with $d := |\Obs|$, and let $\States$ be the state space with $k := |\States|$.
We assume $d \geq k$.
To simplify notation, let $\Obs = \{e_1,\dotsc,e_d \} \subset \R^d$ and $\States = \{e_1,\dotsc,e_k \} \subset \R^k$, where $e_i$ is the $i^{\text{th}}$ vector in the standard basis, i.e., $[e_i]_i = 1$, $[e_i]_j = 0$ for $j \neq i$.
% 
The parameters of interests are the \textit{transition matrix} $\mTrans \in \R^{k \times k}$ and the \textit{emission matrix} $\mEmiss \in \R^{d \times k}$; the linear parameterization is without loss of generality since the hidden states and the observables are both discrete.
With $\mEmiss, \mTrans$, the dynamics of the model can be written as
\begin{align}
  \E[h_{t+1} \mid h_t] & = \mTrans h_t, \\
  \E[x_t \mid h_t] & = \mEmiss h_t.
\end{align}

\subsection{Conditionally-Gaussian HMM (\GHMM)}

%% Note: (the naming: acronyms; speech-recognition)

Next, we consider a HMM where the observations follow a Gaussian with identity covariance when conditioned on the hidden states; we will abbreviate this setup as \textit{\GHMM}.
The state space $\gH := \{e_1, ..., e_k\} \subset \R^k$ is the same as in the discrete case, while the observation space is now continuous with $\gX := \R^d$, for $d \geq k$.
% 
The parameters of interests are the transition matrix $\mTrans \in \R^{k \times k}$, and the means of the $k$ Gaussians $\{\mu_i\}_{i \in [k]} \subset \R^{d}$; that is, $P(x_t|h_t = \ve_i) = (2\pi)^{-\frac{d}{2}} \exp\Big(-\frac{\|x-\mu_i\|^2}{2}\Big)$.
Denoting by $\mMeans := [\mu_1, \dotsc, \mu_k] \in \R^{d \times k}$ the matrix whose columns are the conditional means, we can write the dynamics of the model as
\begin{equation}
\begin{split}
    \E[h_{t+1}|h_t] =& \mTrans h_t,
    \\
    \E[x_t|h_t = e_i] =& \mMeans h_t = \mu_{i}.
\end{split}
\end{equation}


\subsection{Masked prediction tasks}

We are interested in the regression task of predicting masked out tokens conditioned on certain observed ones.
For example, we may predict the token $x_2$ given $x_1$, or predict the joint of two tokens $x_1 \otimes x_3$ given $x_2$.
Denoting the tensor of predicted tokens as $\otimes_{i} \xpred_i$, and the tensor of conditioned tokens as $\otimes_j \xcond_j$, 
we can write the optimal predictor for this prediction task as
\begin{equation}
\begin{split}
    f(\otimes_j \xcond_j) 
    = \E[\otimes_i \xpred_i | \otimes_j \xcond_j]
\end{split}
\end{equation}
The predictor may have superscript to make explicit the set of parameters.
As an example, consider the simplest case of predicting $x_2$ given $x_{1}$ under the discrete HMM.
The optimal predictor is
\begin{equation*}
\begin{split}
  &f^{2|1}(x; \mTrans, \mEmiss)
  = \E[x_2|x_1] = \sum_{i \in [k]} \E[x_2|h_2=i] P(h_2=i|x_1)
  \\
  =& \sum_{i \in [k]} \sum_{j \in [k]} \E[x_2|h_2=e_i] P(h_2=e_i|h_1=e_j) \underbrace{P(h_1=e_j|x_1)}_{:= [\phi(x_1)]_j}
  = \sum_{i \in [k]} \sum_{j \in [k]} \mEmiss_{i} \mTrans_{ij} \underbrace{\frac{\mEmiss_{x_1,j}}{\sum_{l \in [k]} \mEmiss_{x_1,l}}}_{:= [\phi(x_1)]_j}
\end{split}
\end{equation*}
Here with a slight abuse of notation, we used $x_1$ to index the matrix $\mEmiss$, where $x_1$ is treated as $x_1 \in [d]$ when being used as an index.
We will use $\phi: \R^d \rightarrow \R^k$ to denote the posterior distribution over the hidden state given the observable, i.e. $\phi(x_1) = \E[h_1 | x_1]$.

\textcolor{Orange}{todo: what we mean by identifiability for multiple tasks}
mainly for non-identifiable results


\subsection{Tensor decomposition}

Our identifiability results ties closely to the uniqueness of tensor decompositions.
A tensor is a multidimensional array that can be considered as a generalization of matrices; for example, a matrix can be treated as a second order tensor (or 2-tensor).
Similar to matrices, we can define rank for tensors. The \textit{tensor rank} is defined to be the minimal number $\tRank$ such that $\mW$ can be written as a sum of $\tRank$ rank-1 tensors.
For instance, if a $t$-tensor $\mW$ has rank-$\tRank$, it means $\mW$ can be written as the sum of $\tRank$ rank-1 tensors, i.e. $\mW = \sum_{i \in [r]} \otimes_{j \in [t]} U_i^{(j)}$ for some matrices $\mU^{(j)} \in \R^{n_j \times r}$, where $U_i^{(j)}$ denotes the $i^{\text{th}}$ column of matrix $\mU^{(j)}$.

In this work, we will focus on 3-tensors of the form $\mW = \sum_{i \in [\tRank]} A_i \otimes B_i \otimes C_i$ for some matrices $\mA \in \R^{n_1 \times \tRank}$, $\mB \in \R^{n_2 \times \tRank}$, $\mC \in \R^{n_3 \times \tRank}$.
The reason for considering 3-tensors is that 3 is the minimum order sufficient for identifiability.
\footnote{To apply our results on higher order tensors, one can consider an order-3 slice of the higher order tensor.}
A classic work by \cite{kruskal77} gives a sufficient condition under which $\mA, \mB, \mC$ can be recovered up to column-wise permutation and scaling.
The condition is stated in terms of the \textit{Kruskal rank}, which is the maximum number $\kRank$ such that any $\kRank$ columns of the matrix are linearly independent.
Let $k_A$ denote the Kruskal rank of matrix $\mA$, then:
%  Kruskal's result states that:
\vspace{-1em}
\begin{proposition}[Kruskal's theorem, \cite{kruskal77}]
\label{prop:kruskal}
  The components $\mA, \mB, \mC$ of a 3-tensor $\mW := \sum_{i\in[\tRank]} A_i \otimes B_i \otimes C_i$ are identifiable up to a shared column-wise permutation and scaling if $k_A + k_B + k_C \geq 2\tRank + 2$.
\end{proposition}
\vspace{-1em}
% \textcolor{Orange}{todo: tensor preliminaries: e.g. \href{https://www.cs.utah.edu/~bhaskara/files/tensor-unique.pdf}{Kruskal}}
We note that this work focuses on identifiability result rather than providing an algorithm, though the proofs can be adapted into algorithms using \textcolor{peach}{Jennrich's algorithm} \citep{Jennrich70} under slightly more restrictive conditions.


\paragraph{Assumptions}
We next state the assumptions used in our results.
The first assumption is that the transition matrices of the HMMs are doubly stochastic.
\vspace{-1em}
\begin{assumption}[Doubly stochastic transitions]
\label{assump:latent}
  The transition matrix $\mTrans$ is doubly stochastic.
  Further, assume $h_1$ is at stationarity, i.e. $\pi^{(1)}(i) = \frac{1}{k}$, $\forall i \in [k]$.
\end{assumption}
\vspace{-1em}
This assumption guarantees that the stationary distribution of the latent distribution is uniform for any $t$, and the transition matrix for the reversed chain is simply $\mTrans^\top$.
Moreover, this assumption reduces the parameter space and hence will make the non-identifiability results stronger.
\textcolor{Orange}{add a remark: (how) can we remove this?}

We require the following non-degeneracy condition on the parameters, for both the discrete HMM and \GHMM:
\vspace{-1em}
\begin{assumption}[Non-degeneracy, discrete HMM]
\label{assump:discrete_full_rank}
$\rank(\mTrans) = \rank(\mEmiss) = k \leq d$.
\end{assumption}
% 
\vspace{-1.5em}
\begin{assumption}[Non-degeneracy, \GHMM]
\label{assump:gmm_full_rank}
$\rank(\mTrans) = \rank(\mMeans) = k \leq d$.
\end{assumption}
\vspace{-1em}
The results in this work are on population level quantities, hence we only need the parameters to be degenerate, rather than bounded away from 0.

Lastly, for \GHMM, we assume that the norms of the means are known and equal:
\vspace{-1em}
\begin{assumption}[Equal norms of the means] 
\label{assump:gmm_equal_norms}
  $\forall i \in [k]$, $\|\mu_i\|_2 = C$ for some known constant $C$.
\end{assumption}

\textcolor{Orange}{remark: strong / standard / essential}

==> COLT2022/bak/Feb6th_4pm/3.discrete.tex <==
\section{Learning with discrete hidden Markov models}

Our goal is to characterize the types of prediction task that enables parameter recovery.
For sufficient conditions, prior work by \cite{kruskal77}
% and \cite{anandkumar2014tensor}
and \cite{allman2009identifiability}
have shown that third-order moments suffice for parameter identifiability.
%  we only need to focus on tasks involving tensors of order no more than 3.
Regarding necessary conditions, it is well-known in the factor analysis literature that matrices (i.e. second-order moments) are insufficient for identifiability in general, unless under additional conditions such as sparsity~\citep{donoho2003optimally,candes2006stable,spielman2012exact,arora2014new}, low-rankness~\citep{georgiev2005sparse,aharon2006uniqueness,cohen2019identifiability}, or orthogonality.
% \textcolor{Orange}{(todo: other citations?)}

Given results in prior work, it seems natural to use tasks which predict 3 masked out tokens.
It turns out that we can do better: predicting only 1 or 2 tokens can suffice for identifiability, provided that the task involves three tokens when counting also the conditioned tokens:
\vspace{-1em}
\begin{theorem}[Identifiability of masked prediction task on three tokens]
% \label{lem:discrete_two_given_one}
\label{thm:discrete}
    % Let $t_1, t_2,t_3$ be distinct time steps.
    Let $(t_1, t_2, t_3)$ be any permutation of $(1,2,3)$.
    Under Assumption \ref{assump:latent}, \ref{assump:discrete_full_rank},
    %  \ref{assump:discrete_distinct_diag},
    if the predictor has \emph{\textcolor{Orange}{the correct parametric form}},
    then parameters $\tilde\mEmiss, \tilde\mTrans$ of the the optimal predictors for the following tasks are the same as the ground truth $\mEmiss, \mTrans$ up to permutation:
    \vspace{-0.8em}
    \begin{enumerate}
        \item the task of predicting $x_{t_2} \otimes x_{t_3}$ given $x_{t_1}$;
        \item the task of predicting $x_{t_3}$ given $x_{t_1} \otimes x_{t_2}$ (\textcolor{Orange}{todo}).
        % \item \textcolor{Orange}{[todo]} the tasks of predicting $x_{t_2}$ given $x_{t_1}$, and predicting $x_{t_3}$ given $x_{t_1}$.
    \end{enumerate}
    %  then $f^{t_2,t_3|t_1}(\cdot; \mTrans, \mEmiss) = f^{t_2,t_3|t_1}(\cdot; \tilde\mTrans, \tilde\mEmiss)$ implies $\tilde\mTrans = \mTrans$, $\tilde\mEmiss = \mEmiss$.
\end{theorem}
The proof of Theorem \ref{thm:discrete} works by constructing a third-order tensor from the conditional second-order tensors given by the masked prediction task, for which Kruskal's theorem gives identifiability up to column-wise permutation and scaling.
The indeterminacy in scaling can be further removed since columns of $\mTrans$ sum up to 1.

As a remark, the choice of time step $1,2,3$ can be generalized to $\tOne, \tTwo, \tThr$ provided that they contain at least one pair of adjacent time steps.
We cannot generalize beyond adjacent time steps though, as shown by the following result:
\vspace{-1em}
\begin{theorem}[Nonidentifiability from large time gaps]
\label{thm:power_nonId}
    Let $\tOne, \tTwo, \tThr$ be distinct time steps such that any pair of time steps are at least 2 steps apart.
    Then, there exist parameters $\mMeans,\mTrans$ and $\tilde\mMeans, \tilde\mTrans$ following Assumption \ref{assump:latent}. \ref{assump:discrete_full_rank},
    such that $\tilde{\mTrans} \neq \mPerm\mTrans$ for any permutation $\mPerm$, yet one of the following is satisfied:
    % \vspace{-0.4em}
    % \begin{itemize}[leftmargin=*]
        1) $f_{\mMeans,\mTrans}^{\tTwo, \tThr|\tOne}(x_\tOne) = f_{\tilde\mMeans,\tilde\mTrans}^{\tTwo, \tThr|\tOne}(x_\tOne)$, $\forall x_\tOne$;
        or 2) $f_{\mMeans,\mTrans}^{\tThr|\tOne, \tTwo}(x_\tOne, x_\tTwo) = f_{\tilde\mMeans,\tilde\mTrans}^{\tThr|\tOne, \tTwo}(x_\tOne, x_\tTwo)$.
    % \end{itemize}
\end{theorem}
\vspace{-0.5em}
The intuition is that the conditional distribution of one token given another is defined with the transition matrix raised to the power of the difference in time.
When the time steps are at least 2 steps apart, matching the predictors only matches the matrix power, which however does not imply the transition matrices themselves are the same.

Moreover, we note that it is indeed necessary for the prediction task to involve three tokens.
The following result show that if each task involves only two tokens, then the parameters are not identifiable even when considering multiple tasks together:
\vspace{-1em}
\begin{theorem}[Nonidentifiability of pairwise masked prediction tasks]
\label{thm:discrete_nonId}
    Under Assumption \ref{assump:latent}, \ref{assump:discrete_full_rank},
    % \ref{assump:discrete_distinct_diag},
    when the predictor has the correct parametric form,
    parameters $\tilde\mEmiss, \tilde\mTrans$ of the the optimal predictors for the following tasks even when the predictor learns all pairwise prediction tasks $x_{t_2} | x_{t_1}$ for any $t_1, t_2 \in \{1,2,3\}$.
\end{theorem}
\vspace{-1em}
\textcolor{draftGray}{\textcolor{Orange}{todo}: the non-identifiability result can generalize to generic timesteps as well? e.g. we know that $\mTrans^2 = \tilde\mTrans^2$ doesn't imply $\mTrans = \tilde\mTrans$; the same likely applies to other powers as well.}

% \subsection{Identifiability from predicting a single token}
% Next, we show that with proper conditioning, predicting a single token also suffices for parameter recovery:
% \vspace{-1em}
% \begin{theorem}[Identifiability of predicting a single token, conditioned on two]
% \label{lem:discrete_one_given_two}
%     Consider the task of \textcolor{peach}{predicting $x_{t_3}$ given $x_{t_1} \otimes x_{t_2}$},
%     where $t_1, t_2,t_3$ are distinct time steps.
%     Under Assumption \ref{assump:discrete_uniform_latent}, \ref{assump:discrete_full_rank}, \ref{assump:discrete_distinct_diag}, if the predictor has \emph{\textcolor{Orange}{the correct parametric form}}, then
%     $f^{t_3|t_1,t_2}(\cdot; \mTrans, \mEmiss) = f^{t_3|t_1, t_2}(\cdot; \tilde\mTrans, \tilde\mEmiss)$ implies $\tilde\mTrans = \mTrans$, $\tilde\mEmiss = \mEmiss$.
% \end{theorem}
% \textcolor{Orange}{todo: merge the two lemmas into 1 theorem}


% We note that it is important to predict the two tokens jointly.
% Learning both the task of $x_{t_2} | x_{t_1}$ and $x_{t_3} | x_{t_1}$ also gives identifiability.
% For this negative result, let's consider a more restricted set of parameters, where the emission matrix is also row normalized.
% \vspace{-1em}
% \begin{assumption}[Row normalization]
% \label{assump:discrete_row_normed}
%     $\forall i \in [d]$, $\sum_{j \in [k]}B_{ij} = 1$.
% \end{assumption}
% The following lemma states that a pair of single-token prediction tasks cannot guarantee identifiability even under the additional assumption of row normalization:
% \vspace{-1em}
% \begin{lemma}[\textcolor{Orange}{Identifiability} of predicting a pair of single tokens, conditioned on one]
% \label{lem:discrete_pair_single}
%     Let $\mTrans, \tilde\mTrans \in \R^{d \times k}$, $\mEmiss, \tilde\mEmiss \in \R^{k \times k}$ satisfy Assumption \ref{assump:discrete_uniform_latent}, \ref{assump:discrete_full_rank}, and \ref{assump:discrete_distinct_diag}.
%     %  and \ref{assump:discrete_row_normed}.
%     For any distinct time steps $t_1, t_2, t_3$, if the predictor has \emph{\textcolor{Orange}{the correct parametric form}}
%     then having $f^{t_2|t_1}(\cdot; \mTrans, \mEmiss) = f^{t_2|t_1}(\cdot; \tilde\mTrans, \tilde\mEmiss)$ and $f^{t_3|t_1}(\cdot; \mTrans, \mEmiss) = f^{t_3|t_1}(\cdot; \tilde\mTrans, \tilde\mEmiss)$ implies $\tilde\mTrans = \mTrans$, $\tilde\mEmiss = \mEmiss$.
%     % Then, there exist an infinite number of $\tilde\mTrans \in \R^{d \times k}, \tilde\mEmiss \in \R^{k \times k}$ satisfying the same assumptions, such that $f^{2|1}(\cdot ; \mTrans,\mEmiss) = f^{2|1}(\cdot ; \tilde\mTrans, \tilde\mEmiss)$ and $f^{3|1}(\cdot ; \mTrans,\mEmiss) = f^{3|1}(\cdot ; \tilde\mTrans, \tilde\mEmiss)$.
% \end{lemma}





==> COLT2022/bak/Feb6th_4pm/4.gmm.tex <==
\section{Learning with conditionally-Gaussian HMMs}
% \section{Learning with Gaussian mixture hidden Markov models}


Contrasting to HMM, pairwise prediction of a single token already suffices for identifiability:
\begin{theorem}[Identifiability of \GHMM~ from predicting $x_2$ given $x_1$]
\label{thm:gmm_2_1_id}
    Under Assumption \ref{assump:latent}, \ref{assump:gmm_full_rank}, and \ref{assump:gmm_equal_norms},
    if $\mMeans, \mTrans$ and $\tilde\mMeans, \tilde\mTrans$ give the same predictor for $x_2$ given $x_1$,
    then it must be that $\tilde\mMeans$ is equal to (up to permutation) either $\mMeans$ or $\mR\mMeans$,
    where $\mR$ is a unique Householder transformation.
\end{theorem}
\textcolor{gray}{\textcolor{Orange}{Note}: Assumption \ref{assump:gmm_equal_norms} says the norms of the means are equal and known.}

\textcolor{Orange}{todo: organize results on 3 tokens.}
\textcolor{gray}{(even if we can already get the same identifiability from $x_2|x_1$, it's still interesting to see that the tensor decomposition proof can be applied to \GHMM, rather than just HMM.)}

%% Commenting out previous theorem statements
% \input{COLT2022/not_used/gmm_previous_statements}


==> COLT2022/bak/Feb6th_4pm/5.proofs_discrete.tex <==
\section{Proofs for HMM results}

\subsection{Proof of Theorem \ref{thm:discrete}}

% \textcolor{Orange}{todo: explain why backward prediction incurs $\mTrans^\top$}

We will prove the identifiability for each prediction task individually.

\textcolor{Orange}{highlight the difference bewteen discrete and Gaussian case}
(e.g. explain the invariances; why 1 case id for Gaussian but not for discrete, and 1 case the other way around.)

\textcolor{Orange}{explain how/why the tensor is contructed}


\input{COLT2022/proof_HMM/draft_noJoint}

% \input{COLT2022/proof_HMM/proof_with_kruskal}


\input{COLT2022/proof_HMM/hmm_23_1}

\input{COLT2022/proof_HMM/hmm_13_2}


\subsection{Proof for Theorem \ref{thm:discrete_nonId}: non-identifiability of pairwise prediction tasks on HMM}

% We again summarize all six possible orderings into two configurations: one is $\tOne < \tTwo < \tThr$, and the other is $\tTwo < \tOne < \tThr$.

% \paragraph{Case I, $\tOne < \tTwo < \tThr$}
% The optimal predictors are
% \begin{equation}
% \begin{split}
%   f^{\tTwo|\tOne}(x_\tOne)
%   :=& \E[x_\tTwo| x_\tOne]
%   = \sum_{i,j \in [k]} \E[x_\tTwo | h_\tTwo=\ej] P(h_\tTwo=\ej|h_\tOne=\ei) P(h_\tOne=\ei|x_\tOne)
%   \\
%   =& \sum_{j\in [k]} \mEmiss_j \sum_{i\in[k]} (\mTrans^{\tTwo-\tOne})_{ij} [\phi(x_\tOne)]_i
%   = \mEmiss \mTrans^{\tTwo-\tOne} \phi(x_\tOne),
%   \\
%   f^{\tThr|\tOne}(x_\tThr)
%   :=& \E[x_{\tThr}|x_\tOne]
%   = \mEmiss \mTrans^{\tThr-\tOne} \phi(x_\tOne).
% \end{split}
% \end{equation}
% To construct a 3-tensor for which Kruskal's theorem applies,
% suppose there exists a set \textcolor{Orange}{$\gS_k := {x^{(i)}}_{i\in[k]}$ such that $\Phi_k := [\phi(x^{(1)}), ..., \phi(x^{(k)})] \in \R^{k \times k}$ is of rank $k$} \textcolor{gray}{(e.g. by using ``anchors")}.
% Consider the following tensor:
% \begin{equation}
% \begin{split}
%     &\Tensor_\weight :=
%     \sum_{x_{\tOne} \in \gS_k} x_{\tOne} \otimes \E[x_{\tTwo}|x_{\tOne}] \otimes \E[x_{\tThr}|x_{\tOne}]
%     \\
%     =& \sum_{x_\tOne \in \gS_k} x_\tOne \otimes \mEmiss\mTrans^{\tTwo-\tOne}\phi(x_\tOne) \otimes \mEmiss \mTrans^{\tThr-\tOne} \phi(x_\tOne)
%     \\
% \end{split}
% \end{equation}
% The three components of $\Tensor_\weight$ are $\mA := [x^{(1)}, ..., x^{(k)}]$, $\mB := \mEmiss\mTrans^{\tTwo-\tOne}\Phi_k$, $\mC := \mEmiss\mTrans^{\tThr-\tOne}\Phi_k$, which are all of Kruskal rank $k$.
% Therefore Kruskal's theorem applies, and we recover the columns of $\mEmiss\mTrans^{\tThr-\tTwo} \mEmiss^{\dagger}$.

% \textcolor{RoyalBlue}{// special case: 1) $\phi(x) = \mEmiss^\top x$, and 2) learning with $x_2|x_1$ and $x_3|x_1$}

Let's start with the tasks of predicting $x_2$ given $x_1$ and predicting $x_3$ given $x_1$.
We will find a counterexample where $\tilde\mTrans \neq \mP\mTrans$ for any permutation matrix $\mP$, yet $\tilde\mMeans, \tilde\mTrans$ form an optimal predictor for predicting both $x_2|x_1$ and $x_3|x_1$.
Moreover, we will make $\mTrans, \tilde\mTrans$ symmetric, so that $\tilde\mTrans, \tilde\mMeans$ also form an optimal predictor for the reversed direction, i.e. for predicting $x_1|x_2$ and $x_1|x_3$.

In our counterexample, let's consider the ground truth and learned emission matrices $\mEmiss, \tilde\mEmiss$ with rows summing up to $\frac{k}{d}$, such that the posterior function is simply $\phi(x) = \frac{\mEmiss^\top x}{\|\mEmiss^\top x\|_1} = \frac{d}{k} \mEmiss^\top x$, and similarly $\tilde\phi(x) = \frac{d}{k}\tilde{\mEmiss}^\top x$.
The optimal predictors are of the form:
\begin{equation}
\begin{split}
  f^{2|1}(x) = \mEmiss\mTrans\phi(x) = \frac{d}{k}\mEmiss\mTrans\mEmiss^\top x,~
  f^{3|1}(x) = \mEmiss\mTrans^2\phi(x) = \frac{d}{k}\mEmiss\mTrans^2 \mEmiss^\top x.
\end{split}
\end{equation}
Matching $f^{2|1} = \tilde{f}^{2|1}$ on all $x \in \gX := \{\ei\}_{i \in [d]}$ means
\begin{equation}\label{eq:31_21_part1}
\begin{split}
  &\mEmiss\mTrans\mEmiss^\top \mI_d = \mEmiss\mTrans\mEmiss^\top
  = \tilde\mEmiss \tilde\mTrans \tilde\mEmiss^\top 
  \Rightarrow \tilde\mTrans = \tilde\mEmiss^\dagger \mEmiss \cdot \mTrans \cdot (\tilde\mEmiss^\dagger \mEmiss)^{\top}.
  \\
\end{split}
\end{equation}
We also have $f^{3|1} = \tilde{f}^{3|1}$, i.e. $\mEmiss\mTrans^2\mEmiss^\top = \tilde\mEmiss \tilde\mTrans^2 \tilde\mEmiss^\top$, hence 
\begin{equation}\label{eq:discrete_nonid_31}
\begin{split}
  &\tilde\mEmiss \tilde\mTrans^2 \tilde\mEmiss^\top
  = \tilde{\mEmiss} \tilde\mEmiss^\dagger \mEmiss \mTrans (\tilde\mEmiss^\dagger \mEmiss)^\top \cdot \tilde\mEmiss^\dagger \mEmiss \mTrans (\tilde\mEmiss^\dagger \mEmiss)^\top \tilde\mEmiss^\top 
  \eqLabel{1}= \mEmiss \mTrans \cdot (\tilde\mEmiss^\dagger \mEmiss)^\top \tilde\mEmiss^\dagger \mEmiss \cdot \mTrans\mEmiss^\top 
  \\
  =&~ \mEmiss \mTrans \cdot \mTrans\mEmiss
  \Rightarrow (\tilde\mEmiss^\dagger \mEmiss)^\top \cdot \tilde\mEmiss^\dagger \mEmiss = \mI_k,
\end{split}
\end{equation}
where step $\rnum{1}$ uses $\tilde\mEmiss\tilde\mEmiss^\dagger \mEmiss = \mEmiss$, since $\tilde\mEmiss, \mEmiss$ share the same column space.

Equation \ref{eq:discrete_nonid_31} means $\mR := \tilde\mEmiss^\dagger \mEmiss$ is orthogonal.
% i.e. $\tilde\mEmiss = \mEmiss \mR$,
To construct a counterexample, consider $k=3$, and let $\mR$ represent a rotation whose rotation axis is $\frac{1}{3}e_1 + \frac{1}{3}e_2 + \frac{1}{3}e_3$.
Such choice of rotation axis is the direction pointing from the origin to the projection of the origin on the hyperplane $\gP_c := \{v \in \R^d: \sum_{i\in[d]} v_i =c\}$ for any positive constant $c$. Such rotation guarantees $\mR v \in \gP_c$, $\forall v \in \gP_c$, and has the following property:
\vspace{-1em}
\begin{claim}
\label{clm:rotation_sumRowCol}
    Each row and each column of $\mR$ sum up to 1.
\end{claim}
% 
Define $\tilde\mEmiss := \mEmiss\mR$, $\tilde\mTrans := \mR^\top \mTrans \mR$, Claim \ref{clm:rotation_sumRowCol} ensures that row sum and column sum of $\tilde\mEmiss, \tilde\mTrans$ remain the same as those of $\mEmiss, \mTrans$.
When the rotation angle represented by $\mR$ is sufficiently small, entries $\tilde\mEmiss, \tilde\mTrans$ remain in $[0,1]$, hence such $\tilde\mEmiss, \tilde\mTrans$ form a valid counterexample.
To show the existence of such $\mR$, the following is a concrete example for $d = 4$, $k=3$:
{\small
\begin{equation}
\begin{split}
  &\mEmiss = \begin{bmatrix}
    0.23016003 & 0.3549092  & 0.16493077 \\
    0.30716059 & 0.06962305 & 0.37321636 \\
    0.2580854  & 0.26965425 & 0.22226035 \\
    0.20459398 & 0.3058135  & 0.23959252
  \end{bmatrix},
  ~\tilde\mEmiss = \begin{bmatrix}
    0.24120928 & 0.35062535 & 0.15816537 \\
    0.28937626 & 0.07433156 & 0.38629218 \\
    0.26077674 & 0.26749114 & 0.22173212 \\
    0.20863772 & 0.30755194 & 0.23381033
  \end{bmatrix},
  \\
  &\mTrans = \begin{bmatrix}
    0.56893146 & 0.35811118 & 0.07295736 \\
    0.35811118 & 0.10805638 & 0.53383243 \\
    0.07295736 & 0.53383243 & 0.39321021
  \end{bmatrix},
  ~\tilde{\mTrans} = \begin{bmatrix}
    0.59740926 & 0.30452087 & 0.09806987 \\
    0.30452087 & 0.1331689  & 0.56231024 \\
    0.09806987 & 0.56231024 & 0.33961989
  \end{bmatrix},
  \\
  & \det(\mEmiss) = \det(\tilde\mEmiss) = 0.0110,
  \det(\mTrans) = \det(\tilde\mTrans) = -0.1611.
\end{split}
\end{equation}
}
Note that $\mTrans, \tilde\mTrans$ are both symmetric, which means this is also a valid counter example for learning to predict all of $x_2|x_1$, $x_1|x_2$, $x_3|x_1$, $x_1|x_3$.


% \textcolor{RoyalBlue}{// special case: learning with $x_2|x_1$ and $x_3|x_1$, general $\mEmiss$}

% For general emission matrices, the posterior is $\phi(x) = \frac{\mO^\top x}{\|\mO^\top x\|_1}$.
% The optimal predictors are
% \begin{equation}
% \begin{split}
%   f^{2|1}(x) = \mEmiss\mTrans\frac{\mEmiss^\top x}{\|\mEmiss^\top x\|_1},~
%   f^{3|1}(x) = \mEmiss\mTrans^2\frac{\mEmiss^\top x}{\|\mEmiss^\top x\|_1}.
% \end{split}
% \end{equation}
% % 
% Matching $f^{2|1} = \tilde{f}^{2|1}$ on all $x \in \gX := \{\ei\}_{i \in [d]}$ means
% \begin{equation}
% \begin{split}
%   % &\mEmiss\mTrans\mEmiss^\top \mI_d \cdot \diag([\|\mEmiss_i^\top\|_1]_{i\in[d]})^{-1}
%   &\mEmiss\mTrans\mEmiss^\top \diag([\|\mEmiss_i^\top\|_1]_{i\in[d]})^{-1}
%   = \tilde\mEmiss \tilde\mTrans \tilde\mEmiss^\top \diag([\|\tilde\mEmiss_i^\top\|_1]_{i\in[d]})^{-1}
%   \\
%   \Rightarrow&~ \tilde\mTrans = \tilde\mEmiss^\dagger \mEmiss \cdot \mTrans \cdot \mEmiss^\dagger \diag\big(\big[\|\tilde\mEmiss_i^\top\|_1/\|\mEmiss_i^\top\|_1\big]_{i\in[d]}\big) \tilde\mEmiss.
% \end{split}
% \end{equation}
% We also have $f^{3|1} = \tilde{f}^{3|1}$, i.e. $\mEmiss\mTrans^2 \mEmiss^\top \diag([\|\mEmiss_i^\top\|_1]_{i\in[d]})^{-1} = \tilde\mEmiss \tilde\mTrans^2 \tilde\mEmiss^\top \diag([\|\tilde\mEmiss_i^\top\|_1]_{i\in[d]})^{-1}$.
% Hence 
% \begin{equation}
% \begin{split}
%   &\mEmiss\mTrans^2 \mEmiss^\top \diag([\|\mEmiss_i^\top\|_1]_{i\in[d]})^{-1} \cdot (\mEmiss\mTrans \mEmiss^\top \diag([\|\mEmiss_i^\top\|_1]_{i\in[d]})^{-1})^\dagger
%   = \mEmiss\mTrans\mEmiss^\dagger = \tilde{\mEmiss} \tilde\mTrans \tilde\mEmiss^\top 
%   \\
%   \Rightarrow& \tilde\mTrans = \tilde\mEmiss^\dagger \mEmiss \cdot \mTrans \cdot \mEmiss^\dagger \tilde\mEmiss
% \end{split}
% \end{equation}
% % 
% Combining the above two equations we get 
% \begin{equation}
% \begin{split}
%   &\mEmiss^\dagger \diag([\|\mEmiss_i^\top\|_1]_{i\in[d]})^{-1}\diag([\|\tilde\mEmiss_i^\top\|_1]_{i\in[d]}) \tilde\mEmiss
%   = \mEmiss^\dagger \tilde\mEmiss 
%   \\
%   \Rightarrow&~ \mEmiss\mEmiss^\dagger \diag([\|\mEmiss_i^\top\|_1]_{i\in[d]})^{-1} = \tilde\mEmiss \tilde\mEmiss^\dagger \diag([\|\tilde\mEmiss_i^\top\|_1]_{i\in[d]})^{-1}
% \end{split}
% \end{equation}
% \textcolor{Orange}{(todo: can we find a counterexample from this?)}


% \textcolor{RoyalBlue}{// special case: 1) $\phi(x) = \mEmiss^\top x$, and 2) learning with $x_1|x_2$ and $x_3|x_2$}

For the task of predicting both $x_1|x_2$ and $x_3|x_2$ (i.e. conditioning on the middle token of a triplet), since there is no connection between $x_1$ and $x_3$, this task gives the same information as predicting both $x_1|x_2$ and $x_2|x_1$, which is not identifiable.

% Same as the previous case, assume $\mEmiss, \tilde\mEmiss$ are row-normalized so that $\phi(x)= \mEmiss^\top x$.
% The optimal predictors are $f^{1|2}(x) = \mEmiss\mTrans^\top \mEmiss^\top x, ~f^{3|2}(x) = \mEmiss\mTrans \mEmiss^\top x$.
% Matching the predictors using all $d$ choices of $x$ gives
% $\mEmiss\mTrans^\top \mEmiss^\top = \tilde\mEmiss \tilde\mTrans^\top \tilde\mEmiss$ and $\mEmiss\mTrans \mEmiss^\top = \tilde\mEmiss \tilde\mTrans \tilde\mEmiss^\top$, which are the transpose of each other.
% This case is \textcolor{Orange}{not identifiable} even by parameter counting.

% Since the prediction task doesn't relate $x_1$ and $x_3$, this is the same as predicting both $x_2|x_1$ and $x_1|x_2$, which we have shown a counterexample for \GHMM (i.e. by rotation).
% For the discrete case, we can similarly find an counterexample by setting $\tilde\mEmiss$ to be a perturbed version of $\mEmiss$, such that $\tilde\mTrans := \tilde\mEmiss^\dagger \mEmiss \cdot \mTrans \cdot \mEmiss^\dagger \diag\big(\big[\|\tilde\mEmiss_i^\top\|_1/\|\mEmiss_i^\top\|_1\big]_{i\in[d]}\big) \tilde\mEmiss$ is a valid transition matrix.
% For example, let $\mEmiss$ have rows summing up to $\frac{k}{d}$ for simplicity, and perturb entries of $\mEmiss$ such that $\tilde\mEmiss$ also has rows summing up to $\frac{k}{d}$. Then when the perturbation is sufficiently smaller, $\tilde\mEmiss^\dagger \mEmiss$ is close to the identity, hence $\tilde\mTrans$ stays a valid transition matrix.
% The previous counterexample hence also applies here.

% The following is another concrete counterexample:
% \small{
% \begin{equation}
% \begin{split}
%   &\mEmiss = \begin{bmatrix}
%     0.62722885 & 0.18672434 & 0.18604681 \\
%     0.23736775 & 0.62612608 & 0.13650617 \\
%     0.13540341 & 0.18714958 & 0.67744701\\
%   \end{bmatrix},~
%   \tilde\mEmiss = \begin{bmatrix}
%     0.38078711 & 0.3394932  & 0.27971969 \\
%     0.3394932  & 0.37590462 & 0.28460219 \\
%     0.27971969 & 0.28460219 & 0.43567812\\
%   \end{bmatrix},
%   \\
%   &\mTrans = \begin{bmatrix}
%     0.57720127 & 0.31134919 & 0.11144955 \\
%     0.31134919 & 0.50962391 & 0.1790269 \\
%     0.11144955 & 0.1790269  & 0.70952355\\
%   \end{bmatrix},~
%   \tilde\mTrans = \begin{bmatrix}
%     0.55989204 & 0.24172041 & 0.19838755 \\
%     0.24172041 & 0.51634238 & 0.24193721 \\
%     0.19838755 & 0.24193721 & 0.55967524 \\
%   \end{bmatrix},
%   \\
%   &\det(\mEmiss) = 0.2159, ~\det(\tilde\mEmiss) = 0.2448,
%   ~\det(\mTrans) = 01275, ~\det(\tilde\mTrans) = 0.0992.
% \end{split}
% \end{equation}
% }

%% Buggy proof commented out: problem was on the conditioning of $h_\tTwo$
% \input{COLT2022/not_used/discrete_31_21_wrong.tex}


%% The following is the wrong proof for *non*-identifiability: the problem is that $\tilde\mEmiss := \mEmiss\mR$ can no longer be a valid emission matrix.
% The optimal predictors for $x_2$ given $x_1$ and $x_3$ given $x_1$ are $\E_W[x_2|x_1] = \mEmiss\mTrans\phi(x_1)$ and $\E_W[x_3|x_1] = \mEmiss\mTrans^2 \phi(x_1)$ respectively.
% Under Assumption \ref{assump:discrete_row_normed} that the rows of $\mEmiss$ sum up to 1, we have $\phi(x) = \mEmiss^\top x$, then matching these two equations are the same as matching $\mEmiss\mTrans\mEmiss^\top$ and $\mEmiss\mTrans^2\mEmiss^\top$.
% This is not sufficient for identifiable, since for any orthogonal $\mR \in \R^{k\times k}$ such that $\mR\mTrans\mR^\top$ is a valid stochastic matrix, $\tilde\mTrans = \mR\mTrans\mR^\top$, $\tilde\mEmiss = \mEmiss\mR$ can satisfy the two conditions.
% \textcolor{Orange}{todo: double check with numerical example}


%
\subsubsection{Proof of Claim \ref{clm:rotation_sumRowCol}}
  Let's first check that the columns of $\mR$ sum up to 1.
  Denote $\simplex_d := \{x\in \R^d: \sum_{i\in[d]} x_i = 1\}$.
  Any $v \in \gP_c$ can be written as $v = c\cdot [\alpha_1, \alpha_2, ..., \alpha_{d-1}, 1-\sum_{i\in[d-1]}\alpha_i]$ for some $[\alpha_1, ..., \alpha_{d-1}] \in \simplex_{d-1}$.
  Let $r_i$ denote the $i_{th}$ row of $\mR$,
  then $\mR v \in \gP_c$ means $\sum_{i \in [d]} \langle r_i, v \rangle = \langle \sum_{i \in [d]} r_i, v \rangle = c$.
  Let $\beta_j$ denote the $j_{th}$ coordinate of $\sum_{i\in[d]} r_i$, then
  \begin{equation}
  \begin{split}
    &\sum_{i\in[d-1]} \beta_i\alpha_i + \beta_d \big(1 - \sum_{i \in [d-1]}\alpha_i\big) = 1,~ \forall [\alpha_1, ..., \alpha_{d-1}] \in \simplex_{d-1}
    \\
    \Rightarrow& \sum_{i \in [d-1]} (\beta_i - \beta_d) \alpha_i + \beta_d = 1, ~ \forall [\alpha_1, ..., \alpha_{d-1}] \in \simplex_{d-1}
    \\
    \Rightarrow&~ \beta_i = 1,~ \forall i \in [d].
  \end{split}
  \end{equation}
  It then follows that $\mR^{-1} = \mR^\top$ also has columns summing up to 1, since 
  \begin{equation}
  \begin{split}
    \sum_{i\in[d]} (\mR\mR^{-1})_{ij}
    = \langle\sum_{i\in[d]} r_i, (\mR^{-1})_j\rangle
    = \langle \1, (\mR^{-1})_j\rangle
    = 1,~\forall j \in [d].
  \end{split}
  \end{equation}


\subsection{Proof of Theorem \ref{thm:power_nonId}: nonidentifiability of large time gaps}

The theorem is a direct consequence of the following lemma:
\vspace{-1em}
\begin{lemma}
\label{lem:transPower_nonId}
      For any positive integer $t$, there exist doubly stochastic matrices $\mTrans, \tilde{\mTrans}$ such that $\mTrans \neq \tilde\mTrans$, and $\mTrans^t = \tilde\mTrans^{t}$. 
\end{lemma}
\vspace{-1em}
In particular, the proof is complete by setting $\tilde\mEmiss = \mEmiss$, and $\tilde\mTrans$ to be an example for Lemma \ref{lem:transPower_nonId}.

We now prove Lemma \ref{lem:transPower_nonId}.
\begin{proof}[Lemma \ref{lem:transPower_nonId}]
% 
% We will provide counterexamples for $\mTrans^t = \tilde\mTrans^t$ yet $\mTrans \neq \tilde\mTrans$, for $t$ being even or odd separately.
% 
% \textbf{Even $t$} The counterexample uses symmetric $\mTrans, \tilde\mTrans$.
% The idea is that symmetric matrices are guaranteed to have eigendecomposition with real eigenvalues. However, matching even powers of the matrices only ensures the eigenvalues of $\mTrans, \tilde\mTrans$ share the same absolute values, but the signs of the eigenvalues can still differ.
% The following shows a concrete example where $\mTrans^2 = \tilde\mTrans^2$:
% {\small
% \begin{alignat*}{2}
%     &\mTrans = \begin{bmatrix}
%         0.57336879 & 0.14364175 & 0.28298946 \\
%         0.14364175 & 0.50741389 & 0.34894437 \\
%         0.28298946 & 0.34894437 & 0.36806617 \\
%     \end{bmatrix},
%     &&~\tilde\mTrans = \begin{bmatrix}
%         0.56613875 & 0.13080026 & 0.30306098 \\
%         0.13080026 & 0.48460574 & 0.38459399 \\
%         0.30306098 & 0.38459399 & 0.31234503 \\
%     \end{bmatrix},
%     \\
%     &\lambda(\mTrans) = [1, 0.40596918, 0.04287966],
%     &&~\lambda(\tilde\mTrans) = [1, 0.40596918, -0.04287966].
% \end{alignat*}}
% 
% \textbf{Odd $t$} 
The intuition for finding a counterexample is that we can let $\tilde\mTrans$ be a rotation of $\mTrans$. For any $t$, set the rotation angle to be $\frac{2\pi}{t}$, so that $\tilde\mTrans = \mR \mTrans \neq \mTrans$, yet $\tilde\mTrans^t = \mTrans^t \mR^t = \mTrans^t$.
The following shows one implementation of this idea.
Choose $a \in [0,1]$, and let the ground truth parameters be 
\begin{equation*}
\begin{split}
    \mTrans =& \begin{bmatrix}a & 0 & 1-a \\ 1-a & a & 0 \\ 0 & 1-a & a \end{bmatrix},
    ~\mMeans = \begin{bmatrix}1 & -1/2 & -1/2 \\ 0 & \sqrt{3}/2 & \sqrt{3}/2 \\ 1/\sqrt{2} & 1/\sqrt{2} & 1/\sqrt{2} \end{bmatrix}.
    \\
\end{split}
\end{equation*}
Let $\theta$ be some rotation angle, and denote by $\mR_2(\theta) := \begin{bmatrix} \cos(\theta) & -\sin(\theta) & 0 \\ \sin(\theta) & \cos(\theta) & 0 \\ 0 & 0 & 1 \end{bmatrix}$ a rotation that acts on the first two dimensions.
It can be checked that for any $\theta \in \R$, we have \textcolor{Orange}{(why?)}
\begin{equation}
\begin{split}
  \big(\mMeans^{-1} \big(\mR_2(\theta)\big)^{-1} \mMeans\big) \cdot \mTrans
    % = \begin{bmatrix}0.8123 & 0.0583 & 0.1294 \\ 0.1294 & 0.8123 & 0.0583 \\ 0.0583 & 0.1294 & 0.8123 \end{bmatrix}
    = \mTrans \cdot \big(\mMeans^{-1} \big(\mR_2(\theta)\big)^{-1} \mMeans\big).
\end{split}
\end{equation}
Since $\mR_2(\theta)$ represents a rotation of angle $\theta$, $\big(\mR_2(\theta)\big)^{\tau}$ corresponds to a rotation of angle $\tau\theta$ for any integer $\tau$ ($\tau$ could be negative).
Let $\theta := \frac{2\pi}{t}$, then 
\begin{equation}
\begin{split}
  \tilde\mTrans^t
  =& \big(\mMeans^{-1} \big(\mR_2(\theta)\big)^{-1} \mMeans \cdot \mTrans\big)^t
  = \mTrans^{t} \big(\mMeans^{-1} \big(\mR_2(\theta)\big)^{-1} \mMeans)\big)^{t}
  = \mTrans^t \mMeans^{-1} \big(\mR_2(\theta)\big)^{-t} \mMeans
  \\
  =& \mTrans^t \mMeans^{-1} \cdot \mR_2(2\pi) \cdot \mMeans
  = \mTrans^t.
\end{split}
\end{equation}
Finally, it can be checked that for every $t$, there exists a choice of $a$ such that $\tilde\mTrans := \mR\mTrans$ where $\mR := \mMeans^{-1}\big(\mR_2(\frac{2\pi}{t})\big)^{-1}\mMeans$ has entries bounded within $[0,1]$.
Hence such $\tilde\mTrans$ serves as a valid counterexample.
\end{proof}


==> COLT2022/bak/Feb6th_4pm/6.proofs_gmm.tex <==
\section{Proofs for conditionally-Gaussian HMMs}

\input{COLT2022/proof_GHMM/draft_fixBug}

% 
%% Comment out the buggy non-id proof: phi shouldn't be the same for $\tilde{M} = RM$.
% \input{COLT2022/not_used/gmm_pairwise_nonId_buggyPhi.tex}




==> COLT2022/bak/Feb9th_11am/2.setup.tex <==
\section{Setup}
\label{sec:setup}

This work focuses on two classes of latent-variable sequence models. The first are fully discrete hidden Markov models (HMMs), and the second are HMMs whose observables marginally follow a mixtures of Gaussians with identity covariance.
We will denote the observations and hidden states by $\{x_t\}_{t\geq 1}$ and $\{h_t\}_{t \geq 1}$, respectively.
The hidden states $h_1 \to h_2 \to \dotsb$ form a Markov chain, and conditional on $h_t$, the observable $x_t$ is independent of all other variables.
Throughout, we refer to the observations $\{x_t\}_{t\geq 1}$ as tokens, following the nomenclature from language models.

\subsection{Discrete Hidden Markov Model}

We first describe the parameterization of (discrete) HMMs.
Let $\Obs$ denote the observation space with $d := |\Obs|$, and let $\States$ be the state space with $k := |\States|$.
%We assume $d \geq k$.
To simplify notation, let $\Obs = \{e_1,\dotsc,e_d \} \subset \R^d$ and $\States = \{e_1,\dotsc,e_k \} \subset \R^k$, where $e_i$ is the $i^{\text{th}}$ vector in the standard basis, i.e., $[e_i]_i = 1$, $[e_i]_j = 0$ for $j \neq i$.
% 
The parameters of interest are the \textit{transition matrix} $\mTrans \in \R^{k \times k}$ and the \textit{emission matrix} $\mEmiss \in \R^{d \times k}$.
%the linear parameterization is without loss of generality since the hidden states and the observables are both discrete.
With $\mEmiss, \mTrans$, the dynamics of the model can be written as:
\begin{equation*}
  \E[h_{t+1} \mid h_t = e_i] = \mTrans e_i, \qquad
  \E[x_t \mid h_t = e_i] = \mEmiss e_i .
\end{equation*}

\subsection{Conditionally-Gaussian HMM (\GHMM)}

%% Note: (the naming: acronyms; speech-recognition)

We next describe the parameterization of \emph{conditionally-Gaussian HMMs ({\GHMM}s)}.
%Next, we consider a HMM where the observations follow a Gaussian with identity covariance when conditioned on the hidden states; we will abbreviate this setup as \textit{\GHMM}.
The state space $\gH := \{e_1, \dotsc, e_k\} \subset \R^k$ is the same as in the discrete case, while the observation space is now continuous with $\gX := \R^d$.
% 
The parameters of interest are the transition matrix $\mTrans \in \R^{k \times k}$, and the means of the $k$ identity-covariance Gaussians $\{\mu_i\}_{i \in [k]} \subset \R^{d}$; that is, $P(x_t = x \mid h_t = \ve_i) = (2\pi)^{-\frac{d}{2}} \exp(-\|x-\mu_i\|^2/2)$.
We let $\mMeans := [\mu_1, \dotsc, \mu_k] \in \R^{d \times k}$ be the matrix whose columns are the conditional means, so we can write the dynamics of the model as:
\begin{equation*}
    \E[h_{t+1} \mid h_t = e_i] = \mTrans e_i, \qquad
    \E[x_t \mid h_t = e_i] = \mMeans e_i = \mu_{i}.
\end{equation*}


\subsection{Masked prediction tasks}

We are interested in the (regression) task of predicting one or more ``masked out'' tokens as a function of another observed token, with the goal of minimizing expected squared loss under a distribution given by an HMM or \GHMM.
For example, we may want to predict the token $x_2$ from $x_1$, or predict the tensor product of tokens $x_1 \otimes x_3$ from $x_2$.
%We will denote the tensor of predicted tokens as $\otimes_{i} \xpred_i$, and the tensor of conditioned tokens as $\otimes_j \xcond_j$.
Since the objective is the expected squared loss, the optimal predictor of the tensor product of tokens $\otimes_i \xpred_i$ from another token $\xcond$ is provided by the conditional expectation operator:
\begin{equation*}
%\begin{split}
    f(\xcond) 
    = \E[\otimes_i \xpred_i  \mid \xcond] .
%\end{split}
\end{equation*}
%We will denote in the superscript the configuration of the prediction task.
For instance, consider the case of predicting $x_2$ given $x_{1}$ under the HMM with parameters $(\mEmiss,\mTrans)$.
The optimal predictor, denoted by $f^{2|1}$, can be written in terms of $(\mEmiss,\mTrans)$ as
\begin{equation*}
\begin{split}
  &f^{2|1}(x)
  = \E[x_2 \mid x_1] = \sum_{i \in [k]} \E[x_2 \mid h_2=i] P(h_2=i \mid x_1)
  \\
  =& \sum_{i \in [k]} \sum_{j \in [k]} \E[x_2 \mid h_2=e_i] P(h_2=e_i \mid h_1=e_j) \underbrace{P(h_1=e_j \mid x_1)}_{:= [\phi(x_1)]_j}
  = \sum_{i \in [k]} \sum_{j \in [k]} \mEmiss_{i} \mTrans_{ij} \underbrace{\frac{\mEmiss_{x_1,j}}{\sum_{l \in [k]} \mEmiss_{x_1,l}}}_{:= [\phi(x_1)]_j} .
\end{split}
\end{equation*}
Here with a slight abuse of notation, we used $x_1$ to index the matrix $\mEmiss$, where $x_1$ is treated as $x_1 \in [d]$ when being used as an index.
We will use $\phi: \R^d \rightarrow \R^k$ to denote the posterior distribution of a hidden state $h_t$ given the corresponding observation $x_t$, i.e., $\phi(x_t) = \E[h_t  \mid  x_t]$.

% \Anote{Wonder if this should be a definition?} 
Our goal is to study the parameter identifiability from the prediction tasks, when the predictors have the correct parametric form.
Formally, we define identifiability from a prediction task as follows:
%For instance, identifiability from a prediction task on HMM refers to:
%\Anote{Optimal predictors? not clear otherwise}
%\vspace{-0.8em}
\begin{definition*}[Identifiability from a prediction task, HMM]
  A prediction task suffices for identifiability if, for any two HMMs with parameters $(\mEmiss,\mTrans)$ and $(\tilde\mEmiss,\tilde\mTrans)$, equality of their optimal predictors for this task implies that there is a permutation matrix $\Pi$ such that $\mEmiss = \tilde\mEmiss \Pi$ and $\mTrans = \tilde\mTrans \Pi$.
%  A prediction task suffices for identifiability, if for any two predictors $f, \tilde{f}$ parameterized by $\mEmiss,\mTrans$ and $\tilde\mEmiss, \tilde\mTrans$,
%  $f = \tilde{f}$ implies that $\mEmiss = \tilde\mEmiss$ and $\mTrans = \tilde\mTrans$, up to a permutation of labeling.
\end{definition*}
%\vspace{-0.6em}
In other words, the mapping from the equivalence classes of HMMs to optimal predictors for a task is injective, where equivalence is considered up to a shared column-wise permutation of the parameter matrices $O$ and $T$.
%
By identifiability from a collection of prediction tasks, we refer to the injectiveness of the mapping from equivalence classes of HMMs to collections of optimal predictors for all such tasks.
%Moreover, by identifiability from multiple prediction tasks, we refer to the same definition as above, except that now the two set of parameters must produce the same predictors for all of the tasks simultaneously.
Identifiability for {\GHMM}s is defined analogously with $\mEmiss,\tilde\mEmiss$ changed to $\mMeans,\tilde\mMeans$.

\subsection{Tensor decomposition}

Our identifiability results tie closely to the uniqueness of \emph{tensor rank decompositions}~\citep{hitchcock1927expression}.
An \emph{order-$t$ tensor} (or \emph{$t$-tensor}) is an $t$-way multidimensional array; a matrix is a 2-tensor.
%Similar to matrices, we can define rank for tensors.
The \textit{tensor rank} of a tensor $\mW$ is the minimum number $\tRank$ such that $\mW$ can be written as a sum of $\tRank$ rank-1 tensors.
That is, if a $t$-tensor $\mW$ has rank-$\tRank$, it means that $\mW = \sum_{i \in [r]} \otimes_{j \in [t]} \mU_i^{(j)}$ for some matrices $\mU^{(j)} \in \R^{n_j \times r}$, where $U_i^{(j)}$ denotes the $i^{\text{th}}$ column of matrix $\mU^{(j)}$.

In this work, we only need to work with 3-tensors of the form $\mW = \sum_{i \in [\tRank]} A_i \otimes B_i \otimes C_i$ for some matrices $\mA \in \R^{n_1 \times \tRank}$, $\mB \in \R^{n_2 \times \tRank}$, $\mC \in \R^{n_3 \times \tRank}$, as 3-tensors will suffice for identifiability in all of our settings of interest. 
\footnote{To apply our results on higher order tensors, one can consider an order-3 slice of the higher order tensor.}
A classic work by \cite{kruskal77} gives a sufficient condition under which $\mA, \mB, \mC$ can be recovered up to column-wise permutation and scaling.
The condition is stated in terms of the \textit{Kruskal rank}, which is the maximum number $\kRank$ such that every $\kRank$ columns of the matrix are linearly independent.
Let $k_A$ denote the Kruskal rank of matrix $\mA$, then:
%  Kruskal's result states that:
%\vspace{-1em}
\begin{proposition}[Kruskal's theorem, \cite{kruskal77}]
\label{prop:kruskal}
  The components $\mA, \mB, \mC$ of a 3-tensor $\mW := \sum_{i\in[\tRank]} \mA_i \otimes \mB_i \otimes \mC_i$ are identifiable up to a shared column-wise permutation and column-wise scaling if $k_A + k_B + k_C \geq 2\tRank + 2$.
\end{proposition}
%\vspace{-1em}
% \textcolor{Orange}{todo: tensor preliminaries: e.g. \href{https://www.cs.utah.edu/~bhaskara/files/tensor-unique.pdf}{Kruskal}}
We note that this work focuses on identifiability result rather than providing an algorithm, though the proofs can be adapted into algorithms \citep[see, e.g.,][]{Jennrich70} under slightly more restrictive conditions (which will be satisfied by all of our identifiability results).


\subsection{Assumptions}

We now state the assumptions used in our results.
The first assumption is that the transition matrices of the HMMs are doubly stochastic.
%\vspace{-1em}
\begin{assumption}[Doubly stochastic transitions]
\label{assump:latent}
  The transition matrix $\mTrans$ is doubly stochastic, and the marginal distribution of the initial hidden state $h_1$ is stationary with respect to $\mTrans$.
%  Further, assume $h_1$ is at stationarity, i.e. $\pi^{(1)}(i) = \frac{1}{k}$, $\forall i \in [k]$.
\end{assumption}
%\vspace{-1em}
This assumption guarantees that the stationary distribution of the latent distribution is uniform for any $t$, and the transition matrix for the reversed chain is simply $\mTrans^\top$.
Moreover, this assumption reduces the parameter space and hence will make the non-identifiability results stronger.
% \textcolor{Orange}{add a remark: (how) can we remove this? -- answer: we can't.} 

We require the following conditions on the parameters for the discrete HMM:
%\vspace{-1em}
\begin{assumption}[Non-redundancy, discrete HMM]
\label{assump:discrete_rowNE}
    Every row of $\mEmiss$ is non-zero.
\end{assumption}
%\vspace{-1em}
Assumption \ref{assump:discrete_rowNE} can be interpreted as requiring each token to have a non-zero probability of being observed, which is a mild assumption.
% 
We also require the following non-degeneracy condition:
%\vspace{-1em}
\begin{assumption}[Non-degeneracy, discrete HMM]
\label{assump:discrete_full_rank}
$\rank(\mTrans) = \rank(\mEmiss) = k \leq d$.
\end{assumption}
%\vspace{-1em}
Note that Assumption \ref{assump:discrete_full_rank} only requires the parameters to be non-degenerate, rather than have singular values bounded away from 0.
The reason is that this work will focus on population level quantities and make no claims on finite sample behaviors or robustness.

For \GHMM, we similarly require the parameters to be non-degenerate:
%\vspace{-1em}
\begin{assumption}[Non-degeneracy, \GHMM]
\label{assump:gmm_full_rank}
$\rank(\mTrans) = \rank(\mMeans) = k \leq d$.
\end{assumption}
%\vspace{-1em}
Moreover, we assume that the norms of the means are known and equal:
%\vspace{-1em}
\begin{assumption}[Equal norms of the means] 
\label{assump:gmm_equal_norms}
  For each $i \in [k]$, $\mu_i$ is a unit vector.
%  
%  $\forall i \in [k]$, $\|\mu_i\|_2 = C$ for some known constant $C$.
\end{assumption}
(Assumption~\ref{assump:gmm_equal_norms} can be changed to $\|\mu_i\|_2=c$ for all $i \in [k]$, for any other fixed number $c>0$.)

% 
Assumptions \ref{assump:latent}-\ref{assump:gmm_full_rank} are fairly standard~\citep[see, e.g.,][]{anandkumar2012multiview}; Assumption \ref{assump:gmm_equal_norms} may be an artifact of our proofs, and it would be interesting to relax in future work.
%It will be an interesting future direction to see how to relax these conditions.

Our notion of identifiability from a prediction task (or a collection of prediction tasks) will restrict attention to HMMs satisfying Assumptions \ref{assump:latent}, \ref{assump:discrete_rowNE}, \ref{assump:discrete_full_rank} and {\GHMM}s satisfying Assumptions \ref{assump:latent}, \ref{assump:gmm_full_rank}, \ref{assump:gmm_equal_norms}.



==> COLT2022/not_used/discrete_31_21_wrong.tex <==

To construct a 3-tensor for which Kruskal's theorem applies,
let $\weight(x_{\tOne})$ be some weighting defined on $x_{\tOne}$.
Consider the following tensor:
\begin{equation}
\begin{split}
    &\Tensor_\weight :=
    \sum_{x_{\tOne} \in \gS_k} x_{\tOne} \otimes \E[x_{\tTwo}|x_{\tOne}] \otimes \E[x_{\tThr}|x_{\tOne}]
    \\
    =& \sum_{x_{\tOne}} \weight(x_{\tOne}) x_{\tOne}
      \otimes \Big(\sum_{i\in[k]} P(h_{\tTwo}=i|x_\tOne)\E[x_\tTwo|h_\tTwo=i]\Big)
      \otimes \Big(\sum_{j\in[k]} P(h_{\tTwo}=j|x_\tOne)\E[x_\tTwo|h_\tTwo=j]\Big)
    \\
    =& \sum_{x_{\tOne}} \weight(x_{\tOne}) x_{\tOne} \otimes \sum_{i \in [k]} \E[x_{\tTwo}|h_\tTwo=i] \otimes \E[x_{\tThr}|h_\tTwo=i] \cdot P(h_\tTwo)
    \\
    =& \sum_{x_{\tOne}} \sum_{i\in[k]} \weight(x_{\tOne}) P(h_{\tTwo}=i|x_{\tOne}) x_{\tOne} \otimes \E[x_{\tTwo}|h_{\tTwo}=i] \otimes \E[x_{\tThr}|h_{\tTwo}=i]
    \\
    =& \sum_{i\in[k]} \Big(\sum_{x_{\tOne}}  \weight(x_{\tOne}) P(h_{\tTwo}=i|x_{\tOne}) x_{\tOne}\Big) \otimes \E[x_{\tTwo}|h_{\tTwo}=i] \otimes \E[x_{\tThr}|h_{\tTwo}=i]
\end{split}
\end{equation}
Take $\weight(x_{\tOne}) = P(x_{\tOne})$, then the first component on $x_\tOne$ is 
\begin{equation}
\begin{split}
  \sum_{x_{\tOne}} P(x_{\tOne}) P(h_{\tTwo}=i|x_{\tOne}) x_{\tOne}
  = P(h_\tTwo=i) \E[x_\tOne|h_\tTwo=i]
  = \Pstat{\tTwo}{i} \big(\mEmiss(\mTrans^{\tTwo-\tOne})^\top\big)_i
\end{split}
\end{equation}
Hence $\Tensor_\weight = \sum_{i\in[k]} \Pstat{\tTwo}{i} \big(\mEmiss(\mTrans^{\tTwo-\tOne})^\top\big)_i \otimes \mEmiss_i \otimes (\mEmiss(\mTrans^{\tThr-\tTwo}))_i$,
where the three components are all of Kruskal rank $k$ by Assumption \ref{assump:discrete_full_rank}.
Therefore Kruskal's theorem guarantees the recovery of $\mEmiss$ and $\mTrans^{\tThr-\tTwo}$, \textcolor{red}{hence also $\mTrans$}.


\paragraph{Case II, $\tTwo < \tOne < \tThr$}
The optimal predictors are
$f^{\tTwo|\tOne}(x_\tOne) = \mEmiss(\mTrans^{\tOne-\tTwo})^\top \phi(x_\tOne)$,
$f^{\tThr|\tOne}(x_\tOne) = \mEmiss\mTrans^{\tThr-\tOne} \phi(x_\tOne)$.
Let $\weight(x_{\tOne})$ be some weighting on $x_{\tOne}$, and consider the following third-order tensor:
\begin{equation}
\begin{split}
    \Tensor_\weight :=
    &\sum_{x_{\tOne}} \weight(x_{\tOne}) x_{\tOne} \otimes \E[x_{\tTwo}|x_{\tOne}] \otimes \E[x_{\tThr}|x_{\tOne}]
    \\
    =& \sum_{x_{\tOne}} \sum_{i\in[k]} \weight(x_{\tOne}) P(h_{\tOne}=i|x_{\tOne}) x_{\tOne} \otimes \E[x_{\tTwo}|h_{\tOne}=i] \otimes \E[x_{\tThr}|h_{\tOne}=i]
    \\
    =& \sum_{i\in[k]} \Big(\sum_{x_{\tOne}} \weight(x_{\tOne}) P(h_{\tOne}=i|x_{\tOne}) x_{\tOne}\Big) \otimes \E[x_{\tTwo}|h_{\tOne}=i] \otimes \E[x_{\tThr}|h_{\tOne}=i]
\end{split}
\end{equation}
Take $\weight(x_{\tOne}) = P(x_{\tOne})$, then the first component on $x_\tOne$ is 
\begin{equation}
\begin{split}
  \sum_{x_{\tOne}} P(x_{\tOne}) P(h_{\tOne}=i|x_{\tOne}) x_{\tOne}
  = P(h_\tOne=i) \E[x_\tOne|h_\tOne=i]
  = \Pstat{\tOne}{i} \mEmiss_i
\end{split}
\end{equation}
Hence $\Tensor_\weight = \sum_{i\in[k]} \Pstat{\tOne}{i} \mEmiss_i \otimes \big(\mEmiss(\mTrans^{\tOne-\tTwo})^\top\big)_i \otimes (\mEmiss(\mTrans^{\tThr-\tOne}))_i$,
where the three components are all of Kruskal rank $k$ by Assumption \ref{assump:discrete_full_rank}.
Therefore Kruskal's theorem recovers $\mEmiss$ and $\mTrans^{\tThr-\tOne}$, \textcolor{red}{hence also $\mTrans$}.

==> COLT2022/not_used/gmm_21_12.tex <==

\subsection{Proof for Lemma \ref{lem:gmm_nonid} and Corollary \ref{cor:gmm_12_21} (nonidentifiability of predicting a single token, conditioned on one)}

We provide a counterexample for Lemma \ref{lem:gmm_nonid}, in which $\mTrans, \tilde\mTrans$ are both symmetric, hence the same counterexample also applies to Corollary \ref{cor:gmm_12_21}.

% \begin{proof}
    We claim that there exists an orthogonal matrix $\mR\in \R^{d \times d}$ representing a rigid rotation,
    such that setting $\tilde\mMeans = \mR\mMeans$, $\tilde{\mTrans} = \mMeans^{-1}\mR^{-1}\mMeans \mTrans$ satisfies $\mMeans\mTrans = \tilde\mMeans\tilde\mTrans$, and $\frac{\|\mu_i - \tilde\mu_i\|_2}{\|\mu_i\|_2} \geq $, $\forall i\in[k]$; we leave the details to the end of the proof.

    Then, since $\tilde\mMeans$ is a rigid rotation of $\mMeans$, we have $\mu_i - \tilde{\mu}_i = \mu_j - \tilde{\mu}_j$ and $\|\mu_i\|^2 - \|\tilde\mu_i\|^2 = 0$, which implies $\phi(x) = \tilde{\phi}(x),\ \forall x$.
    % hence satisfying the necessary and sufficient condition for $\phi = \tilde{\phi}$.
    This is because the softmax is invariant to scaling, i.e. $\frac{\exp(-\|x - \mu_i\|^2)}{\sum_{j\in[k]} {\exp(-\|x -\mu_j\|^2)}} = \frac{\exp(-\|x - \mu_i\|^2 + c)}{\sum_{j\in[k]} {\exp(-\|x -\mu_j\|^2 + c)}}$ for any $c \in \R$.
    % Hence the sufficient and necessary condition for $\phi = \tilde\phi$ is simply:
    Hence:
    \begin{equation}
    \begin{split}
        &\forall i, j \in [k], \begin{cases}
            \mu_i - \tilde\mu_i = \mu_j - \tilde\mu_j, \\
            \|\tilde{\mu}_j\|^2 - \|\mu_j\|^2 = \|\tilde\mu_i\|^2 - \|\mu_i\|^2
        \end{cases}
        \\
        \Rightarrow&~ 2\left(\mu_i - \tilde{\mu}_i - (\mu_j - \tilde{\mu}_j)\right)^\top x = (\|\tilde{\mu}_j\|^2 - \|\mu_j\|^2) - (\|\tilde\mu_i\|^2 - \|\mu_i\|^2),  \ \forall i, j \in [k], \forall x \in \R^d
        \\
        \Rightarrow&~ \|x - \tilde{\mu}_i\|^2 - \|x - \mu_i\|^2 = \|x - \tilde{\mu}_j\|^2 - \|x - \mu_j\|^2, \ \forall i, j \in [k], \forall x \in \R^d.
        \\
    \end{split}
    \end{equation}
    Therefore we have $\mMeans\mTrans = \tilde\mMeans\tilde\mTrans$ and $\phi(x) = \tilde\phi(x),~\forall x \in \R^d$, hence $\mMeans\mTrans\phi = \tilde{\mMeans}\tilde\mTrans\tilde{\phi}$ and the proof is complete.

    Finally, to construct such a counterexample by rotation, we only need to make sure $\mTrans$ is still a valid stochastic matrix after the rotation, that is, entries of $\tilde\mTrans$ should lie in $[0, 1]$.
    We provide a 3-dimensional counterexample, which can be extended straightforwardly to higher dimensions.
    The idea is to let $\mu_1, \mu_2, \mu_3$ form a right triangle in a plane. Matching $\mMeans\mTrans$ means matching the convex combinations of the means, which lie within this right triangle (i.e. a convex hull).
    Denote these convex combinations as $v_1, v_2, v_3$, i.e. $[v_1, v_2, v_3] = \mMeans\mTrans$.
    Then, if the rigid rotation $\mR$ is sufficiently small (as determined by the conditioning of $\mTrans$), then $v_1, v_2, v_3$ still lie within the triangle formed by the rotated means $\tilde\mu_1, \tilde\mu_2, \tilde\mu_3$, which means there exists a stochastic matrix $\tilde\mTrans$ such that $\tilde\mMeans \tilde\mTrans = [v_1, v_2, v_3] = \mMeans\mTrans$.
    \textcolor{Orange}{(add figure to illustrate?)}
    
    As a concrete example,
    % (as shown in Figure \ref{fig:predictNext_wellSepc_2to1}),
    let $a = \frac{7}{8}$ and set:
    \begin{equation}
    \begin{split}
        &\mTrans = \begin{bmatrix}
            a & 0 & 1-a \\
            0 & 1-a & a \\
            1-a & a & 0 \\
        \end{bmatrix},
        ~\tilde\mTrans = \begin{bmatrix}
            a & 1-a & 0 \\
            1-a & 0 & a \\
            0 & a & 1-a \\
        \end{bmatrix},
        % \det(\tilde{\mTrans}) = -a^3 -(1-a)^3
        \\
        &\mM = \begin{bmatrix}
            1 & -1/2 & -1/2 \\
            0 & \sqrt{3}/2 & -\sqrt{3}/2 \\
            1 & 1 & 1
        \end{bmatrix},
        ~\tilde\mM = \mMeans\mTrans\tilde\mTrans^{-1}.
        \\
    \end{split}
    \end{equation}
    Here the rotation is $\mR = \tilde\mMeans\mMeans^{-1} = \mMeans\mTrans\tilde\mTrans^{-1} \mMeans^{-1}$.
    We now have $\mMeans \mTrans = \tilde\mMeans \tilde\mTrans = \mMeans\mTrans^\top = \tilde\mMeans \tilde\mTrans^\top$,
    but $\min_{\alpha}\frac{\|\mu_i - \tilde\mu_{\alpha(i)}\|_2}{\|\mu_i\|_2} > 0.2$, $\forall i \in [k]$.
% \end{proof}


==> COLT2022/not_used/gmm_23_1_extreme_points.tex <==
One choice could be $x^{(i)} = x_c^{(i)} := \mu_i + c (\mu_i - \nu_i)$ for some $\nu_i$, such that $\lim_{c\rightarrow \infty}\phi(x_c^{(i)}) \rightarrow \ei^{(k)}$; there exists a set of such $\{x^{(i)}: i \in [k]\}$ that is also linearly independent as we will show later.
Then
\begin{equation}
\begin{split}
    a_i :=& \sum_{j \in [k]} \phi(x_1=x_c^{(j)})^\top \mTrans^\top \ei^{(k)} x_c^{(j)}
    = [x_c^{(1)}, ..., x_c^{(k)}] [\phi(x_c^{(1)}), ..., \phi(x_c^{(k)})]^\top \mTrans^\top \ei^{(k)},
    \\
    \mA :=&~ [a_1, ..., a_k] = [x_c^{(1)}, ..., x_c^{(k)}] [\phi(x_c^{(1)}), ..., \phi(x_c^{(k)})]^\top \mTrans^\top.
\end{split}
\end{equation}
Thus each component of the tensor $\Tensor := \sum_{i \in [k]} a_i \otimes \mMeans_i \otimes (\mMeans\mTrans)_i$ has Kruskal rank $k$, and we can recover columns of $\mMeans, \mMeans\mTrans$ and hence also $\mTrans$.

We now show such choices of $\{\nu_i\}_{i \in[k]}$ exist.
First note that in order to have $\lim_{c\rightarrow \infty} \phi(x_c^{(i)}) \rightarrow \ei$, we need $\|x_c^{(i)} - \mu_j\|^2 - \|x_c^{(i)} - \mu_i\|^2 > 0$, $\forall j \neq i$,
which means 
\begin{equation}
\begin{split}
    (2x_c^{(i)} - \mu_i - \mu_j)^\top (\mu_i - \mu_j)
    = 2c\Big(\frac{1}{2c}(\mu_i - \mu_j) + (\mu_i - \nu_i)\Big)^\top (\mu_i - \mu_j) > 0
\end{split}
\end{equation}
As $c \rightarrow \infty$, we can ignore the $\frac{1}{2c}$ term and focus on $(\mu_i - \nu_i)^\top (\mu_i - \mu_j)$.
Since $\{\mu_i\}_{i \in [k]}$ is a linearly independent set, and the polytope formed by $\{\mu_i\}_{i \in [k]}$ is convex.
This means for each $i \in [k]$, there exists a hyperplane (strictly) separating $\mu_i$ and $\{\mu_j\}_{j \neq i}$,
and we can choose $\nu_i$ to be the projection of $\mu_i$ on such a hyperplane.

The final step is to show that the set $\{x_c^{(i)}\}_{i \in [k]}$ is linearly independent.
% \textcolor{gray}{\textcolor{Orange}{todo: show this}; e.g. can we make it s.t. $\{\mu_i - \nu_i\}_{i \in [k]}$ spans $(k-1)$-dimensional subspace, and $\{\mu_i\}_{i \in [k]}$ spans a $k$ dimensional subspace?}
% \textcolor{gray}{Can we pick the hyperplane to be the one formed by 3 ``closest'' vertices?}
We note that there must exist a hyperplane separating $\mu_i$ and all other $\{\mu_j\}_{j\neq i}$ such that the projection of $\mu_i$ on such hyperplane lies in the $(k-1)$-dimensional subspace that embeds the convex polytope formed by $\{\mu_i\}_{i \in [k]}$. \textcolor{Orange}{(is this true?)}
With these hyperplanes, the span of $\{\mu_i - \nu_i\}_{i \in [k]}$ is $(k-1)$-dimensional.
The span of $\{\mu_i\}_{i \in [k]}$ is $k$-dimensional, hence $c \rightarrow \infty$, the span of $\{\mu_i + c(\mu_i - \nu_i)\}_{i\in[k]} = \{x_c^{(i)}\}_{i \in [k]}$ is of $k$-dimensional.

\textcolor{gray}{Let $\mV_c := c[\mu_1-\nu_1, ..., \mu_k-\nu_k] \in \R^{d \times k}$. The null space of $\mEmiss + \mV_c$ is non-trivial only for a measure-zero set of $c$.}

\textcolor{Orange}{todo: use $x^{(i)} = \mu_i$.}

==> COLT2022/not_used/gmm_2_13_attempts_matchM.tex <==
we can choose $x$ s.t. $\phi(x) \rightarrow \ei$ for any $i \in [k]$.
This means $\forall i, j$ such that $\mTrans_{i}^\top \odot \mTrans_{j} \neq 0$,
we can pick $x_1, x_3$ s.t. 
\begin{equation}
\begin{split}
    &\phi_{13}(x_1, x_3)
    \rightarrow \frac{\mTrans_{i}^\top \odot \mTrans_{j}}{\|\mTrans_{i}^\top \odot \mTrans_{j}\|_1}
    % \rightarrow \frac{\mTrans_{ip} \mTrans_{qi}}{\sum_{j \in [k]} \mTrans_{jp} \mTrans_{qj}}, ~\forall p, q \in [k].
\end{split}
\end{equation}
\textcolor{RoyalBlue}{\textit{If $\mTrans, \tilde\mTrans$ are both symmetric}}, $\mTrans$ is directly determined from $\phi_{13}$ using the same argument as in the discrete case.
% \textcolor{gray}{(\textcolor{red}{this is wrong}, since $\phi(x) \rightarrow \ei$ does not mean $\phi_{13}$ has a term going to $\mTrans_{ip}$ due to normalization. e.g. if $\phi(x_1) \rightarrow e_1$, $\phi(x_3) \rightarrow e_2$, and $\mTrans = \mI$, then $\phi_{13}(x_1, x_3)$ can be anything.)}

Generic $\mTrans$: \textcolor{gray}{(in progress)}
Assuming for now that $\mTrans_i^\top \odot \mTrans_j \neq 0$, $\forall i, j \in [k]$.
Then $\mTrans = \tilde\mTrans$ iff $s_{ij} := \|\mTrans_i^\top \odot \mTrans_j\|_1 = \|\tilde\mTrans_i^\top \odot \tilde\mTrans_j\|_1 := \tilde{s}_{ij}$.
\textcolor{gray}{
\vspace{-0.8em}
\begin{itemize}[leftmargin=*]
    \item If $\mTrans_j = \tilde\mTrans_j$, then $s_{ij} = \tilde{s}_{ij}$:
    $(\sum_{i \in [k]} \frac{\tilde{s}_{ij}}{s_{ij}} \mTrans_i^\top) \odot \mTrans_j
        = (\sum_{i \in [k]} \tilde\mTrans_i^\top) \odot \tilde\mTrans_j
        = \tilde\mTrans_j$,
    i.e. the vector $\mTrans^\top[\frac{\tilde{s}_{ij}}{s_{ij}}]_{i\in[k]} = \frac{\tilde\mTrans_j}{\mTrans_j} = \1_k$, which has a unique solution where $\frac{\tilde{s}_{ij}}{s_{ij}} = 1$. 
    % 
    \item If $s_{ij} = \tilde{s}_{ij}$, then $\mTrans_j = \tilde\mTrans_j$:
    $(\sum_{i \in [k]}\mTrans_i^\top) \odot \mTrans_j = \mTrans_j = \tilde\mTrans_j$.
\end{itemize}
}

\begin{equation}
\begin{split}
    &\underbrace{\frac{\|\tilde\mTrans_i^\top \odot \tilde\mTrans_j\|_1}{\|\mTrans_i^\top \odot \mTrans_j\|_1}}_{:= r_{ij}} \mTrans_i^\top \odot \mTrans_j = \tilde\mTrans_i^\top \odot \tilde\mTrans_j
    \eqLabel{1}\Rightarrow~ \mTrans^\top r_{:j} \odot \mTrans_j = \tilde\mTrans_j
    \Rightarrow~ \mTrans^\top R \odot \mTrans = \tilde\mTrans
\end{split}
\end{equation}
where step $\rnum{1}$ sums over $i \in [k]$ on both sides.
Similarly we also have $\mTrans^\top \odot \mTrans R^\top = \tilde\mTrans^\top$, i.e. $\tilde\mTrans = R \mTrans^\top \odot \mTrans$.
If all entries of $\mTrans$ are positive, then $\mTrans^\top R = R^\top \mTrans^\top$.

==> COLT2022/not_used/gmm_2_13_wrong.tex <==
For the Gaussian case (\textcolor{peach}{identifiable}),
define the following 3-tensor similar to the discrete case:
\begin{equation}
\begin{split}
    &\Tensor
    := \int_{x_1, x_3} \tilde{p}(x_1, x_3) x_1 \otimes x_3 \otimes \tilde\E[x_2|x_1,x_3]
    \\
    =& \int_{x_1, x_3} \tilde{p}(x_1, x_3) \tilde{p}(h_2|x_1,x_2) x_1 \otimes x_3 \otimes \tilde\E[x_2|x_1, x_3, h_2]
    \\
    =& \sum_{h_2} \Big(\int_{x_1,x_2} \tilde{p}(x_1, x_3) \tilde{p}(h_2|x_1,x_2) x_1 \otimes x_3 \Big) \otimes \tilde\E[x_2|h_2]
    \\
    =& \sum_{h_2} \tilde{p}(h_2) \tilde\E[x_1|h_2] \otimes \tilde\E[x_3|h_2] \otimes \tilde\E[x_2|h_2]
    = \frac{1}{k}\sum_{i\in[k]} (\tilde\mMeans\tilde\mTrans^\top)_i \otimes (\tilde\mMeans\tilde\mTrans)_i \otimes \tilde\mMeans_i.
\end{split}
\end{equation}
On the other hand, since $\tilde\E[x_2|x_1,x_3] = \E[x_2|x_1,x_3]$, the above tensor can also be written as
\begin{equation}
\begin{split}
    \Tensor
    = \int_{x_1, x_3} \tilde{p}(x_1, x_3) x_1 \otimes x_3 \otimes \E[x_2|x_1,x_3]
    = \frac{1}{k}\sum_{i\in[k]} (\tilde\mMeans\tilde\mTrans^\top)_i \otimes (\tilde\mMeans\tilde\mTrans)_i \otimes \mMeans_i.
\end{split}
\end{equation}
Hence $\mMeans = \mMeans_i$ by applying Kruskal's theorem on $\Tensor$.
\textcolor{red}{how to determine the scaling?}

The optimal predictor takes the form $\E[x_2|x_1,x_3] = \mMeans\phi_{13}(x_1, x_3)$, hence matching both the predictor and $\mMeans$ means $\phi_{13}(x_1, x_3) = \tilde{\phi}(x_1, x_3)$.
Moreover, since the stationary distribution for the latent is uniform by Assumption \ref{assump:latent}, the marginal distribution on $x_3$ is also matched for the ground truth and the learned parameters.
Then the posterior vector of $h_2$ given $x_1$, denoted as $P(h_2|x_1) \in \R^k$, is also matched, since 
\begin{equation}
\begin{split}
    P(h_2|x_1)
    =& \int_{x_3} p(x_3=x) P(h_2|x_1, x)dx
    = \int_{x_3} p(x_3=x) \phi_{13}(x_1, x)dx
    \\
    =& \int_{x_3} \tilde{p}(x_3=x) \tilde\phi_{13}(x_1, x)dx
    = \tilde{P}(h_2|x_1).
\end{split}
\end{equation}
On the other hand, we also have $P(h_2|x_1) = \mTrans\phi(x_1)$.
Let the set $\gX := \{x^{(i)}: i \in [k]\}$ be such that ${\phi(x^{(i)}): x^{(i)} \in \gX}$ are linearly independent; one such choice could be $\gX = \{\mu_i: i \in [k]\}$ \textcolor{grass}{as explained earlier}.
Note also that $\phi(x) = \tilde\phi(x)$ since $\mMeans = \tilde\mMeans$.
Then
\begin{equation}
\begin{split}
    &[P(h_2|x^{(1)}), P(h_2|x^{(2)}), ..., P(h_2|x^{(k)})]
    = [\tilde{P}(h_2|x^{(1)}), \tilde{P}(h_2|x^{(2)}), ..., \tilde{P}(h_2|x^{(k)})]
    \\
    \Rightarrow& \mTrans \underbrace{[\phi(x^{(1)}), \phi(x^{(2)}), ..., \phi(x^{(k)})]}_{:= \Phi}
        = \tilde\mTrans[\phi(x^{(1)}), \phi(x^{(2)}), ..., \phi(x^{(k)})]
    \\
    \Rightarrow& \mTrans = \tilde\mTrans,
\end{split}
\end{equation}
where the last step is because the matrix $\Phi$ is of rank $k$ by the choice of $\gX$.

==> COLT2022/not_used/gmm_31_21_generic_wrong.tex <==
As an example \textcolor{Orange}{(do we need to duplicate the full proofs?)}, let's check the identifiability from predicting $x_\tTwo|x_\tOne$ and $x_\tThr|x_\tOne$, where $\tOne < \tTwo < \tThr$.
The optimal predictor is the same as in the discrete case, i.e. 
$f^{\tTwo|\tOne}(x_\tOne) := \E[x_\tTwo|x_\tOne]
        = \mMeans \mTrans^{\tTwo-\tOne}\phi(x_\tOne)$,
and similarly $f^{\tThr|\tOne}(x_\tOne) := \E[x_\tThr|x_\tOne]
        = \mMeans \mTrans^{\tThr-\tOne}\phi(x_\tOne)$.
Let $\weight(x_\tOne)$ be some weighting on $x_\tOne$, and consider the following tensor:
\begin{equation}
\begin{split}
    &\Tensor_\weight 
    := \sum_{x_\tOne} \weight(x_\tOne)  x_\tOne \otimes \E[x_\tTwo|x_\tOne] \otimes \E[x_\tThr|x_\tOne]
    \\
    =& \sum_{x_\tOne} \weight(x_\tOne) x_\tOne \otimes \sum_{i,j \in [k]} P(h_\tTwo=j|h_{\tOne}=i) [\phi(x_\tOne)]_{i} \cdot \E[x_\tTwo|h_\tTwo=j] \otimes \E[x_\tThr|h_\tTwo=j]
    \\
    =& \sum_{j \in [k]} \Big(\sum_{i \in [k]} \sum_{x_\tOne} \weight(x_\tOne) P(h_\tOne=i|x_\tOne) P(h_\tTwo=j|h_\tOne=i) x_\tOne \Big) \otimes \mMeans_j \otimes (\mMeans\mTrans^{\tThr-\tTwo})_j
\end{split}
\end{equation}
Take $\weight(x_\tOne) = P(x_\tOne)$, then the first component involving $x_\tOne$ is 
\begin{equation}
\begin{split}
    &\sum_{i \in [k]} \sum_{x_\tOne} P(x_\tOne) P(h_\tOne=i|x_\tOne) P(h_\tTwo=j|h_\tOne=i) x_\tOne 
    \\
    =& \sum_{i \in [k]} \Big(\sum_{x_\tOne} P(x_\tOne|h_\tOne=i) x_\tOne\Big) \cdot P(h_\tOne=i, h_\tTwo=j)
    \\
    =& P(h_\tTwo=j) \cdot \Big(\sum_{i\in[k]} \E[x_\tOne|h_\tOne=i] \cdot P(h_\tOne=i|h_\tTwo=j) \Big)
    \\
    =& \Pstat{\tTwo}{j} \Big(\sum_{i\in[k]} \mMeans_i \cdot (\mTrans^{\tTwo-\tOne})^\top_{ij} \Big)
    = \Pstat{\tTwo}{j} \big(\mMeans (\mTrans^{\tTwo-\tOne})^\top\big)_j
\end{split}
\end{equation}
Hence $\Tensor_\weight = \sum_{j \in [k]} \Pstat{\tTwo}{j} \big(\mMeans (\mTrans^{\tTwo-\tOne})^\top\big)_j \otimes \mMeans_j \otimes (\mMeans\mTrans^{\tThr-\tTwo})_j$, where the three components are all of Kruskal rank $k$ by Assumption \ref{assump:gmm_full_rank}.
Therefore we can recover columns of $\mMeans$ and $\mTrans^{\tThr-\tTwo}$ up to a shared column-wise permutation, and \textcolor{red}{hence also $\mTrans$}.

==> COLT2022/not_used/gmm_31_21_new.tex <==
Assuming for now that $\tOne < \tTwo < \tThr$.
Matching $x_\tTwo|x_\tOne$ and $x_\tThr|x_\tOne$ means:
\begin{equation}
\begin{split}
    \begin{cases}
        f^{\tTwo|\tOne}(x) = \mMeans\mTrans^{\tTwo-\tOne}\phi(x)
        = \tilde{f}_{\tTwo|\tOne}(x) = \tilde\mMeans\tilde\mTrans^{\tTwo-\tOne}\tilde\phi(x)
        \\
        f_{\tThr|\tOne}(x) = \mMeans\mTrans^{\tThr-\tOne}\phi(x)
        = \tilde{f}_{\tThr|\tOne}(x) = \tilde\mMeans\tilde\mTrans^{\tThr-\tOne}\tilde\phi(x)
    \end{cases}
\end{split}
\end{equation}
Choose a set $\gX := \{x^{(i)}\}_{i \in [k]}$ s.t. $\Phi_{\gX} := [\phi(x^{(1)}), ..., \phi(x^{(k)})]$ is of rank $k$.
Let $\tilde\Phi_{\gX}$ be defined similarly.
Then $\mMeans\mTrans^{\tTwo-\tOne}\Phi_{\gX} = \tilde\mMeans\tilde\mTrans^{\tTwo-\tOne}\tilde\Phi_{\gX}
\Rightarrow \mMeans^{\dagger}\tilde\mMeans = (\mTrans^{\tTwo-\tOne}\Phi_{\gX}) \cdot (\tilde\mTrans^{\tTwo-\tOne}\tilde\Phi_{\gX})^{-1}$,
\begin{equation*}
\begin{split}
    &\mMeans\mTrans^{\tThr-\tOne}\Phi_{\gX} = \tilde\mMeans\tilde\mTrans^{\tThr-\tOne}\tilde\Phi_{\gX}
    \\
    \Rightarrow&\ \tilde\mTrans^{\tThr-\tTwo} = \tilde\mMeans^{\dagger} \mMeans \cdot \mTrans^{\tThr-\tTwo} \cdot (\mTrans^{\tTwo-\tOne} \Phi_{\gX}) (\tilde{\mTrans}^{\tTwo-\tOne} \tilde\Phi_{\gX})^\dagger
            = \tilde\mMeans^{\dagger} \mMeans \cdot \mTrans^{\tThr-\tTwo} \cdot \mMeans^\dagger \tilde\mMeans.
    \\
\end{split}
\end{equation*}
% 
When \textcolor{Orange}{$\tThr-\tTwo = \tTwo - \tOne$},
\begin{equation}
\begin{split}
    &\tilde\mMeans \tilde\mTrans^{\tTwo-\tOne} \tilde\phi(x)
    = \tilde\mMeans \tilde\mTrans^{\tThr-\tTwo} \tilde\phi(x)
    = (\tilde\mMeans \tilde\mMeans^{\dagger}) \mMeans \cdot \mTrans^{\tThr-\tTwo} \cdot \mMeans^\dagger \tilde\mMeans \tilde\phi(x)
    \\
    \eqLabel{1}{=}& \mMeans \mTrans^{\tThr-\tTwo} \cdot \mMeans^\dagger \tilde\mMeans \tilde\phi(x)
        = \mMeans\mTrans^{\tThr-\tTwo} \cdot \phi(x), ~\forall x
    \\
    \Rightarrow&\ \mMeans^\dagger \tilde\mMeans \tilde\phi(x) = \phi(x), ~\forall x
    ~\eqLabel{2}\Rightarrow\ \tilde\mMeans\tilde\phi(x) = \mMeans\phi(x), ~\forall x
\end{split}
\end{equation}
where step $\rnum{1}$ uses $(\tilde\mMeans \tilde\mMeans)^\dagger \mMeans = \mMeans$, since $\tilde{\mMeans}, \mMeans$ share the same column space;
step $\rnum{2}$ uses $(\mMeans \mMeans)^\dagger \tilde\mMeans = \tilde\mMeans$, since $\tilde{\mMeans}, \mMeans$ share the same column space.

Denote $g(x) := \mMeans\phi(x)$, and $\tilde{g}(x) := \tilde\mMeans\tilde\phi(x)$.
Then we have $\forall x$, $g(x)=\tilde{g}(x)$, and $\nabla_{x} g(x) = \nabla_{x} \tilde{g}(x)$:
\begin{equation}
\begin{split}
    &\nabla_x g(x) = \mMeans \nabla_{x} \phi(x)
    = \mMeans \diag(\phi(x)) \mMeans^\top - (\mMeans \phi(x)) \cdot (\mMeans\phi(x))^\top
    \\
    =& \nabla_x \tilde{g}(x)
    = \tilde\mMeans \diag(\tilde\phi(x)) \tilde\mMeans^\top - (\tilde\mMeans \tilde\phi(x)) \cdot (\tilde\mMeans\tilde\phi(x))^\top 
    \\
    \eqLabel{1}{=}& \tilde\mMeans \diag(\tilde\phi(x)) \tilde\mMeans^\top - (\mMeans \phi(x)) \cdot (\mMeans\phi(x))^\top
    \\
    \Rightarrow& \mMeans\diag(\phi(x))\mMeans^\top = \tilde{\mMeans} \diag(\tilde{x}) \tilde\mMeans^\top 
\end{split}
\end{equation}
where step $\rnum{1}$ substitutes in $g(x) = \tilde{g}(x)$ for the second term.

Our goal is to show that $\mu_i = \tilde\mu_{\perm(i)}$ for some permutation $\perm$. Without loss of generality, let's fix \textcolor{Orange}{$\perm = \text{id}$}.
For $i \in [k]$, we claim that there exists $x^{(i)}$ s.t. \textcolor{Orange}{$\lim_{c \rightarrow \infty}\phi(x_c^{(i)}) \rightarrow \ve_i$}.
To construct such $x_c^{(i)}$, it suffices to find a direction $\vv^{(i)} \in \R^d$, $\|\vv^{(i)}\|_2 = 1$, such that $\vv^{(i)}(\mu_i - \mu_j) > 0$, $\forall j \neq i$;
such $\vv^{(i)}$ exists since $\{\mu_i\}_{i \in [k]}$ form a convex hull by the assumption that $\mMeans$ has linearly independent columns.
With such $\vv^{(i)}$, define $\hat{x}_c^{(i)} := \mu_i + c\vv^{(i)}$, then
\begin{equation}
\begin{split}
    \lim_{c\rightarrow \infty}[\phi(\hat{x}_c^{(i)})]_i =& \lim_{c\rightarrow \infty}\frac{\exp\big(-\frac{c^2\|\vv\|^2}{2}\big)}{\exp\big(-\frac{c^2\|\vv\|^2}{2}\big) + \sum_{j \neq i} \exp\big(-\frac{\|\mu_i - \mu_j + c\vv^{(i)}\|_2^2}{2}\big)}
    \\
    =& \lim_{c\rightarrow \infty}\left(1 + \sum_{j\neq i} \exp\Big(-\frac{\|\mu_i - \mu_j\|^2 + 2c\vv^{(i)}(\mu_i - \mu_j)}{2}\Big)\right)^{-1}
    = 1
\end{split}
\end{equation}
Hence \textcolor{Orange}{$\lim_{c \rightarrow \infty}\phi(\hat{x}_c^{(i)}) = \ve_i$}.
For such choices of $\hat{x}^{(i)}$, 
\begin{equation}
\begin{split}
    \mMeans\diag(\phi(\hat{x}^{(i)}))\mMeans^\top 
    = \mu_i \mu_i^\top 
    = \sum_{j \in [k]} [\tilde\phi(\hat{x}^{(i)})]_j \tilde\mu_j\tilde\mu_j^\top 
\end{split}
\end{equation}
The LHS is of rank 1, so the the RHS must also be of rank 1, i.e. $\tilde\phi(\hat{x}^{(i)}) = \ve_i$, and $\mu_i = \tilde\mu_i$.
Hence $\mMeans = \tilde\mMeans$, and $\phi = \tilde\phi$, and \textcolor{red}{consequently $\mTrans = \tilde\mTrans$}.
% \end{proof}


==> COLT2022/not_used/gmm_31_21_old.tex <==

\textcolor{RoyalBlue}{// Matching $x_2|x_1$ and $x_3|x_1$ gives identifiability}

    Matching $x_2|x_1$ and $x_3|x_1$ means:
    \begin{equation}
    \begin{split}
        \begin{cases}
            f^{2|1}(x) = \mMeans\mTrans\phi(x)
            = \tilde{f}_{2|1}(x) = \tilde\mMeans\tilde\mTrans\tilde\phi(x)
            \\
            f_{3|1}(x) = \mMeans\mTrans^{3-1}\phi(x)
            = \tilde{f}_{3|1}(x) = \tilde\mMeans\tilde\mTrans^2\tilde\phi(x)
        \end{cases}
    \end{split}
    \end{equation}
    Choose a set $\gX := \{x^{(i)}\}_{i \in [k]}$ s.t. $\Phi_{\gX} := [\phi(x^{(1)}), ..., \phi(x^{(k)})]$ is of rank $k$.
    Let $\tilde\Phi_{\gX}$ be defined similarly.
    Then
    \begin{equation}
    \begin{split}
        &\begin{cases}
            \mMeans\mTrans\Phi_{\gX} = \tilde\mMeans\tilde\mTrans\tilde\Phi_{\gX}
            &\Rightarrow \mMeans^{\dagger}\tilde\mMeans = (\mTrans\Phi_{\gX}) \cdot (\tilde\mTrans\tilde\Phi_{\gX})^\dagger
            \\
            \mMeans\mTrans^2\Phi_{\gX} = \tilde\mMeans\tilde\mTrans^2\tilde\Phi_{\gX}
            &\Rightarrow \tilde\mTrans = \tilde\mMeans^{\dagger} \mMeans \cdot \mTrans \cdot (\mTrans \Phi_{\gX}) (\tilde{\mTrans} \tilde\Phi_{\gX})^\dagger
                = \tilde\mMeans^{\dagger} \mMeans \cdot \mTrans \cdot \mMeans^\dagger \tilde\mMeans
        \end{cases}
        \\
        \Rightarrow&\ \tilde\mMeans \tilde\mTrans \tilde\phi(x)
            = (\tilde\mMeans \tilde\mMeans^{\dagger}) \mMeans \cdot \mTrans \cdot \mMeans^\dagger \tilde\mMeans \tilde\phi(x)
            \eqLabel{1}{=} \mMeans \mTrans \cdot \mMeans^\dagger \tilde\mMeans \tilde\phi(x)
            = \mMeans\mTrans\phi(x), ~\forall x
        \\
        \Rightarrow&\ \mMeans^\dagger \tilde\mMeans \tilde\phi(x) = \phi(x), ~\forall x
        ~\eqLabel{2}\Rightarrow\ \tilde\mMeans\tilde\phi(x) = \mMeans\phi(x), ~\forall x
    \end{split}
    \end{equation}
    where step $\rnum{1}$ uses $(\tilde\mMeans \tilde\mMeans)^\dagger \mMeans = \mMeans$, since $\tilde{\mMeans}, \mMeans$ share the same column space;
    step $\rnum{2}$ uses $(\mMeans \mMeans)^\dagger \tilde\mMeans = \tilde\mMeans$, since $\tilde{\mMeans}, \mMeans$ share the same column space.
    
    Denote $g(x) := \mMeans\phi(x)$, and $\tilde{g}(x) := \tilde\mMeans\tilde\phi(x)$.
    Then we have $\forall x$, $g(x)=\tilde{g}(x)$, and $\nabla_{x} g(x) = \nabla_{x} \tilde{g}(x)$:
    \begin{equation}
    \begin{split}
        &\nabla_x g(x) = \mMeans \nabla_{x} \phi(x)
        = \mMeans \diag(\phi(x)) \mMeans^\top - (\mMeans \phi(x)) \cdot (\mMeans\phi(x))^\top
        \\
        =& \nabla_x \tilde{g}(x)
        = \tilde\mMeans \diag(\tilde\phi(x)) \tilde\mMeans^\top - (\tilde\mMeans \tilde\phi(x)) \cdot (\tilde\mMeans\tilde\phi(x))^\top 
        \\
        \eqLabel{1}{=}& \tilde\mMeans \diag(\tilde\phi(x)) \tilde\mMeans^\top - (\mMeans \phi(x)) \cdot (\mMeans\phi(x))^\top
        \\
        \Rightarrow& \mMeans\diag(\phi(x))\mMeans^\top = \tilde{\mMeans} \diag(\tilde{x}) \tilde\mMeans^\top 
    \end{split}
    \end{equation}
    where step $\rnum{1}$ substitutes in $g(x) = \tilde{g}(x)$ for the second term.
    
    Our goal is to show that $\mu_i = \tilde\mu_{\perm(i)}$ for some permutation $\perm$. Without loss of generality, let's fix \textcolor{Orange}{$\perm = \text{id}$}.
    For $i \in [k]$, we claim that there exists $x^{(i)}$ s.t. \textcolor{Orange}{$\lim_{c \rightarrow \infty}\phi(x_c^{(i)}) \rightarrow \ve_i$}.
    To construct such $x_c^{(i)}$, it suffices to find a direction $\vv^{(i)} \in \R^d$, $\|\vv^{(i)}\|_2 = 1$, such that $\vv^{(i)}(\mu_i - \mu_j) > 0$, $\forall j \neq i$;
    such $\vv^{(i)}$ exists since $\{\mu_i\}_{i \in [k]}$ form a convex hull by the assumption that $\mMeans$ has linearly independent columns.
    With such $\vv^{(i)}$, define $\hat{x}_c^{(i)} := \mu_i + c\vv^{(i)}$, then
    \begin{equation}
    \begin{split}
        \lim_{c\rightarrow \infty}[\phi(\hat{x}_c^{(i)})]_i =& \lim_{c\rightarrow \infty}\frac{\exp\big(-\frac{c^2\|\vv\|^2}{2}\big)}{\exp\big(-\frac{c^2\|\vv\|^2}{2}\big) + \sum_{j \neq i} \exp\big(-\frac{\|\mu_i - \mu_j + c\vv^{(i)}\|_2^2}{2}\big)}
        \\
        =& \lim_{c\rightarrow \infty}\left(1 + \sum_{j\neq i} \exp\Big(-\frac{\|\mu_i - \mu_j\|^2 + 2c\vv^{(i)}(\mu_i - \mu_j)}{2}\Big)\right)^{-1}
        = 1
    \end{split}
    \end{equation}
    Hence \textcolor{Orange}{$\lim_{c \rightarrow \infty}\phi(\hat{x}_c^{(i)}) = \ve_i$}.
    For such choices of $\hat{x}^{(i)}$, 
    \begin{equation}
    \begin{split}
        \mMeans\diag(\phi(\hat{x}^{(i)}))\mMeans^\top 
        = \mu_i \mu_i^\top 
        = \sum_{j \in [k]} [\tilde\phi(\hat{x}^{(i)})]_j \tilde\mu_j\tilde\mu_j^\top 
    \end{split}
    \end{equation}
    The LHS is of rank 1, so the the RHS must also be of rank 1, i.e. $\tilde\phi(\hat{x}^{(i)}) = \ve_i$, and $\mu_i = \tilde\mu_i$.
    Hence $\mMeans = \tilde\mMeans$, and $\phi = \tilde\phi$, and consequently $\mTrans = \tilde\mTrans$.

==> COLT2022/not_used/gmm_3_given_1.tex <==

\textcolor{RoyalBlue}{// [draft] concrete examples for $x_3|x_1$}

We give two counterexamples showing $x_3|x_1$ fails to provide identifiability.
Both cases use a special orthogonal matrix $\mR$ that guarantees $\phi = \tilde\phi$, and both have a non-symmetric $\tilde\mTrans$.
% which means the counterexamples no longer hold when considering $x_1|x_3$.

\paragraph{Case I} $\mR$ satisfies $(\mMeans^{-1}\mR^{-1}\mMeans) \mTrans = \mTrans (\mMeans^{-1}\mR^{-1}\mMeans)$, i.e. the matrix product commutes.
We then have:
\begin{equation}
\begin{split}
    &\tilde\mMeans \tilde\mTrans \tilde\mTrans
    = \mR^2 \mMeans \cdot \mMeans^{-1}\mR^{-1}\mMeans\mTrans \cdot \mMeans^{-1}\mR^{-1}\mMeans\mTrans
    = \mR\mMeans \cdot \mTrans \cdot (\mMeans^{-1} \mR^{-1} \mMeans) \mTrans
    \\
    \eqLabel{1}=& \mR\mMeans \cdot (\mMeans^{-1} \mR^{-1} \mMeans) \mTrans \mTrans
    = \mMeans \mTrans \mTrans
\end{split}
\end{equation}
where $\rnum{1}$ uses the assumption that the choice of $\mR$ allows the matrix product to commute.

% AN EXAMPLE for x_3 | x_1
As a concrete example, consider $\theta = \frac{\pi}{10}$,
% , \theta_T = \frac{\pi}{11}$,
\begin{equation}
\begin{split}
    \mR =&
        \begin{bmatrix} \cos(\theta) & -\sin(\theta) & 0 \\ \sin(\theta) & \cos(\theta) & 0 \\ 0 & 0 & 1 \end{bmatrix},
    % \begin{bmatrix}0.9511 & -0.3090 & 0 \\ 0.3090 & 0.9511 & 0 \\ 0 & 0 & 1 \end{bmatrix},
    % \mR_T = \begin{bmatrix} \cos(\theta_T) & -\sin(\theta_T) & 0 \\ \sin(\theta_T) & \cos(\theta_T) & 0 \\ 0 & 0 & 1 \end{bmatrix},
        % \begin{bmatrix}0.9877 & -0.1564 & 0 \\ 0.1564 & 0.9877 & 0 \\ 0 & 0 & 1 \end{bmatrix},
        % \\
    \mMeans = \begin{bmatrix}1 & -1/2 & -1/2 \\ 0 & \sqrt{3}/2 & \sqrt{3}/2 \\ 1 & 1 & 1 \end{bmatrix},
    % \tilde\mMeans = \mR\mMeans,
    % \\
    \mTrans = \begin{bmatrix}0.8 & 0 & 0.2 \\ 0.2 & 0.8 & 0 \\ 0 & 0.2 & 0 0.8 \end{bmatrix},
    \\
    \tilde\mTrans =& (\mMeans^{-1} \mR^{-1} \mMeans) \cdot \mTrans
        = \mTrans \cdot (\mMeans^{-1} \mR^{-1} \mMeans)
        = \begin{bmatrix}0.8123 & 0.0583 & 0.1294 \\ 0.1294 & 0.8123 & 0.0583 \\ 0.0583 & 0.1294 & 0.8123 \end{bmatrix}.
\end{split}
\end{equation}

% ANOTHER EXAMPLE for x_3 | x_1
\paragraph{Case II} The matrix product does not commute in this case.
\begin{equation}
\begin{split}
    \mR =& \begin{bmatrix}0.9511 & -0.3090 & 0 \\ 0.3090 & 0.9511 & 0 \\ 0 & 0 & 1 \end{bmatrix},
    \mR_T = \begin{bmatrix}0.9212 & -0.3891 & 0 \\ -0.3891 & -0.9212 & 0 \\ 0 & 0 & 1 \end{bmatrix},
    \\
    \mMeans =& \begin{bmatrix}1 & -1/2 & -1/2 \\ 0 & \sqrt{3}/2 & \sqrt{3}/2 \\ 1 & 1 & 1 \end{bmatrix},
    \tilde\mMeans = \mR\mMeans,
    \\
    \mTrans =& \begin{bmatrix}0.8 & 0 & 0.8 \\ 0 & 0.8 & 0.2 \\ 0.8 & 0.2 & 0 \end{bmatrix},
    \tilde\mTrans = (\mMeans^{-1} \mR_T \mMeans) \cdot \mTrans 
        = \begin{bmatrix}0.8082 & 0.1611 & 0.0308 \\ 0.0308 & 0.8082 & 0.1611 \\ 0.1611 & 0.0308 & 0.8082\end{bmatrix}
\end{split}
\end{equation}
Here $\mR, \mR_T$ can also be written in terms of the sine or cosine of appropriate rotation angles as in the previous example.



==> COLT2022/not_used/gmm_pairwise_nonId_buggyPhi.tex <==
\subsubsection{Nonidentifiability proof - predicting with time $\{1,2,3\}$ \textcolor{red}{(bug)}}

Next, we construct a counterexample to show the nonidentifiability of predicting $x_2|x_1$ and $x_1|x_2$, for any $k \geq 3$.
The idea is to find a special orthogonal matrix $\mR\in \R^{d \times d}$ that is not a permutation,
    such that setting $\tilde\mMeans = \mR\mMeans$, $\tilde{\mTrans} = \mMeans^{-1}\mR^{-1}\mMeans \mTrans$ satisfies $\mMeans\mTrans = \tilde\mMeans\tilde\mTrans$.
We will make $\mTrans, \tilde\mTrans$ symmetric, such that $\mMeans\mTrans^\top = \tilde\mMeans\tilde\mTrans^\top$, hence such choices of $\tilde\mMeans, \tilde\mTrans$ form an optimal predictor for both directions, i.e. $x_2|x_1$ and $x_1|x_2$.

    We claim that choosing $\tilde\mMeans = \mR\mMeans$ means $\phi(x) = \tilde\phi(x)$, $\forall x \in \R^d$.
    This is because every special orthogonal matrix can be considered as a rigid-body rotation, hence such $\tilde\mMeans$ means \textcolor{red}{$\mu_i - \tilde{\mu}_i = \mu_j - \tilde{\mu}_j$} (\textcolor{red}{this is wrong: this requires a translation, i.e. $\tilde\mMeans = \mMeans + [v, v, ..., v]$ for some $v \in \R^d$}) and $\|\mu_i\|^2 = \|\tilde\mu_i\|^2$, $\forall i,j \in [k]$.
    % Then, since the softmax is invariant to scaling, i.e. $\frac{\exp(-\|x - \mu_i\|^2)}{\sum_{j\in[k]} {\exp(-\|x -\mu_j\|^2)}} = \frac{\exp(-\|x - \mu_i\|^2 + c)}{\sum_{j\in[k]} {\exp(-\|x -\mu_j\|^2 + c)}}$ for any $c \in \R$.
    Then, using the scale-invariance of softmax,
    % \begin{equation}
    % \begin{split}
    %     [\phi(x)]_i
    %     =& \frac{\exp(-\|x - \mu_i\|^2)}
    %         {\sum_{j\in[k]} \exp(-\|x -\mu_j\|^2)}
    %     = \frac{\exp(-\|x - \tilde\mu_i + \tilde\mu_i \mu_i\|^2 )}
    %         {\sum_{j\in[k]} \exp(-\|x - \tilde\mu_j + \tilde\mu_j \mu_j\|^2)}
    %     \\
    %     =& \frac{\exp\big(-\|x-\tilde\mu_i\|^2 + 2(\mu_i - \tilde\mu_i)^\top x + \|\tilde\mu_i\|^2 - \|\mu_i\|^2\big)}
    %         {\sum_{j\in [k]} \exp\big(-\|x-\tilde\mu_j\|^2 + 2(\mu_j - \tilde\mu_j)^\top x + \|\tilde\mu_j\|^2 - \|\mu_j\|^2\big)}
    %     \\
    %     =& \frac{\exp(-\|x-\tilde\mu_i\|^2 + 2(\mu_i - \tilde\mu_i)^\top x)}
    %         {\sum_{j\in [k]} \exp(-\|x-\tilde\mu_j\|^2 + 2(\mu_i - \tilde\mu_i)^\top x)} 
    %     = \frac{\exp(-\|x-\tilde\mu_i\|^2)}
    %         {\sum_{j\in [k]} \exp(-\|x-\tilde\mu_j\|^2)}
    %     = [\tilde{\phi}(x)]_i.
    % \end{split}
    % \end{equation}
    % 
    \begin{equation}
    \begin{split}
        &[\phi(x)]_i
        = \frac{\exp\big(-\frac{\|x - \mu_i\|^2}{2}\big)}
            {\sum_{j\in[k]} \exp\big(-\frac{\|x -\mu_j\|^2}{2}\big)}
        = \frac{\exp\big(-\frac{\|x - \mu_i\|^2 - \|\mu_i\|^2 + \|\tilde\mu_i\|^2}{2}\big)}
            {\sum_{j\in[k]} \exp\big(-\frac{\|x - \mu_j\|^2 - \|\mu_j\|^2 + \|\tilde\mu_j\|^2}{2}\big)}
        \\
        =& \frac{\exp\big(-\frac{\|x\|^2 - 2\mu_i^\top x + \|\tilde\mu_i\|^2}{2}\big)}
            {\sum_{j\in[k]} \exp\big(-\frac{\|x\|^2 - 2\mu_j^\top x + \|\tilde\mu_j\|^2}{2}\big)}
        = \frac{\exp\big(-\frac{\|x\|^2 - 2\tilde\mu_i^\top x + 2(\tilde\mu_i - \mu_i)^\top x + \|\tilde\mu_i\|^2}{2}\big)}
            {\sum_{j\in[k]} \exp\big(-\frac{\|x\|^2 - 2\tilde\mu_j^\top x + 2(\tilde\mu_j - \mu_j)^\top x + \|\tilde\mu_j\|^2}{2}\big)} 
        \\
        =& \frac{\exp\big(-\frac{\|x\|^2 - 2\tilde\mu_i^\top x + \|\tilde\mu_i\|^2}{2}\big)}
            {\sum_{j\in[k]} \exp\big(-\frac{\|x\|^2 - 2\tilde\mu_j^\top x + \|\tilde\mu_j\|^2}{2}\big)}  
        = [\tilde\phi(x)]_i.
    \end{split}
    \end{equation}


    Therefore we have $\mMeans\mTrans = \tilde\mMeans\tilde\mTrans$ and $\phi(x) = \tilde\phi(x),~\forall x \in \R^d$, hence $\mMeans\mTrans\phi = \tilde{\mMeans}\tilde\mTrans\tilde{\phi}$ and the proof is complete.
    Note that to construct such a counterexample by rotation, we need to make sure $\mTrans$ is still a valid stochastic matrix after the rotation, that is, $\tilde\mTrans$ should have non-negative entries and columns summing up to 1.
    This is achievable, for instance, by controlling the rotation angle represented by $\mR$ to be sufficiently small.
    
    The following is a concrete counterexample for $d = k = 3$.
    The idea is to let $\mu_1, \mu_2, \mu_3$ form a right triangle in a plane. Matching $\mMeans\mTrans$ means matching the convex combinations of the means, which lie within this right triangle (i.e. a convex hull).
    Denote these convex combinations as $v_1, v_2, v_3$, i.e. $[v_1, v_2, v_3] = \mMeans\mTrans$.
    Then, if the rigid rotation $\mR$ is sufficiently small (as determined by the conditioning of $\mTrans$), then $v_1, v_2, v_3$ still lie within the triangle formed by the rotated means $\tilde\mu_1, \tilde\mu_2, \tilde\mu_3$, which means there exists a stochastic matrix $\tilde\mTrans$ such that $\tilde\mMeans \tilde\mTrans = [v_1, v_2, v_3] = \mMeans\mTrans$.
    \textcolor{Orange}{(add figure to illustrate?)}
    % (as shown in Figure \ref{fig:predictNext_wellSepc_2to1}),
    Let $a = \frac{7}{8}$; one choice of such parameters could be:
    \begin{equation}
    \begin{split}
        \mTrans =& \begin{bmatrix}
            a & 0 & 1-a \\
            0 & 1-a & a \\
            1-a & a & 0 \\
        \end{bmatrix},
        ~\mM = \begin{bmatrix}
            1 & -1/2 & -1/2 \\
            0 & \sqrt{3}/2 & -\sqrt{3}/2 \\
            1 & 1 & 1
        \end{bmatrix},
        \\
        \tilde\mTrans =& \begin{bmatrix}
            a & 1-a & 0 \\
            1-a & 0 & a \\
            0 & a & 1-a \\
        \end{bmatrix},
        % \det(\tilde{\mTrans}) = -a^3 -(1-a)^3
        ~\tilde\mM = \mMeans\mTrans\tilde\mTrans^{-1}.
        \\
    \end{split}
    \end{equation}
    Here the rotation matrix is implicitly $\mR = \tilde\mMeans\mMeans^{-1} = \mMeans\mTrans\tilde\mTrans^{-1} \mMeans^{-1}$.
    % We now have $\mMeans \mTrans = \tilde\mMeans \tilde\mTrans = \mMeans\mTrans^\top = \tilde\mMeans \tilde\mTrans^\top$,
    % but $\min_{\alpha}\frac{\|\mu_i - \tilde\mu_{\alpha(i)}\|_2}{\|\mu_i\|_2} > 0.2$, $\forall i \in [k]$.

\paragraph{Extending to higher dimensions} This counterexample by rotation can be easily extended to larger values of $d,k$.
To extend to larger $d$, one can easily embed the 3-dimensional vector to a higher dimension, for instance, by padding the extra coordinates with 0.
To extend to larger $k$, note that as long as $k\geq 3$, we can find a 3-dimensional subspace in $\R^d$, in which the above counterexample applies.

\paragraph{Special case of $k=2$} 
The intuition of the previous counterexample is that matching $\mMeans\mTrans\phi(x) = \tilde\mMeans\tilde\mTrans\tilde\phi(x)$ means matching one particular convex combination of $\{\mu_i\}_{i\in[k]}$ and $\{\tilde\mu_i\}_{i\in[k]}$.
All such combinations lie in the polytope defined with vertices being columns of $\mMeans\mTrans$ (and respectively $\tilde\mMeans\tilde\mTrans$), which specify a $(k-1)$-dimensional subspace.
For $k \geq 3$, this subspace is at least 2-dimensional, which allows for rotation as a counterexample.
However, when $k=2$, matching 2 convex combinations means $\{\mu_1, \mu_2\}, \{\tilde\mu_1, \tilde\mu_2\}$ have to reside in the same 1-dimensional subspace (i.e. co-linear), hence such rotation argument can no longer apply.
In fact, a single pairwise prediction task suffices for identifiability when $k=2$:
\vspace{-1em}
\begin{lemma}[Identifiability of pairwise prediction task for $k=2$]
\label{lem:gmm_21_12_k2}
    When $k=2$, assume Assumption \ref{assump:latent}, \ref{assump:gmm_full_rank} hold,
    and further \textcolor{Orange}{assume that $\|\mu_i\|_2 = c$ for some known $c > 0$}.
    If the predictor has \emph{\textcolor{Orange}{the correct parametric form}},
    then parameters $\tilde\mMeans, \tilde\mTrans$ of the the optimal predictors for $x_2|x_1$ are the same as the ground truth $\mMeans, \mTrans$ up to permutation.
\end{lemma}
%
\begin{proof}
    Pick $x_1, x_2$ such that $\Phi := [\phi(x_1), \phi(x_2)] \in \R^{2\times 2}$ is of full rank.
    Similarly, denote $\tilde\Phi := [\tilde\phi(x_1), \tilde\phi(x_2)]$;
    $\tilde\Phi$ is also of full rank since $\mMeans\mTrans\Phi = \tilde\mMeans\tilde\mTrans\tilde\Phi$.
    $\Phi, \tilde\Phi$ are both stochastic matrices since their columns are probability vectors, and the products $\mA := \mTrans\Phi, \tilde\mA := \tilde\mTrans\tilde\Phi$ are also stochastic matrices.
    % 
    We now have $\mMeans \mA = \tilde\mMeans \tilde\mA$, which means the convex combinations of $\mu_1, \mu_2$ and $\tilde\mu_1, \tilde\mu_2$ match.
    Write $\tilde\mu_1 = \mu_1 + \alpha(\mu_2 - \mu_1)$ for some $\alpha \in \R$.
    By assuming known norms, we have:
    \begin{equation}
    \begin{split}
        R^2 = \|\tilde{\mu}_1\|^2
        = ((1-\alpha)^2 + \alpha^2) R^2 + 2\alpha(1-\alpha)\mu_1^\top \mu_2
        \eqLabel{1}{\leq} \big[(1-\alpha)^2 + \alpha^2 + 2\alpha(1-\alpha)\big] R^2
        = R^2
    \end{split}
    \end{equation}
    where step $\rnum{1}$ holds with equality if 1) $\mu_1 = \mu_2$, or 2) $\alpha \in \{0, 1\}$.
    The former is impossible since $\mMeans$ is of full-rank by Assumption \ref{assump:gmm_full_rank}, hence the latter must hold, i.e. $\tilde\mu_1= \mu_1$ or $\tilde\mu_1 = \mu_2$, i.e. $\mMeans$ is determined up to permutation.
\end{proof}


\subsubsection{Nonidentifiability proof - $x_{t+1}|x_1$ and $x_1|x_{t+1}$ \textcolor{red}{(bug)}}

Let's consider the case where \textcolor{peach}{$d = k$}.
The counterexample consists of an orthogonal $\mMeans$, a special orthogonal matrix $\mR$ such that $(\mMeans^{-1}\mR^{-1}\mMeans) \mTrans = \mTrans (\mMeans^{-1}\mR^{-1}\mMeans)$, i.e. \textcolor{peach}{the matrix product commutes}.
and learned parameters $\tilde\mMeans = \mR^t$, $\tilde\mTrans = (\mMeans^{-1}\mR^{-1}\mMeans) \mTrans = \mTrans (\mMeans^{-1}\mR^{-1}\mMeans)$.
A concrete counterexample could be the one used in the proof of Lemma \ref{lem:transPower_nonId}.

We next show why such choices of parameters implies non-identifiability.
As explained before, \textcolor{red}{$\mR$ being special orthogonal implies $\phi = \tilde\phi$ (bug)}.
Predicting $x_{t+1}$ given $x_1$ gives $\mMeans \mTrans^t \phi = \tilde\mMeans \tilde\mTrans^t \tilde\phi$, which is now reduced to $\mMeans\mTrans^t = \tilde\mMeans\tilde\mTrans^t$ by canceling out $\phi, \tilde\phi$.
For any $s \in \{0, 1, ..., n-1\}$,
\begin{equation}
\begin{split}
    &\mR^{t-s} \mMeans \mTrans^{s} \tilde\mTrans^{t-s}
    = \mR^{t-s} \mMeans \mTrans^{s} \cdot (\mMeans^{-1} \mR^{-1} \mMeans) \mTrans \cdot \tilde\mTrans^{t-s-1}
    \\
    =& \mR^{t-s} \mMeans \mTrans^{s-1} \cdot \mTrans(\mMeans^{-1} \mR^{-1} \mMeans) \cdot \mTrans \cdot \tilde\mTrans^{t-s-1}
    \\
    \eqLabel{1}{=}& \mR^{t-s} \mMeans \mTrans^{s-1} \cdot (\mMeans^{-1} \mR^{-1} \mMeans) \cdot \mTrans^2 \cdot \tilde\mTrans^{t-s-1}
    \\
    \eqLabel{2}{=}& \mR^{t-s} \mMeans (\mMeans^{-1} \mR^{-1} \mMeans) \cdot \mTrans^{s+1} \cdot \tilde\mTrans^{t-s-1}
    \\
    =& \mR^{t-(s+1)} \mMeans \mTrans^{s+1} \cdot \tilde\mTrans^{t-(s+1)}
\end{split}
\end{equation}
where step $\rnum{1}, \rnum{2}$ use the commutative assumption.

Applying the above equality for $s = 0, 1, ..., t-1$, we get 
\begin{equation}\label{eq:gmm_single_oneway}
\begin{split}
    \tilde\mMeans\tilde\mTrans^{t}
    = \mR^t \mM \tilde\mTrans^{t}
    = \mMeans \mTrans^t
    \Rightarrow \E[x_{t+1}|x_{1}; \mMeans, \mTrans] = \E[x_{t+1}|x_{1}; \tilde\mMeans, \tilde\mTrans],~ \forall x_1 \in \R^d.
\end{split}
\end{equation}
%
For the reverse direction of $x_{1}|x_{t+1}$, note that $\mMeans^\dagger = \mMeans^\top$, hence for any $s \in \{0, 1, ..., t-1\}$, we similarly have 
\begin{equation}
\begin{split}
    &\mR^{t-s} \mMeans (\mTrans^\top)^{s} (\tilde\mTrans^\top)^{t-s}
    = \mR^{t-s} \mMeans (\mTrans^\top)^{s} \big((\mTrans \mMeans^{-1} \mR^{-1}\mMeans)^\top\big)^{t-s}
    \\
    =& \mR^{t-s} \mMeans (\mTrans^\top)^{s-1} \mTrans^{\top} (\mMeans^{-1} \mR^{-1}\mMeans)^\top \mTrans^\top \big((\mTrans \mMeans^{-1} \mR^{-1}\mMeans)^\top\big)^{t-s-1}
    \\
    \eqLabel{1}=& \mR^{t-s} \mMeans (\mTrans^\top)^{s-1} (\mMeans^{-1} \mR^{-1}\mMeans)^\top \mTrans^{\top} \mTrans^\top \big((\mTrans \mMeans^{-1} \mR^{-1}\mMeans)^\top\big)^{t-s-1}
    \\
    \eqLabel{2}=& \mR^{t-s} \mMeans (\mMeans^{-1} \mR^{-1}\mMeans)^\top (\mTrans^{\top})^{s+1} \big((\mTrans \mMeans^{-1} \mR^{-1}\mMeans)^\top\big)^{t-s-1}
    \\
    \eqLabel{3}=& \mR^{t-s} \mMeans \mMeans^\top \mR \mMeans (\mTrans^{\top})^{s+1} \big((\mTrans \mMeans^{-1} \mR^{-1}\mMeans)^\top\big)^{t-s-1}
    \\
    \eqLabel{4}=& \mR^{t-(s+1)} \mMeans (\mTrans^{\top})^{s+1} \big((\mTrans \mMeans^{-1} \mR^{-1}\mMeans)^\top\big)^{t-(s+1)}
\end{split}
\end{equation}
where step $\rnum{1}, \rnum{2}$ use the commutative assumption,
and step $\rnum{3}, \rnum{4}$ are because $\mMeans$ is orthogonal.
Hence $\mMeans(\mTrans^\top)^t = \tilde\mMeans(\tilde\mTrans^\top)^\top$, i.e. $\tilde\mMeans, \tilde\mTrans$ also form an optimal predictor for $x_{1}|x_{t+1}$.



==> COLT2022/not_used/gmm_previous_statements.tex <==
First note that the identifiability results for the discrete HMM apply to \GHMM\ as well:
\vspace{-0.8em}
\begin{theorem}[Identifiability of masked prediction task on three tokens, \GHMM]
\label{thm:gmm}
    % Let $t_1, t_2,t_3$ be distinct time steps.
    Let $(t_1, t_2, t_3)$ be any permutation of $(1,2,3)$.
    Under Assumption \ref{assump:latent}, \ref{assump:gmm_full_rank},
    if the predictor has \emph{\textcolor{Orange}{the correct parametric form}},
    then parameters $\tilde\mMeans, \tilde\mTrans$ of the the optimal predictors for the following tasks are the same as the ground truth $\mMeans, \mTrans$ up to permutation:
    \textcolor{red}{(todo: fix proof)}
    \vspace{-0.8em}
    \begin{enumerate}
        \item the task of predicting $x_{t_2} \otimes x_{t_3}$ given $x_{t_1}$;
        \item the task of predicting $x_{t_3}$ given $x_{t_1} \otimes x_{t_2}$.
    \end{enumerate}
\end{theorem}
The proof \textcolor{peach}{follows the exact structure} of that of the discrete case, that is, by constructing a proper 3-tensor on which Kruskal's theorem applies.
The key observation is that the conditional mean of $x_t$ given $h_t$ is $\mMeans_{h_t}$, which takes the same form as the discrete case (i.e. $\mEmiss_{h_1}$).

However, in contrast to discrete HMM, pairwise prediction tasks do not necessarily lead to non-identifiability.
Rather, identifiability will depend on the specific task configuration.
We show that:
\vspace{-1em}
\begin{theorem}[Pairwise prediction tasks for \GHMM]
\label{thm:gmm_pair}
Under Assumption \ref{assump:latent}, \ref{assump:gmm_full_rank},
    if the predictor has \emph{\textcolor{Orange}{the correct parametric form}},
then the parameters $\tilde\mMeans, \tilde\mTrans$:
\vspace{-1em}
\begin{itemize}[leftmargin=*]
    \item can recover the ground truth parameters up to permutation, by predicting $x_{2}$ given $x_1$ and predicting $x_3$ given $x_1$, $\forall k \geq 2$;\textcolor{Orange}{double check the proof}
    \item fails to recover the ground truth parameters, by predicting $x_1|x_2$, $x_2|x_1$, $x_3|x_2$ and $x_2|x_3$, $\forall k \geq 3$;
    \item fails to recover the ground truth parameters, by predicting $x_{t+1}|x_1$ and $x_1|x_{t+1}$, $\forall t$.
\end{itemize}
\end{theorem}

However, while the pairwise prediction tasks fail to provide identifiability, matching the pairwise conditional \textit{distribution} does suffice to uniquely determine the parameters:
%  the discrete HMM is that matching the pairwise conditional distribution suffices for identifiability of \GHMM.
\vspace{-1em}
\begin{theorem}[Identifiability of conditional distribution]
\label{thm:gmm_conditional}
    % If $p(x_2|x_1; \mMeans,\mTrans) = p(x_2|x_1; \tilde\mMeans,\tilde{\mTrans})$, $\forall x_1,x_2 \in \R^d$,
    If $p(x_{t_2}|x_{t_1}; \mMeans,\mTrans) = p(x_{t_2}|x_{t_1}; \tilde\mMeans,\tilde{\mTrans})$, $\forall x_{t_1},x_{t_2} \in \R^d$,
    then $\mMeans = \tilde\mMeans$, $\mTrans = \tilde\mTrans$ up to a permutation on the labeling. 
\end{theorem}
\vspace{-1em}
Contrasting Theorem \ref{thm:gmm_pair} and \ref{thm:gmm_conditional} highlights that unlike discrete HMMs, the non-identifiability of pairwise prediction task in \GHMM~is not because there is not enough information in pairs, but that masked prediction only utilizes the conditional \textit{expectation}, which is too weak a task.
Moreover, while there likely exist self-supervised tasks whose objectives correspond to matching the conditional distribution, our goal is not to propose specific algorithms, and thus Theorem \ref{thm:gmm_conditional} should be treated only as a characterization for identifiability.

% Moreover, learning a pair of single-token prediction task suffice for parameter recovery for Gaussian mixture HMM:
% \vspace{-1em}
% \begin{theorem}[Identifiability from predicting $x_{t_2}|x_{t_1}$ and $x_{t_3}|x_{t_1}$]
% \label{thm:gmm_pair_single}
%     % If $\E_{\mMeans,\mTrans}[x_2|x_1] = \E_{\tilde\mMeans,\tilde\mTrans}[x_2|x_1]$ and $\E_{\mMeans,\mTrans}[x_3|x_1] = \E_{\tilde\mMeans,\tilde\mTrans}[x_3|x_1]$ for any $x_1, x_2, x_3 \in \R^d$,
%     Let $\tOne, \tTwo, \tThr$ be time steps such that \textcolor{Orange}{$\tThr-\tTwo = \tTwo - \tOne$}.
%     If $\E_{\mMeans,\mTrans}[x_{\tTwo}|x_{\tOne}] = \E_{\tilde\mMeans,\tilde\mTrans}[x_{\tTwo}|x_{\tOne}]$ and $\E_{\mMeans,\mTrans}[x_{\tThr}|x_{\tOne}] = \E_{\tilde\mMeans,\tilde\mTrans}[x_{\tThr}|x_{\tOne}]$ for any $x_{\tOne}, x_{\tTwo}, x_{\tThr} \in \R^d$,
%     then $\mMeans = \tilde\mMeans$, $\mTrans = \tilde\mTrans$ up to a shared column-wise permutation.
% \end{theorem}

% However, although there is enough information in the pairwise conditional \textit{distribution}, the masked prediction tasks only utilize the pairwise conditional \textit{expectation}, which is too weak for parameter recovery.
% In particular, we show that the next-token prediction task fails to provide identifiability:
% \vspace{-1em}
% \begin{lemma}[Nonidentifiability of predicting $x_{t+1}|x_1$ and $x_1|x_{t+1}$, for \textcolor{Orange}{odd $t$}]
% \label{lem:gmm_nonid_t1_1t}
%     Under Assumption \ref{assump:latent}, \ref{assump:gmm_full_rank},
%     there exist $\tilde\mMeans, \tilde\mTrans$,
%     such that $\E_{\mMeans,\mTrans}[x_2|x_1] = \E_{\tilde\mMeans,\tilde{\mTrans}}[x_2|x_1]$, $\forall x_1 \in \R^d$,
%     but for any permutation $\alpha$, $\frac{\|\mu_i - \tilde\mu_{\alpha(i)}\|_2}{\|\mu_i\|_2} > c(\mTrans)$, $\forall i \in [k]$. 
% \end{lemma}
% \textit{Note}: we can also show that for any $t$, matching $x_{t+1}|x_1$ is not sufficient for identifiability; but we currently do not have the result for matching both $x_{t+1}|x_1$ and $x_1|x_{t+1}$ for $t$ being even.

% \vspace{-1em}
% \begin{lemma}[Nonidentifiability of predicting $x_2|x_1$]
% \label{lem:gmm_nonid}
% Under Assumption \ref{assump:discrete_uniform_latent}, \ref{assump:gmm_full_rank},
% there exist $\tilde\mMeans, \tilde\mTrans$,
% such that $\E_{\mMeans,\mTrans}[x_2|x_1] = \E_{\tilde\mMeans,\tilde{\mTrans}}[x_2|x_1]$, $\forall x_1 \in \R^d$,
% but for any permutation $\alpha$, $\frac{\|\mu_i - \tilde\mu_{\alpha(i)}\|_2}{\|\mu_i\|_2} > c(\mTrans)$, $\forall i \in [k]$.
% \end{lemma}

% The nonidentifiability is not a result of being unidirectional.
% In fact, using both $x_2|x_1$ \textit{and} $x_1|x_2$ still does not give identifiability:
% \vspace{-1em}
% \begin{lemma}[Nonidentifiability of both predicting $x_2|x_1$ and $x_1|x_2$]
% \label{cor:gmm_12_21}
% \textcolor{Orange}{(todo: update labeling)}
%     Under Assumption \ref{assump:discrete_uniform_latent}, \ref{assump:gmm_full_rank},
%     there exist $\tilde\mMeans, \tilde\mTrans$,
%     such that $\E_{\mMeans,\mTrans}[x_2|x_1] = \E_{\tilde\mMeans,\tilde{\mTrans}}[x_2|x_1]$ and $\E_{\mMeans,\mTrans}[x_1|x_2] = \E_{\tilde\mMeans,\tilde{\mTrans}}[x_1|x_2]$, $\forall x_1, x_2 \in \R^d$,
%     but for any permutation $\perm$, $\frac{\|\mu_i - \tilde\mu_{\perm(i)}\|_2}{\|\mu_i\|_2} = \Omega(1)$, $\forall i \in [k]$.
% \end{lemma}

% One may wonder whether predicting two-steps ahead, i.e. $x_3|x_1$, would suffice, and the answer is negative:
% \vspace{-1em}
% \begin{lemma}[Nonidentifiability of predicting $x_3|x_1$]
% \label{lem:gmm_nonid_31}
%     Under Assumption \ref{assump:discrete_uniform_latent}, \ref{assump:gmm_full_rank},
%     there exist $\tilde\mMeans, \tilde\mTrans$,
%     such that $\E_{\mMeans,\mTrans}[x_3|x_1] = \E_{\tilde\mMeans,\tilde{\mTrans}}[x_3|x_1]$, $\forall x_1 \in \R^d$,
%     but for any permutation $\pi$, $\frac{\|\mu_i - \tilde\mu_{\pi(i)}\|_2}{\|\mu_i\|_2} = \Theta(1)$, $\forall i \in [k]$.
%     \end{lemma}
% \textcolor{Orange}{todo: merge into 1 general theorem}

% A corollary is that we also have identifiability from pairwise marginals:
% \textcolor{Orange}{(do we want this result?)}
% \vspace{-1em}
% \begin{lemma}
% \label{lem:gmm_marginal}
% If $p(x_1, x_2; \mMeans,\mTrans) = p(x_1, x_2; \tilde\mMeans, \tilde{\mTrans})$, $\forall x_1, x_2 \in \R^d$,
% then $\mMeans = \tilde\mMeans$, $\mTrans = \tilde\mTrans$ up to a permutation on the labeling.
% \end{lemma}



==> COLT2022/not_used/gmm_t1_generic_wrong.tex <==
\subsection{Proof for Lemma \ref{lem:gmm_nonid_t1_1t} (nonidentifiability of predicting \textcolor{peach}{$x_{t+1}|x_{1}$})}

For any \textcolor{Orange}{odd number $t$}, let $\tilde\mMeans = \mR^t \mMeans$ and $\tilde\mTrans = (\mMeans^{-1}\mR^{-1}\mMeans)\mTrans$,
where $\mR$ is a \textcolor{Orange}{special orthogonal}.
To construct a counterexample, it suffices to find an example where
(1) $\mTrans$ is symmetric,
(2) $\mMeans = c\mU$ for some constant $c$ and matrix $\mU \in \R^{d \times k}$ with orthogonal columns (note that $\mMeans^\dagger = \frac{1}{c}\mU^\top = \frac{1}{c^2}\mMeans^\top$),
and (3) $\mR$ satisfies
\vspace{-1em}
\begin{enumerate}[label=(\alph*)]
    \item $(\mMeans^{-1}\mR^{-1}\mMeans)\mTrans = \mTrans (\mMeans^{-1}\mR^{-1}\mMeans)$, i.e. the matrix product commutes,
    \item $\mR$ is symmetric,
    \item $\tilde\mTrans$ is a valid transition matrix,
\end{enumerate}
\vspace{-1em}
% then $\E[x_{t+1}|x_1; \mMeans, \mTrans] = \E[x_{t+1}|x_1; \tilde\mMeans, \tilde\mTrans]$,
% $\E[x_1|x_{t+1}; \mMeans, \mTrans] = \E[x_1|x_{t+1}; \tilde\mMeans, \tilde\mTrans]$, $\forall x_1 \in \R^d$.

Suppose such $\mTrans, \mR$ exist.
Since $\mR$ is orthogonal, we have $\phi = \tilde\phi$.
\textcolor{draftGray}{(todo: add or refer to explanations)}
Predicting $x_{t+1}$ given $x_1$ gives $\mMeans \mTrans^t \phi = \tilde\mMeans \tilde\mTrans^t \tilde\phi$, which is now reduced to $\mMeans\mTrans^t = \tilde\mMeans\tilde\mTrans^t$ by canceling out $\phi, \tilde\phi$.
For any $s \in \{0, 1, ..., n-1\}$,
\begin{equation}
\begin{split}
    &\mR^{t-s} \mMeans \mTrans^{s} \tilde\mTrans^{t-s}
    = \mR^{t-s} \mMeans \mTrans^{s} \cdot (\mMeans^{-1} \mR^{-1} \mMeans) \mTrans \cdot \tilde\mTrans^{t-s-1}
    \\
    =& \mR^{t-s} \mMeans \mTrans^{s-1} \cdot \mTrans(\mMeans^{-1} \mR^{-1} \mMeans) \cdot \mTrans \cdot \tilde\mTrans^{t-s-1}
    \\
    \eqLabel{1}{=}& \mR^{t-s} \mMeans \mTrans^{s-1} \cdot (\mMeans^{-1} \mR^{-1} \mMeans) \cdot \mTrans^2 \cdot \tilde\mTrans^{t-s-1}
    \\
    \eqLabel{2}{=}& \mR^{t-s} \mMeans (\mMeans^{-1} \mR^{-1} \mMeans) \cdot \mTrans^{s+1} \cdot \tilde\mTrans^{t-s-1}
    \\
    =& \mR^{t-(s+1)} \mMeans \mTrans^{s+1} \cdot \tilde\mTrans^{t-(s+1)}
\end{split}
\end{equation}
Applying the above equality for $s = 0, 1, ..., n-1$, we get 
\begin{equation}\label{eq:gmm_single_oneway}
\begin{split}
    \tilde\mMeans\tilde\mTrans^{t}
    = \mR^t \mM \tilde\mTrans^{t}
    = \mMeans \mTrans^t
    \Rightarrow \E[x_{t+1}|x_{1}; \mMeans, \mTrans] = \E[x_{t+1}|x_{1}; \tilde\mMeans, \tilde\mTrans],~ \forall x_1 \in \R^d.
\end{split}
\end{equation}

Note that the product $\mMeans^\dagger \mR^{-1} \mMeans$ is symmetric:
\begin{equation}
\begin{split}
    (\mMeans^\dagger \mR^{-1} \mMeans)^\top 
    = \mMeans^\top \mR (\mMeans^\dagger)^\top
    \eqLabel{1}{=} c^2\mMeans^\dagger \mR \frac{1}{c^2}\mMeans
    \eqLabel{2}{=} \mMeans^\dagger \mR^{-1} \mMeans
\end{split}
\end{equation}
where step $\rnum{1}$ uses $\mMeans = c\mU$, and step $\rnum{2}$ uses $\mR$ is symmetric.

Since $\mTrans, (\mMeans^\dagger \mR^{-1} \mMeans)$ are both symmetric and their product commutes, 
$\tilde\mTrans := (\mMeans^\dagger \mR^{-1} \mMeans)\mTrans$ is also symmetric.
Hence $\tilde\mMeans(\tilde\mTrans^\top)^{t} = \mMeans (\mTrans^\top)^t$, that is, $\E[x_1|x_{t+1}; \mMeans, \mTrans] = \E[x_1|x_{t+1}; \tilde\mMeans, \tilde\mTrans]$, $\forall x_{t+1} \in \R^d$.

As a concrete example, let $\hat\mR \in \R^{3 \times 3}$ be any special orthogonal matrix, then the conditions can be satisfied by the following choice of $\mMeans, \mTrans$, and $\mR$:
\textcolor{draftGray}{(\textcolor{red}{NOTE: invalid since $\mR$ is not special orthogonal};
recall that $\phi = \tilde\phi$ requires $\mu_i - \tilde\mu_i = \mu_j - \tilde\mu_j$ and $\|\mu_i\|^2 - \|\tilde\mu_i\|^2 = \|\mu_j\|^2 - \|\tilde\mu_j\|^2$).}
\begin{equation}
\begin{split}
    &\mMeans = \hat\mR \begin{bmatrix}
        1 & -1/2 & -1/2 \\
        0 & -\sqrt{3}/2 & \sqrt{3}/2 \\
        1/\sqrt{2} & 1/\sqrt{2} & 1/\sqrt{2} \\
    \end{bmatrix},~
    \mR = \hat\mR \begin{bmatrix}
        -1 & 0 & 0 \\
        0 & 1 & 0 \\
        0 & 0 & 1
    \end{bmatrix},
    \\
    &\mTrans = \begin{bmatrix}
        2/3 & 1/6 & 1/6 \\
        1/6 & 2/3 & 1/6 \\
        1/6 & 1/6 & 2/3 \\
    \end{bmatrix},~
    \tilde\mTrans = \begin{bmatrix}
        0 & 1/2 & 1/2 \\
        1/2 & 1/2 & 0 \\
        1/2 & 0 & 1/2
    \end{bmatrix}.
\end{split}
\end{equation}

\textit{Note}: if we only match $x_{t+1}|x_1$ (or $x_1|x_{t+1}$, but not both), then we do not need $\mR$ to be symmetric, and we get non-identifiability for any $t$ as shown in equation \ref{eq:gmm_single_oneway}.

\textcolor{Orange}{todo: can we show that if $t$ is even, then learning both $x_{t+1}|x_1$ and $x_1|x_{t+1}$ gives identifiability?}

\textcolor{RoyalBlue}{// discrete HMM}

$[\phi(x)]_i = \frac{\mEmiss_{xi}}{\|\mEmiss_{x:}\|_1}$,  $\phi = \tilde\phi$ allows for rescaling of rows in the emission matrix; e.g. 
\begin{equation}
\begin{split}
    \mEmiss = \begin{bmatrix}
        6/8 & 1/8 \\ 1/8 & 6/8 \\ 1/8 & 1/8
    \end{bmatrix},~
    \tilde\mEmiss = \begin{bmatrix}
        6/16 & 1/16 \\ 1/16 & 6/16 \\ 9/16 & 9/16
    \end{bmatrix}
    = \Big[\frac{1}{2}\ve_1, \frac{1}{2}\ve_2, \frac{9}{2}\ve_3\Big] \mEmiss.
\end{split}
\end{equation}

==> COLT2022/not_used/hmm_13_2_attempts.tex <==
We have \textcolor{peach}{identifiability when $d = k$}: we show that assuming $\mS \neq \mI$, then $\mEmiss$ is of rank at most $(k-1)$ which contradicts Assumption \ref{assump:discrete_full_rank}, hence it must be that $\mS = \mI$.
Let $s \in \R^d$ denote the diagonal of $\mS$.
Given some $s \neq \1$, columns of $\mEmiss$ are a subset of $\gX_1 := \{u \in \R^d: \sum_{j\in[d]} u_j = 1\}$; that is, each column of $\mEmiss$ has to sum up to 1.
Moreover, columns of $\mEmiss$ also form a subset $\gX_s := \{u \in \R^d: \sum_{j\in[d]} s_j u_j = 1\}$ since columns of $\tilde\mEmiss$ need to sum up to 1.
This means columns of $\mEmiss$ belong to $\gX_1 \cap \gX_s$.
Given the assumption that $s \neq \1$, $\gX_1 \cap \gX_s$ is a subspace of dimension $(k-1)$ or the empty set (which is possible, for instance, when $s = c\1$ for some $c \neq 1$).
The latter is clearly not possible, so $\gX_1 \cap \gX_s$ is of dimension $(k-1)$.
Hence any size-$d$ subset (e.g. the columns of $\mEmiss$) can be of dimension at most $(k-1)$, which contradicts Assumption \ref{assump:discrete_full_rank} that $\mEmiss$ is of rank $k$.

% This is because columns of $\mEmiss$ lie in the intersection of two hyperplanes (whose coefficients are specified by $\1$ and $\diag(\mS)$). 

For $d \geq k+1$,
\begin{equation}
\begin{split}
    \begin{cases}
        \mEmiss\mTrans = \tilde\mEmiss \tilde\mTrans = \mS\mEmiss \tilde\mTrans
        &\Rightarrow \tilde\mEmiss = \mS\mEmiss = \mEmiss\mTrans\tilde\mTrans^{-1}
        \\
        \mEmiss\mTrans^\top = \tilde\mEmiss \tilde\mTrans^\top 
        &\Rightarrow \tilde\mEmiss = \mEmiss\mTrans^\top (\tilde\mTrans^\top)^{-1}
        \\
    \end{cases}
    \Rightarrow \mTrans^{-1} \mTrans^\top = \tilde\mTrans^{-1} \tilde\mTrans^\top
\end{split}
\end{equation}

Let's see if we can find a counterexample for $d \geq k+1$ \textcolor{Orange}{(in progress)}.

\textcolor{gray}{requirements: 1) $\mS$ preserves the column space of $\mEmiss$; 2) $(\mTrans^\top)^{-1}\mTrans = (\tilde\mTrans^\top)^{-1}\tilde{\mTrans}$; 3) $\tilde\mTrans = \tilde\mEmiss^\dagger \mEmiss \mTrans$.}

\textcolor{RoyalBlue}{\textit{Direction 1}}: A counterexample requires $\tilde\mTrans := \mEmiss^\dagger\mS^{-1}\mEmiss \mTrans$ that also satisfies $\mEmiss\mTrans^\top = \tilde\mEmiss\tilde\mTrans^\top$.
Denote $\mR := \mTrans^{-1}\tilde\mTrans$, i.e. $\tilde\mTrans = \mTrans\mR$.
Then 
\begin{equation}
\begin{split}
    \tilde{\mEmiss}\tilde\mTrans = \mS \mEmiss \mTrans\mR
    = \mEmiss\mTrans
    \Rightarrow& \mR = (\mEmiss\mTrans)^{\dagger} \mS^{-1} \mEmiss\mTrans
    \\
    \tilde\mEmiss\tilde\mTrans^\top = \mS\mEmiss \mR^\top \mTrans^\top 
    = \mEmiss\mTrans^\top 
    \Rightarrow& \mR = (\mEmiss^\dagger \mS^{-1}\mEmiss)^\top.
\end{split}
\end{equation}
This means we need to find $\mEmiss, \mTrans, \mS$ s.t. 
\begin{equation}
\begin{split}
    (\mEmiss\mTrans)^{\dagger} \mS^{-1} \mEmiss\mTrans
    = \mTrans^{-1} (\mEmiss^\dagger \mS^{-1} \mEmiss) \mTrans
    = (\mEmiss^\dagger \mS^{-1}\mEmiss)^\top
\end{split}
\end{equation}
Since a matrix is always similar to its transpose, we only need to make sure such $\mTrans$ is doubly stochastic.
In particular, write the Jordan normal form of $\mJ = \mP^{-1}(\mEmiss^\dagger \mS^{-1}\mEmiss) \mP$ for appropriate $\mP$,
then we want $\mTrans := \mP\mB^{-1}\mP^\top$ to be doubly stochastic.
\textcolor{gray}{todo: analytical form of $\mP$?}

{\small\textcolor{gray}{
Why $\mP\mB^{-1}\mP^\top$:
let $\mB := \begin{bmatrix}
    0 & 0 & ... & 0 & 1 \\
    0 & 0 & ... & 1 & 0 \\
    \vdots & \vdots & \vdots & \vdots & \vdots \\
    1 & 0 & ... & 0 & 0 \\
\end{bmatrix} = \mB^{-1}$,
then $\mJ^\top = \mB \mJ \mB^{-1}$ for any Jordan matrix $\mJ$.
Let this $\mJ$ be the Jordan form of $\mA := \mEmiss^\dagger \mS^{-1}\mEmiss$, i.e. $\mP^{-1}\mA\mP = \mJ$,
then 
\begin{equation}
\begin{split}
    \mJ^\top = \mP^\top \mA^\top \mP^{-\top}
    \Rightarrow \mA^\top = (\mP^\top)^{-1} \mJ^\top \mP 
    = (\mP^\top)^{-1}\mB \mJ \mB^{-1} \mP^\top 
    = (\mP^\top)^{-1}\mB \mP^{-1} \mA \mP \mB^{-1} \mP^\top
\end{split}
\end{equation}
}}

\textcolor{RoyalBlue}{\textit{Direction 2}}: we want to find $\mS \in \R^{d \times d}$ s.t. $\mS\mO = \mO\mR$ for some $\mR \in \R^{k \times k}$; such $\mR$ should always exist since $\mS$ cannot change the column space of $\mEmiss$.
\textcolor{gray}{(but how to calculate $\mR$? $\mEmiss^\dagger\mS^{-1}\mEmiss$ could be $\mI_k$ even though $\mS \neq \mI_d$; e.g. see the example below)}
Then setting we can set $\tilde\mEmiss = \mEmiss\mR$, $\tilde\mTrans = \mR^{-1}\mTrans$ suffice.
Since $\tilde\mEmiss\tilde\mTrans^\top = \mEmiss\mTrans$, $\mR$ also needs to satisfy $\mR^{-1} \mTrans \mR^{\top} = \mTrans$.
\textcolor{gray}{(how?)}

To find such $\mS, \mR$, write $\mS := \begin{bmatrix}
    \mS_1 & 0 \\ 0 & \mS_2
\end{bmatrix}$ for $\mS_1 \in \R^{k \times k}$, $\mS_2 \in \R^{(d-k) \times (d-k)}$,
then 
\begin{equation}
\begin{split}
    \mS\mEmiss = \begin{bmatrix} \mS_1 \mEmiss_k \\ \mS_2 \mEmiss_{d-k} \end{bmatrix}
    = \begin{bmatrix}
        \mEmiss_k \mR \\ \mEmiss_{d-k} \mR
    \end{bmatrix}
    \Rightarrow \mR = \mEmiss_k^{-1} \mS_1 \mEmiss_k,
    ~\mS_2\mEmiss_{d-k} = \mEmiss_{d-k} \mEmiss_k^{-1} \mS_1 \mEmiss_k.
\end{split}
\end{equation}

\textcolor{RoyalBlue}{\textit{Direction 3}} (perhaps the cleanest route):
find $\mS$ that can preserve the column space of $\mEmiss$.
One example could be the following: choose $a,b,c \in (0,1)$, and set
\begin{equation}
\begin{split}
    \mEmiss =& \Big[ae_1 + (1-a)e_2, be_3 + (1-b)e_4, ce_5 + (1-c)e_6 \Big],
    \\
    \mS =& \diag\Big(\Big[s_1, \frac{1-s_1a}{1-a}, s_2, \frac{1-s_2b}{1-b}, s_3, \frac{1-s_3c}{1-c}\Big]\Big).
\end{split}
\end{equation}
Then $\tilde\mEmiss = \Big[s_1ae_1 + (1-s_1a)e_2, s_2be_3 + (1-s_2b)e_4, s_3ce_5 + (1-s_3c)e_6\Big]$, and
\begin{equation}
\begin{split}
    \tilde\mEmiss^\dagger \mEmiss
    = \diag\Big(\Big[
        \frac{2s_1a^2 - (1+s_1)a+1}{2s_1^2a^2 - 2s_1a + 1},
        \frac{2s_2b^2 - (1+s_2)b+1}{2s_2^2b^2 - 2s_2b + 1},
        \frac{2s_3c^2 - (1+s_3)c+1}{2s_3^2c^2 - 2s_3c + 1} \Big]\Big).
\end{split}
\end{equation}
% 
Since $\tilde\mTrans = \tilde\mEmiss^\dagger \mEmiss \mTrans$, we need columns of $\mEmiss^\dagger \mS^{-1} \mEmiss$ to sum up to 1,
which in this case means each diagonal entry is 1.
Hence $s_1 = \frac{1}{2a}$ and similar for $s_2, s_3$,
and $\tilde\mTrans = \mTrans$.
It can be checked that this case indeed have $\phi = \tilde\phi$, however $\mEmiss\mTrans \neq \tilde\mEmiss\tilde\mTrans$.

\textcolor{gray}{This kind of counterexample (i.e. aligning with the standard basis) doesn't seem promising, since the row space is now divided into disjoint subspaces, and the scaling is uniquely determined within each subspace.}


\textcolor{gray}{
\vspace{-0.8em}
\begin{itemize}[leftmargin=*]
    \item If $\mEmiss$ is of the form $\mEmiss = \begin{bmatrix} \mA & 0 \\ 0 & \mB \end{bmatrix}$, then we can reason about $\mA$ and $\mB$ separately.
    \item For $d=3$, $k=2$: if $\mEmiss = \begin{bmatrix}a & 0 \\ 1-a & b \\ 0 & 1-b\end{bmatrix}$: it must be that $\mS = \mI$.
\end{itemize}
}

Eliminating the set of possible choices of $s$:
\vspace{-0.8em}
\begin{itemize}[leftmargin=*]
    \item $\mS\mO$ is stochastic: dimension $d-(k-1)$ (at least 1-dim since $s = \1$ is a valid choice).
    \item $\mS\mO$ has the same column space as $\mO$: let $\mU \in \R^{d \times k}$ be the set of left singular vectors, then $\Vspan(\mS\mU) = \Vspan(\mU)$, i.e. $\forall u \in \Vspan(\mU), v \in \Vnull(\mU)$, $\langle s, u \odot v \rangle = 0$. \textcolor{gray}{(todo: what's the dimension of $\{u \odot v: u \in \Vspan(\mU), v \in \Vnull(\mU)\}$? Could be 0, e.g. if $\mU = [e_1, ..., e_k]$.)}
\end{itemize}

% Note that the above argument is necessary for the identifiability proof as well:
% Assume there exists $x_2, x_2'$ s.t. $\frac{\phi(x_2)}{\phi(x_2')}$ (element-wise division) has distinct values.
% Then denote $\mW_1 := \E[x_1 \otimes x_3|x_2]$, $\mW_2 := \E[x_1 \otimes x_3|x_2']$.
% We have 
% $$
% \mW_1\mW_2^{-1} = (\mEmiss\mTrans^{\top}) \diag\left(\frac{\phi(x_2)}{\phi(x_2')}\right) (\mEmiss\mTrans^{\top})^{-1},
% \mW_1^{-1}\mW_2 = (\mEmiss\mTrans)^{-\top} \diag\left(\frac{\phi(x_2')}{\phi(x_2)}\right) (\mEmiss\mTrans)^{\top},
% $$
% i.e. we can identify the products $\mEmiss\mTrans$ and $\mEmiss\mTrans^\top$.
% These two products are however not sufficient for identifiability.
% We need to additionally use the fact that the ratio $\frac{\phi(x_2)}{\tilde\phi(x_2)}$ is matched, which means $\phi(x_2) = \tilde\phi(x_2)$ and $\phi(x_2') = \tilde\phi(x_2')$ (there is no indeterminacy in scaling since $\phi, \tilde\phi$ both sum up to 1).


==> COLT2022/not_used/hmm_2_13_attempts.tex <==
\textcolor{gray}{// the following are some previous attempts}

The optimal predictor is defined with the posterior function $\phi_{13}$, 
\begin{equation}
\begin{split}
    &\phi_{13}(x_1, x_3)
    = [P(h_2=i|x_1, x_3)]_{i \in [k]}
    \eqLabel{1}= \left[\frac{P(x_1|h_2=i) P(x_3|h_2=i)}{\sum_{j \in [k]} P(x_1|h_2=j) P(x_3|h_2=j)}\right]_{i \in [k]}
    \\
    =& \left[\frac{\langle \fll(x_1), \mTrans_i^\top\rangle \langle \fll(x_3), \mTrans_i\rangle}{\sum_{j\in[k]} \langle \fll(x_1), \mTrans_j^\top\rangle \langle \fll(x_3), \mTrans_j\rangle}\right]_{i \in [k]}
    = \left[\frac{\langle \phi(x_1), \mTrans_i^\top\rangle \langle \phi(x_3), \mTrans_i\rangle}{\sum_{j\in[k]} \langle \phi(x_1), \mTrans_j^\top\rangle \langle \phi(x_3), \mTrans_j\rangle}\right]_{i \in [k]}
    \\
    =& \frac{\mTrans^\top \fll(x_1) \odot \mTrans\fll(x_3)}{\|\mTrans^\top \fll(x_1) \odot \mTrans\fll(x_3)\|_1}
    = \frac{\mTrans^\top \phi(x_1) \odot \mTrans\phi(x_3)}{\|\mTrans^\top \phi(x_1) \odot \mTrans\phi(x_3)\|_1},
\end{split}
\end{equation}
where step $\rnum{1}$ uses Assumption \ref{assump:latent} that the latent distribution is uniform.

Matching $\E[x_2|x_1,x_3]$ means 
$\mEmiss\Tensor[x_1, x_3] = \tilde\mEmiss\tilde\Tensor[x_1, x_3]$, where the 3-tensor $\Tensor \in \R^{d \times d \times k}$ is defined as 
\begin{equation}
\begin{split}
    \Tensor[:, :, l]
    := \mH^{(l)}
    := (P(x_1|h_2=l) P(x_3|h_2=l)^\top) \oslash \mS,
\end{split}
\end{equation}
where $\oslash$ denotes the Hadamard division (i.e. entrywise division), and $\mS \in \R^{d \times d}$ is defined as
\begin{equation}
\begin{split}
    \mS_{ij}
    := \sum_{l' \in [k]} P(x_1=i|h_2=l') P(x_3=j|h_2=l')
    = \langle (\mEmiss\mTrans^\top)_{i:}, (\mEmiss\mTrans)_{j:} \rangle
    = (\mEmiss_{i:})^\top \mTrans^\top \mTrans^\top \mEmiss_{j:}.
\end{split}
\end{equation}

\textcolor{RoyalBlue}{Matching $\phi_{13}$ doesn't give identifiability}: 
to construct a counterexample, it suffices to choose symmetric $\mTrans, \tilde\mTrans$, doubly stochastic (up to scaling $\frac{k}{d}$) $\mEmiss,\tilde\mEmiss$, and $\mEmiss\mTrans = \tilde\mEmiss\tilde\mTrans$.
Then
\begin{equation}
\begin{split}
    \phi_{13}(x_1=i, x_3=j)
    = \frac{(\mEmiss\mTrans^\top)_{i:} \odot (\mEmiss\mTrans)_{j:}}{\|(\mEmiss\mTrans^\top)_{i:} \odot (\mEmiss\mTrans)_{j:}\|_1}
    = \frac{(\tilde\mEmiss\tilde\mTrans^\top)_{i:} \odot (\tilde\mEmiss\tilde\mTrans)_{j:}}{\|(\tilde\mEmiss\tilde\mTrans^\top)_{i:} \odot (\tilde\mEmiss\tilde\mTrans)_{j:}\|_1}
    = \tilde\phi_{13}(x_1=i, x_3=j).
\end{split}
\end{equation}
The following is a concrete counterexample: consider $d = k = 3$, and let $a = 0.8$,
\begin{equation}
\begin{split}
    &\mTrans = \begin{bmatrix}
        a & 1-a & 0 \\ 1-a & 0 & a \\ 0 & a & 1-a \\
    \end{bmatrix},
    ~\tilde\mTrans = \begin{bmatrix}
        a & 0 & 1-a \\ 0 & 1-a & a \\ 1-a & a & 0 \\
    \end{bmatrix},
    \mR = \tilde\mTrans \mTrans^{-1},
    \\
    &\mEmiss = \begin{bmatrix}
       0.4695323  & 0.40420827 & 0.12625944 \\
       0.27370492 & 0.40545776 & 0.32083732 \\
       0.25676278 & 0.19033397 & 0.55290324 \\
    \end{bmatrix},
    \\
    &\tilde\mEmiss = \mEmiss\mR^{-1}
        = \begin{bmatrix}
       0.52864941 & 0.30361077 & 0.16773982 \\
       0.30336755 & 0.4098252  & 0.28680725 \\
       0.16798304 & 0.28656402 & 0.54545293 \\
        \end{bmatrix}.
\end{split}
\end{equation}
We can also have $d = 4 > k=3$: let $\mTrans, \tilde\mTrans, \mR$ be the same as above, and let $\mEmiss, \tilde\mEmiss$ be:
{\small
\begin{equation*}
\begin{split}
    \mEmiss = \begin{bmatrix}
       0.36290765 & 0.33875795 & 0.0483344  \\
       0.27741051 & 0.27428275 & 0.19830674 \\
       0.13599324 & 0.23416529 & 0.37984147 \\
       0.22368861 & 0.152794   & 0.37351739 \\
    \end{bmatrix},
    \tilde\mEmiss = \begin{bmatrix}
       0.4280708  & 0.24382385 & 0.07810535 \\
       0.29470284 & 0.25018373 & 0.20511344 \\
       0.10992735 & 0.30164382 & 0.33842882 \\
       0.16729901 & 0.2043486  & 0.37835239 \\
    \end{bmatrix}.
\end{split}
\end{equation*}
}

\textcolor{RoyalBlue}{$\tilde\mEmiss = \mEmiss\mR^{-1}$, $\tilde\Phi_{13} = \mR\Phi_{13}$ for some $\mR$.}
Let's assume $\mTrans$ is symmetric so that we have 
\begin{equation}
\begin{split}
    \E[x_2|x_1=i, x_3=j] 
    = \sum_{h \in [k]} \mEmiss_h \cdot \underbrace{\frac{(\mEmiss\mTrans)_{i,h} (\mEmiss\mTrans)_{j,h}}{\sum_{\bar{h}}(\mEmiss\mTrans)_{i,\bar{h}} (\mEmiss\mTrans)_{j,\bar{h}}}}_{:= \phi_{13}(i,j)}
\end{split}
\end{equation}
One idea is to find some $\mR$ (invertible but not necessarily orthogonal) s.t. $\tilde\mEmiss = \mEmiss\mR^{-1}$.
Let $\Phi_{13} := [\phi_{13}(1,1), ..., \phi_{13}(d,d)] \in \R^{k \times d}$, and define $\tilde\Phi_{13}$ similarly.
Matching the optimal predictor means $\tilde\Phi_{13} = \mR\Phi_{13}$.

Denote $\mA := \tilde\mEmiss \tilde\mTrans$, then
\begin{equation}
\begin{split}
    \phi_{13}(i,i) = \frac{\mA_{i,:} \odot \mA_{i,:}}{\|\mA_{i,:} \odot \mA_{i,:}\|_1}
    \eqLabel{1}\Rightarrow \mA_{i,:} \propto \sqrt{\phi_{13}(i,i)}
    \Rightarrow \tilde\mTrans = \tilde\mEmiss^{-1}\mA.
\end{split}
\end{equation}
where step $\rnum{1}$ chooses the scaling of $\mA$ such that the columns sum up to 1.
We will have a counterexample if we can find $\mEmiss, \mTrans, \mR$ s.t. $\tilde\mTrans$ is symmetric (which implies doubly stochastic).
\textcolor{gray}{\textcolor{Orange}{todo}: find such a counterexample.}

\textcolor{gray}{what properties does $\Phi_{13}$ have for a doubly stochastic $\mTrans$?}


\textcolor{RoyalBlue}{Can we take a dummy $\hat{p}(x_1,x_3)$?}
Suppose we have a dummy distribution where $\hat{p}(x_1, x_3)$ is independent of a specific choice of parameters.
We would like to apply Kruskal on the following tensor:
\begin{equation}
\begin{split}
    \Tensor
    :=& \sum_{x_1,x_3} \hat{p}(x_1,x_3) x_1 \otimes x_3 \otimes \E[x_2|x_1,x_3]
    \\
    =& \sum_{h_2} \Big(\sum_{x_1,x_3} \underbrace{\hat{p}(x_1, x_3) p(h_2|x_1,x_3)}_{:= \hat{p}(x_1,x_3,h_2)} x_1 \otimes x_3 \Big) \otimes \E[x_2|h_2]
    \\
    =& \sum_{h_2} \hat{p}(h_1) \hat\E[x_1|h_2] \otimes \hat\E[x_3|h_2] \otimes \E[x_2|h_2].
\end{split}
\end{equation}
$\Tensor$ will have a unique decomposition if
1) we can find $\hat\mEmiss, \hat\mTrans$ that produce $\hat{p}(x_1, x_3, h_2)$,
and that
2) $\{\hat\E[x_1|h_2=i]: i\in[k]\}$ is of rank-$k$.

Let's first try $\hat{p}(x_1, x_3) = \frac{1}{d^2}$.
Then 
\begin{equation}
\begin{split}
    &\hat{p}(x_1=i, x_3=j, h_2=l)
    \\
    =&~ p(h_2=l|x_1=i,x_3=j) \cdot \hat{p}(x_1,x_3)
    = \frac{(\mEmiss\mTrans^\top)_{il} (\mEmiss\mTrans)_{jl}}{\sum_{l'} (\mEmiss\mTrans^\top)_{il'} (\mEmiss\mTrans)_{jl'}} \cdot \frac{1}{d^2}
    \\
    =&~ \hat{p}(x_1=i|h_2=l) \hat{p}(x_3=j|h_2=l) \hat{p}(h_2)
    = (\hat\mEmiss \hat\mTrans^\top)_{il} \cdot (\hat\mEmiss \hat\mTrans)_{jl} \cdot \hat{p}(h_2)
    \\
    \Rightarrow~& \sum_{l\in[k]} \hat{p}(x_1=i, x_3=j, h_2=l)
        = \frac{1}{d^2} 
        = \hat{p}(h_2) \langle (\hat{\mEmiss}\hat{\mTrans}^\top)_{i:}, (\hat{\mEmiss}\hat{\mTrans})_{j:} \rangle
    \\
    \Rightarrow~& \langle (\hat{\mEmiss}\hat{\mTrans}^\top)_{i:}, (\hat{\mEmiss}\hat{\mTrans})_{j:} \rangle = \frac{\hat{p}(h_2)}{d^2}
\end{split}
\end{equation}
If $\hat{\mTrans}$ is symmetric and $\hat{p}(h_2)$, then $\langle (\hat{\mEmiss}\hat{\mTrans})_{i:}, (\hat{\mEmiss}\hat{\mTrans})_{i:} \rangle = \|\hat\mEmiss \hat\mTrans\|_2 = \frac{1}{\sqrt{d}}$ while $\|\hat\mEmiss \hat\mTrans\|_1 = 1$,
hence $\hat\mEmiss \hat\mTrans = \frac{1}{d}\1$, and $\hat\mEmiss \hat\mTrans$ is of rank-1.
\textcolor{gray}{In fact $\mEmiss\mTrans$ has to be rank-1 just by the choice of $p(x_1,x_3)$:
\begin{equation}
\begin{split}
    &p(x_1=i, x_3=j)
    = \frac{1}{k}\sum_{l\in[k]} p(x_1=i|h_2=l) p(x_3=j|h_2=l)
    = \frac{\langle (\mEmiss\mTrans^\top)_{i:}, (\mEmiss\mTrans)_{j:} \rangle}{k}
    = \frac{1}{d^2}
    \\
    &\Rightarrow (\mEmiss\mTrans^\top)_{i:} = (\mEmiss\mTrans)_{j:}, ~\forall i, j \in [d].
\end{split}
\end{equation}
}

\textcolor{gray}{other choices of $\hat{p}(x_1,x_3), \hat{p}(h_2)$ and non-symmetric $\mTrans$?
May not help: we should keep $\hat{p}(h_2)$ uniform (\textcolor{Orange}{should we?}).
Then to match $p(x_1,x_3)$, $p(h_2|x_1,x_3)$, $p(h_2, x_1, x_3)$, it suffices to match $\mEmiss\mTrans$ and $\mEmiss\mTrans^\top$.}


\textcolor{gray}{// Attempts before Feb 2nd (\textcolor{red}{ignore}, since these are based on the assumption that $\mEmiss = \tilde\mEmiss$)}

The optimal predictor takes the form $\E[x_2|x_1, x_3] 
= \mEmiss \phi_{13}(x_1, x_3)$,
% \begin{equation}
% \begin{split}
%     \E[x_2|x_1, x_3] 
%     = \mEmiss \phi_{13}(x_1, x_3)
%     = \mEmiss \frac{\mTrans^\top \fll(x_1) \odot \mTrans\fll(x_3)}{\|\mTrans^\top \fll(x_1) \odot \mTrans\fll(x_3)\|_1}
%     = \mEmiss \frac{\mTrans^\top \phi(x_1) \odot \mTrans\phi(x_3)}{\|\mTrans^\top \phi(x_1) \odot \mTrans\phi(x_3)\|_1}.
% \end{split}
% \end{equation}
which when combined with $\tilde\mEmiss = \mEmiss$ implies $\phi_{13}(x_1, x_3) = \tilde\phi_{13}(x_1, x_3)$ .

For the discrete case (\textcolor{Orange}{in progress}), matching the posterior $\phi_{13}$ means 
\begin{equation}
\begin{split}
    \phi_{13}(x_1, x_3)
    = \frac{(\mTrans^\top \mEmiss^\top x_1) \odot (\mTrans\mEmiss^\top x_3)}{\|(\mTrans^\top \mEmiss^\top x_1) \odot (\mTrans\mEmiss^\top x_3)\|_1}
    = \frac{(\tilde\mTrans^\top \tilde\mEmiss^\top x_1) \odot (\tilde\mTrans\tilde\mEmiss^\top x_3)}{\|(\tilde\mTrans^\top \tilde\mEmiss^\top x_1) \odot (\tilde\mTrans \tilde\mEmiss^\top x_3)\|_1}
    = \tilde\phi_{13}(x_1, x_3).
    %% matching per entry
    % \frac{(\mEmiss\mTrans^\top)_{i,h} (\mEmiss\mTrans)_{j,h}}{\sum_{\bar{h}}(\mEmiss\mTrans^\top)_{i,\bar{h}} (\mEmiss\mTrans)_{j,\bar{h}}}
    % = \frac{(\mEmiss\tilde\mTrans^\top)_{i,h} (\mEmiss\tilde\mTrans)_{j,h}}{\sum_{\bar{h}}(\mEmiss\tilde\mTrans^\top)_{i,\bar{h}} (\mEmiss\tilde\mTrans)_{j,\bar{h}}},
    % \forall i,j \in [d].
\end{split}
\end{equation}
\textcolor{RoyalBlue}{\textit{If $\mTrans, \tilde\mTrans$ are both symmetric}}: Taking $x_1 = x_3 = \ei$ for $i \in [k]$, then 
$\phi_{13}(\ei, \ei) = \frac{(\mTrans \mEmiss^\top)_i^2}{\|(\mTrans \mEmiss^\top)_i\|_2^2}$ (where the square is applied entrywise).
Since $\mTrans\mEmiss^\top$ has non-negative entries, we can recover $\mTrans\mEmiss^\top$ up to a column-wise scaling, i.e. this suffices to recover $\mTrans\mS_k \mEmiss^\top$ for some positive diagonal matrix $\mS_k$.
Then, given that $\mEmiss$ is known and $\mTrans$ has columns summing up to 1, we also recover $\mTrans$.

\textcolor{RoyalBlue}{Generic $\mTrans$} \textcolor{gray}{(in progress)}:
\begin{equation}
\begin{split}
    &\frac{(\mTrans^\top \mEmiss^\top \ei) \odot (\mTrans\mEmiss^\top \ej)}{\|(\mTrans^\top \mEmiss^\top \ei) \odot (\mTrans\mEmiss^\top \ej)\|_1}
        = \frac{(\tilde\mTrans^\top \tilde\mEmiss^\top \ei) \odot (\tilde\mTrans\tilde\mEmiss^\top \ej)}{\|(\tilde\mTrans^\top \tilde\mEmiss^\top \ei) \odot (\tilde\mTrans \tilde\mEmiss^\top \ej)\|_1},
        ~\forall i, j \in [d]
    \\
    \Rightarrow&~
    \underbrace{\frac{\|(\tilde\mTrans^\top \tilde\mEmiss^\top \ei) \odot (\tilde\mTrans \tilde\mEmiss^\top \ej)\|_1}{\|(\mTrans^\top \mEmiss^\top \ei) \odot (\mTrans\mEmiss^\top \ej)\|_1}}_{:= r_{ij}}
        \cdot (\mTrans^\top \mEmiss^\top \ei) \odot (\mTrans\mEmiss^\top \ej)
        = (\tilde\mTrans^\top \tilde\mEmiss^\top \ei) \odot (\tilde\mTrans\tilde\mEmiss^\top \ej)
    \\
    \Rightarrow&~
    \begin{cases}        
        &(\mTrans^\top \sum_{i} r_{ij} \mEmiss_i^\top) \odot (\mTrans\mEmiss_j^\top)
        = (\mTrans^\top \mEmiss^\top r_{:,j}) \odot (\mTrans\mEmiss_j^\top)
        = \tilde\mTrans\1 \odot (\tilde\mTrans\tilde\mEmiss_j^\top)
        = \tilde\mTrans \tilde\mEmiss_j^\top
        \\
        &(\mTrans^\top\mEmiss_i^\top) \odot (\mTrans\mEmiss^\top r_{i,:}) = \tilde\mTrans^\top \tilde\mEmiss_i^\top
    \end{cases}
    \\
    \Rightarrow&~
    \begin{cases}
        &(\mTrans^\top \mEmiss^\top R) \odot (\mTrans\mEmiss^\top) = \tilde\mTrans \tilde\mEmiss^\top 
        \\
        &(\mTrans^\top \mEmiss^\top) \odot (\mTrans\mEmiss^\top R^\top) = \tilde\mTrans^\top \tilde\mEmiss^\top
    \end{cases}
\end{split}
\end{equation}
\textcolor{gray}{
If $r_{ij} = 1$, i.e. $(\mTrans^\top\mEmiss^\top x_1) \odot (\mTrans\mEmiss^\top x_3)$, then $\mTrans$ is determined.
\begin{equation*}
\begin{split}
    \sum_{i \in [d]} (\mTrans^\top \mEmiss_i^\top) \odot (\mTrans\mEmiss_j^\top)
    = (\mTrans^\top \sum_{i \in [d]} \mEmiss_i^\top)) \odot (\mTrans\mEmiss_j^\top)
    = \mTrans^\top \1 \odot (\mTrans\mEmiss_j^\top)
    = \1 \odot (\mTrans\mEmiss_j^\top)
    = \mTrans\mEmiss_j^\top.
\end{split}
\end{equation*}
The above holds for all $j \in [d]$, hence we have both $\mTrans\mEmiss$ and $\mEmiss$, which gives identifiability.
}

\textcolor{gray}{// the end of previous attempts}



==> COLT2022/not_used/proof_gmm_pairwise_marginals.tex <==
\subsection{Proof for Lemma \ref{lem:gmm_marginal} (identifiability from pairwise marginals)}
% \begin{proof}
    Matching the pairwise marginal $p(x_1, x_2)$ means the singleton marginal $p(x_1)$ also matches.
    The identifiability then follows directly from the identifiability of Gaussian mixtures (Lemma \ref{lem:gmm_id}).
    % In particular, take a basis $\{\vv_l\}_{l \in [d]}$, then the projection of the $d$-dimensional Gaussian mixture on each $\vv_l$ is identifiable by Proposition 1 in \href{https://projecteuclid.org/journals/annals-of-mathematical-statistics/volume-34/issue-4/Identifiability-of-Finite-Mixtures/10.1214/aoms/1177703862.full}{Teicher 63}.
    % These projections recover $\{\vv_l^\top \mu_i\}_{i \in [k]}$, hence knowing the projections for all $l \in [d]$ recovers $\{\mu_i\}_{i \in [k]}$.

    To recover $\mTrans$, write the pairwise marginal as $p(x_1, x_2; \mMeans, \mTrans) = \frac{1}{k(2\pi)^{d}} \psi(x_1)^\top \mTrans \psi(x_2)$, where $\psi: \R^{d} \rightarrow \R^k$ is the (scaled) likelihood function where $[\psi(x)]_i := \exp\big(-\frac{\|x-\mu_i\|^2}{2}\big)$.
    Choose a set $\gX := \{x^{(i)}\}_{i \in [k]}$ s.t. $\Psi_\gX := [\psi(x^{(1)}), ..., \psi(x^{(k)})] \in \R^{k \times k}$ is full rank.
    Then we have:
    \begin{equation}
    \begin{split}
        \Psi_\gX^\top \mTrans \Psi_\gX
        = \tilde\Psi_{\gX}^\top \tilde\mTrans \tilde\Psi_\gX
        = \Psi_\gX^\top \tilde\mTrans \Psi_\gX 
        \Rightarrow \mTrans = \tilde\mTrans.
    \end{split}
    \end{equation}
% \end{proof}

==> COLT2022/proof_GHMM/id_21_31.tex <==
\subsection{Identifiability from predicting both $x_2|x_1$ and $x_3|x_1$}


% \textcolor{RoyalBlue}{// Matching $x_2|x_1$ and $x_3|x_1$ gives identifiability}

% % \vspace{-1em}
% \begin{theorem}[Identifiability for \GHMM~from both $x_2|x_1$ and $x_3|x_1$]
% \label{thm:gmm_21_31}
%     Under Assumption \ref{assump:latent}, \ref{assump:gmm_full_rank}, and \ref{assump:gmm_equal_norms},
%     if $\mMeans, \mTrans$ and $\tilde\mMeans, \tilde\mTrans$ give the same predictor for both predicting $x_2$ given $x_1$ and predicting $x_3$ given $x_1$,
%     then $\tilde\mMeans = \mMeans$, $\tilde\mTrans = \mTrans$ up to a permutation of labeling.
% \end{theorem}
% The proof again leverages Lemma \ref{lem:gmm_matchPhi} that matching the predictor implies matching the posterior function,
% which means the (linear) mapping from the latent to $x_2$ and $x_3$ also need to match.
% Having the same predictor for $x_2$ given $x_1$ means matching the linear map of the form $\mMeans\mTrans$, which is not sufficient to identify the factors $\mMeans, \mTrans$, leaving the indeterminacy of $\mH$ in Theorem \ref{thm:gmm_2_1_id}.
% However, additional matching the predictor for $x_3$ given $x_1$ introduces another equation on $\mMeans\mTrans^2$, which eliminates this indeterminacy.



Theorem \ref{thm:gmm_2_1_id} states that predicting $x_2$ from $x_1$ identifies $\mMeans$ up to a permutation and a unique Householder reflection $\mH$.
Theorem \ref{thm:gmm_conditional} shows that the indeterminacy of $\mH$ can be removed by considering the conditional distribution as opposed to the conditional expectation.
The following result provides another way to eliminate $\mH$, by predicting both $x_2|x_1$ and $x_3|x_1$:
\vspace{-1em}
\begin{theorem}[Identifiability from predicting $x_2|x_1$ and $x_3|x_1$]
\label{thm:gmm_21_31} 
    Under Assumption \ref{assump:latent}, \ref{assump:gmm_full_rank},
    if the predictor has \emph{\textcolor{Orange}{the correct parametric form}},
    then the parameters $\tilde\mMeans, \tilde\mTrans$ can be recovered up to permutation, by predicting $x_{2}$ given $x_1$ and predicting $x_3$ given $x_1$, $\forall k \geq 2$.
\end{theorem}
% 
\begin{proof}
    \textcolor{Orange}{todo: we have a much simpler proof using Lemma \ref{lem:gmm_matchPhi}}

    Learning the optimal predictor for predicting both $x_2|x_1$ and $x_3|x_1$ means:
    \begin{equation}
    \begin{split}
        \begin{cases}
            f^{2|1}(x) = \mMeans\mTrans\phi(x)
            = \tilde{f}_{2|1}(x) = \tilde\mMeans\tilde\mTrans\tilde\phi(x)
            \\
            f_{3|1}(x) = \mMeans\mTrans^{3-1}\phi(x)
            = \tilde{f}_{3|1}(x) = \tilde\mMeans\tilde\mTrans^2\tilde\phi(x).
        \end{cases}
    \end{split}
    \end{equation}
    Choose a set $\gX := \{x^{(i)}\}_{i \in [k]}$ s.t. $\Phi_{\gX} := [\phi(x^{(1)}), ..., \phi(x^{(k)})]$ is of rank $k$.
    Let $\tilde\Phi_{\gX}$ be defined similarly.
    Then
    \begin{equation}
    \begin{split}
        &\begin{cases}
            \mMeans\mTrans\Phi_{\gX} = \tilde\mMeans\tilde\mTrans\tilde\Phi_{\gX}
            &\Rightarrow \mMeans^{\dagger}\tilde\mMeans = (\mTrans\Phi_{\gX}) \cdot (\tilde\mTrans\tilde\Phi_{\gX})^\dagger
            \\
            \mMeans\mTrans^2\Phi_{\gX} = \tilde\mMeans\tilde\mTrans^2\tilde\Phi_{\gX}
            &\Rightarrow \tilde\mTrans = \tilde\mMeans^{\dagger} \mMeans \cdot \mTrans \cdot (\mTrans \Phi_{\gX}) (\tilde{\mTrans} \tilde\Phi_{\gX})^\dagger
                = \tilde\mMeans^{\dagger} \mMeans \cdot \mTrans \cdot \mMeans^\dagger \tilde\mMeans
        \end{cases}
        \\
        \Rightarrow&\ \tilde\mMeans \tilde\mTrans \tilde\phi(x)
            = (\tilde\mMeans \tilde\mMeans^{\dagger}) \mMeans \cdot \mTrans \cdot \mMeans^\dagger \tilde\mMeans \tilde\phi(x)
            \eqLabel{1}{=} \mMeans \mTrans \cdot \mMeans^\dagger \tilde\mMeans \tilde\phi(x)
            = \mMeans\mTrans\phi(x), ~\forall x
        \\
        \Rightarrow&\ \mMeans^\dagger \tilde\mMeans \tilde\phi(x) = \phi(x), ~\forall x
        ~\eqLabel{2}\Rightarrow\ \tilde\mMeans\tilde\phi(x) = \mMeans\phi(x), ~\forall x,
    \end{split}
    \end{equation}
    where step $\rnum{1}$ uses $(\tilde\mMeans \tilde\mMeans)^\dagger \mMeans = \mMeans$, since $\tilde{\mMeans}, \mMeans$ share the same column space;
    step $\rnum{2}$ uses $(\mMeans \mMeans)^\dagger \tilde\mMeans = \tilde\mMeans$, since $\tilde{\mMeans}, \mMeans$ share the same column space.
    
    Denote $g(x) := \mMeans\phi(x)$, and $\tilde{g}(x) := \tilde\mMeans\tilde\phi(x)$.
    Then we have $\forall x$, $g(x)=\tilde{g}(x)$, and $\nabla_{x} g(x) = \nabla_{x} \tilde{g}(x)$:
    \begin{equation}
    \begin{split}
        &\nabla_x g(x) = \mMeans \nabla_{x} \phi(x)
        = \mMeans \diag(\phi(x)) \mMeans^\top - (\mMeans \phi(x)) \cdot (\mMeans\phi(x))^\top
        \\
        =& \nabla_x \tilde{g}(x)
        = \tilde\mMeans \diag(\tilde\phi(x)) \tilde\mMeans^\top - (\tilde\mMeans \tilde\phi(x)) \cdot (\tilde\mMeans\tilde\phi(x))^\top 
        \\
        \eqLabel{1}{=}& \tilde\mMeans \diag(\tilde\phi(x)) \tilde\mMeans^\top - (\mMeans \phi(x)) \cdot (\mMeans\phi(x))^\top
        \\
        \Rightarrow& \mMeans\diag(\phi(x))\mMeans^\top = \tilde{\mMeans} \diag(\tilde{x}) \tilde\mMeans^\top,
    \end{split}
    \end{equation}
    where step $\rnum{1}$ substitutes in $g(x) = \tilde{g}(x)$ for the second term.
    
    Our goal is to show that $\mu_i = \tilde\mu_{\perm(i)}$ for some permutation $\perm$. Without loss of generality, let's fix \textcolor{Orange}{$\perm = \text{id}$}.
    For $i \in [k]$, we claim that there exists $x^{(i)}$ s.t. \textcolor{Orange}{$\lim_{c \rightarrow \infty}\phi(x_c^{(i)}) \rightarrow \ve_i$}.
    To construct such $x_c^{(i)}$, it suffices to find a direction $\vv^{(i)} \in \R^d$, $\|\vv^{(i)}\|_2 = 1$, such that $\vv^{(i)}(\mu_i - \mu_j) > 0$, $\forall j \neq i$;
    such $\vv^{(i)}$ exists since $\{\mu_i\}_{i \in [k]}$ form a convex hull by the assumption that $\mMeans$ has linearly independent columns.
    With such $\vv^{(i)}$, define $\hat{x}_c^{(i)} := \mu_i + c\vv^{(i)}$, then
    \begin{equation}
    \begin{split}
        \lim_{c\rightarrow \infty}[\phi(\hat{x}_c^{(i)})]_i =& \lim_{c\rightarrow \infty}\frac{\exp\big(-\frac{c^2\|\vv\|^2}{2}\big)}{\exp\big(-\frac{c^2\|\vv\|^2}{2}\big) + \sum_{j \neq i} \exp\big(-\frac{\|\mu_i - \mu_j + c\vv^{(i)}\|_2^2}{2}\big)}
        \\
        =& \lim_{c\rightarrow \infty}\left(1 + \sum_{j\neq i} \exp\Big(-\frac{\|\mu_i - \mu_j\|^2 + 2c\vv^{(i)}(\mu_i - \mu_j)}{2}\Big)\right)^{-1}
        = 1
    \end{split}
    \end{equation}
    Hence \textcolor{Orange}{$\lim_{c \rightarrow \infty}\phi(\hat{x}_c^{(i)}) = \ve_i$}.
    For such choices of $\hat{x}^{(i)}$, 
    \begin{equation}
    \begin{split}
        \mMeans\diag(\phi(\hat{x}^{(i)}))\mMeans^\top 
        = \mu_i \mu_i^\top 
        = \sum_{j \in [k]} [\tilde\phi(\hat{x}^{(i)})]_j \tilde\mu_j\tilde\mu_j^\top.
    \end{split}
    \end{equation}
    The LHS is of rank 1, so the the RHS must also be of rank 1, i.e. $\tilde\phi(\hat{x}^{(i)}) = \ve_i$, and $\mu_i = \tilde\mu_i$.
    Hence $\mMeans = \tilde\mMeans$, and $\phi = \tilde\phi$, and consequently $\mTrans = \tilde\mTrans$.
\end{proof}

%% Old proof specific to G-HMM; \tThr-\tTwo = \tTwo-\tOne
% \input{COLT2022/not_used/gmm_31_21_new}

%% wrong proof: mistakes in calculating the 3-tensor 
% \input{COLT2022/not_used/gmm_31_21_generic_wrong.tex}

%% Commented out the special case of predicting x2|x1 and x1|x2
% \input{COLT2022/not_used/gmm_21_12}


==> COLT2022/proof_GHMM/threeTokens_old.tex <==
\subsection{Proof for Theorem \ref{thm:gmm} (identifiability from prediction tasks over three tokens)}
% \begin{proof}

The proof for \GHMM~follows exactly the same argument as in the discrete case, expect that the posterior function $\phi$ takes a different parametric form.
In particular, the posterior function is now
\begin{equation}
\begin{split}
    [\phi(x_t)]_i
    :=& P(h_t=i|x_t)
    = \frac{P(x_t|h_t=i) P(h_t=i)}{\sum_{j \in [k]} P(x_t|h_t=j) P(h_t=j)}
    \\
    \eqLabel{1}=& \frac{P(x_t|h_t=i)}{\sum_{j \in [k]} P(x_t|h_t=j)}
    = \frac{\exp(-\|x_t-\mMeans_i\|^2/2)}{\sum_{j \in [k]} \exp(-\|x_t-\mMeans_j\|^2/2)},
\end{split}
\end{equation}
where step $\rnum{1}$ uses Assumption \ref{assump:latent} that the hidden state is at stationarity and uniformly distributed.

\textcolor{Orange}{As an example}, consider the task of $x_2 \otimes x_3|x_1$.
The optimal predictor is now
\begin{equation}
\begin{split}
    &f^{2,3|1}(x_1) = \E[x_2\otimes x_3|x_1]
    = \sum_{i,j \in [k]} P(h_2=i|h_1=j) P(h_1=j|x_1) \E[x_2\otimes x_3|h_2=i] 
    \\
    =& \sum_{i \in [k]} \big(\sum_{j \in [k]} \mTrans_{ij} [\phi(x_1)]_j\big) \mMeans_i \otimes (\mMeans\mTrans)_i 
    = \mMeans \diag(\mTrans\phi(x_1))\mTrans^\top \mMeans^\top.
\end{split}
\end{equation}
As in the discrete case, we will construct a 3-tensor using the optimal predictor, then apply Kruskal's theorem to this 3-tensor.
Let $\weight(x_1)$ denote a weight
\begin{equation}
\begin{split}
    \Tensor_\weight
    :=& \sum_{x_1} \weight(x_1) x_1 \otimes f^{2,3|1}(x_1) 
    = \sum_{x_1} \weight(x_1) x_1 \otimes \sum_{i \in [k]} \big(\sum_{j \in [k]} \mTrans_{ij} [\phi(x_1)]_j\big) \mMeans_i \otimes (\mMeans\mTrans)_i
    \\
    =& \sum_{i \in [k]} \Big(\sum_{x_1} \sum_{j \in [k]} \mTrans_{ij} [\phi(x_1)]_j \weight(x_1) x_1 \Big) \otimes \mMeans_i \otimes (\mMeans\mTrans)_i 
    \\
    =& \sum_{i \in [k]} \Big(\sum_{x_1} P(h_2=i|x_1) \weight(x_1) x_1 \Big) \otimes \mMeans_i \otimes (\mMeans\mTrans)_i 
\end{split}
\end{equation}
Take $\weight(x_1) = P(x_1)$, then the first component involving $x_1$ is 
\begin{equation}
\begin{split}
    &\sum_{x_1} P(h_2=i|x_1) P(x_1) x_1
    = P(h_2=i) \sum_{x_1} P(x_1|h_2=i) x_1
    \\
    =& P(h_2=i) \E[x_1|h_2=i]
    = \Pstat{2}{i} (\mMeans\mTrans^\top)_i.
\end{split}
\end{equation}
Therefore $\Tensor_\weight = \sum_{i \in [k]} \Pstat{2}{i} (\mMeans\mTrans^\top)_i \otimes \mMeans_i \otimes (\mMeans\mTrans)_i$, where each of the three components has Kruskal rank $k$ by Assumption \ref{assump:gmm_full_rank}.
Then columns of $\mMeans, \mMeans\mTrans$ and hence also $\mTrans$ are identified up to a shared permutation and scaling by Kruskal's theorem.
The indeterminacy in scaling can be further removed since columns of $\mTrans$ need to sum up to 1.

%% Old special case of \tOne=1, \tTwo=2, \tThr=3
% \input{COLT2022/not_used/gmm_31_21_old}

==> COLT2022/proof_HMM/attempt_case3_2_13.tex <==

Let $\fll$ denote the likelihood function, i.e. $[\fll(x)]_i = P(x|h=i)$, then the posterior of $h_2$ is
\begin{equation}
\begin{split}
    P(h_2=i|x_1, x_3)
    =& \frac{P(x_1|h_2=i) P(x_3|h_2=i)}{\sum_{j \in [k]} P(x_1|h_2=j) P(x_3|h_2=j)}
    \\
    =& \frac{\langle \fll(x_1), \mTrans_i^\top\rangle \langle \fll(x_3), \mTrans_i\rangle}{\sum_{j\in[k]} \langle \fll(x_1), \mTrans_j^\top\rangle \langle \fll(x_3), \mTrans_j\rangle}
    \eqLabel{1}= \frac{\langle \phi(x_1), \mTrans_i^\top\rangle \langle \phi(x_3), \mTrans_i\rangle}{\sum_{j\in[k]} \langle \phi(x_1), \mTrans_j^\top\rangle \langle \phi(x_3), \mTrans_j\rangle},
    \\
    \phi_{13}(x_1, x_3) =& \frac{\mTrans \phi(x_1) \odot \mTrans^\top\phi(x_3)}{\|\mTrans \phi(x_1) \odot \mTrans^\top\phi(x_3)\|_1}
\end{split}
\end{equation}
where step $\rnum{1}$ uses the assumption that the latent distribution is uniform.

For Gaussian (\textcolor{Orange}{in progress}), we can choose $x$ s.t. $\phi(x) \rightarrow \ei$ for any $i \in [k]$.
Hence we can pick $x_1, x_3$ s.t.
\begin{equation}
\begin{split}
    &[\phi_{13}(x_1, x_3)]_i
    \rightarrow \frac{\mTrans_{ip} \mTrans_{qi}}{\sum_{j \in [k]} \mTrans_{jp} \mTrans_{qj}}, ~\forall p, q \in [k].
    % \propto P(x_1|h_2=i) P(x_3|h_2=i)
    % \\
    % \propto& \Big(\sum_{j} \mTrans_{ij} \exp\big(-\frac{\|x_1-\mu_j\|^2}{2} + c\big)\Big) \cdot \Big(\sum_{j} \mTrans_{ij} \exp\big(-\frac{\|x_3-\mu_j\|^2}{2} + c\big)\Big)
\end{split}
\end{equation}
\textcolor{gray}{(\textcolor{red}{this is wrong}, since $\phi(x) \rightarrow \ei$ does not mean $\phi_{13}$ has a term going to $\mTrans_{ip}$ due to normalization. e.g. if $\phi(x_1) \rightarrow e_1$, $\phi(x_3) \rightarrow e_2$, and $\mTrans = \mI$, then $\phi_{13}(x_1, x_3)$ can be anything.)}

Denote $x_c^{(i)}$ s.t. $\lim_{c\rightarrow \infty} \phi(x_c^{(i)})$.
Let $x_1 = x_\infty^{(i)}$, $x_3 = x_\infty^{(j)}$, then 
\begin{equation}
\begin{split}
    \E[x_2|x_1, x_3]
    = \mMeans\phi_{13}(x_\infty^{(i)}, x_\infty^{(i)})
    = \mMeans \frac{\mTrans^\top_i \odot \mTrans_j}{\|\mTrans^\top_i \odot \mTrans_j\|_1}
    = \tilde\mMeans \frac{\tilde\mTrans^\top_i \odot \tilde\mTrans_j}{\|\tilde\mTrans^\top_i \odot \tilde\mTrans_j\|_1}
\end{split}
\end{equation}
Define $\Phi := \Big[\phi_{13}(x_\infty^{(1)}, x_{\infty}^{(1)}), ..., \phi_{13}(x_\infty^{(k)}, x_{\infty}^{(k)})\Big]$ and similarly $\tilde\Phi$ as in the discrete case,
we can again get $\tilde\mTrans$ from $\tilde\Phi$, which is fully specified by $\mMeans, \mTrans$, and $\mR$.

\textcolor{gray}{\textcolor{Orange}{todo}: show that
1) considering these $k^2$ ``extreme points'' (i.e. columns of $\Phi$) is enough to cover arbitrary $\phi_{13}$ (may not be true due to scaling?);
2) find a counterexample that $\tilde\mMeans = \mR\mMeans$ for some special orthogonal $\mR$,
    and $\tilde\Phi = \tilde\mMeans^{-1}\mMeans \Phi$, from which we can recover a doubly stochastic $\tilde\mTrans$.
}

\textcolor{gray}{\textcolor{Orange}{note}: the above can only be used to find counterexamples but not as an identifiability proof, due to the error highlighted in red.}



==> COLT2022/proof_HMM/draft_2_13.tex <==
\section{[draft] $x_2 | (x_1 \otimes x_3)$}


The posterior function $\phi_{13}$ is
\begin{equation}
\begin{split}
    &\phi_{13}(x_1, x_3)
    = [P(h_2=i|x_1, x_3)]_{i \in [k]}
    \eqLabel{1}= \left[\frac{P(x_1|h_2=i) P(x_3|h_2=i)}{\sum_{j \in [k]} P(x_1|h_2=j) P(x_3|h_2=j)}\right]_{i \in [k]}
    \\
    =& \left[\frac{\langle \fll(x_1), \mTrans_i^\top\rangle \langle \fll(x_3), \mTrans_i\rangle}{\sum_{j\in[k]} \langle \fll(x_1), \mTrans_j^\top\rangle \langle \fll(x_3), \mTrans_j\rangle}\right]_{i \in [k]}
    = \left[\frac{\langle \phi(x_1), \mTrans_i^\top\rangle \langle \phi(x_3), \mTrans_i\rangle}{\sum_{j\in[k]} \langle \phi(x_1), \mTrans_j^\top\rangle \langle \phi(x_3), \mTrans_j\rangle}\right]_{i \in [k]}
    \\
    =& \frac{\mTrans^\top \fll(x_1) \odot \mTrans\fll(x_3)}{\|\mTrans^\top \fll(x_1) \odot \mTrans\fll(x_3)\|_1}
    = \frac{\mTrans^\top \phi(x_1) \odot \mTrans\phi(x_3)}{\|\mTrans^\top \phi(x_1) \odot \mTrans\phi(x_3)\|_1},
\end{split}
\end{equation}
where step $\rnum{1}$ uses Assumption \ref{assump:latent} that the latent distribution is uniform.



\subsection{Discrete case}

The optimal predictor is:
\begin{equation}
\begin{split}
    &\E[x_2|x_1=i, x_3=j]
    = \mEmiss \phi_{13}(i,j)
    = \mEmiss \frac{(\mTrans\mEmiss^\top)_i \odot (\mTrans^\top\mEmiss^\top)_j}{\|(\mTrans\mEmiss^\top)_i \odot (\mTrans^\top\mEmiss^\top)_j\|_1}
    \\
    =& \sum_{l \in [k]} \mEmiss_l \frac{\langle\mTrans_l, \phi(x_1)\rangle \langle \mTrans_{l:}, \phi(x_3)\rangle}{\|\langle\mTrans_l, \phi(x_1)\rangle \langle \mTrans_{l:}, \phi(x_3)\rangle\|_1}
    = \sum_{l \in [k]} \mEmiss_l \frac{\langle\mTrans_l, \mEmiss_{i:} \rangle \langle \mTrans_{l:}, \mEmiss_{j:}\rangle}{\|\langle\mTrans_l, \mEmiss_{i:}\rangle \langle \mTrans_{l:}, \mEmiss_{j:}\rangle\|_1}
    \\
    =& \sum_{l \in [k]} \mEmiss_l \left\langle\mTrans_l, \frac{\phi(x_1)}{\sqrt{\|\langle\mTrans_l, \mEmiss_{i:}\rangle \langle \mTrans_{l:}, \mEmiss_{j:}\rangle\|_1}} \right\rangle 
        \cdot \left\langle\mTrans_{l:}, \frac{\phi(x_3)}{\sqrt{\|\langle\mTrans_l, \mEmiss_{i:}\rangle \langle \mTrans_{l:}, \mEmiss_{j:}\rangle\|_1}} \right\rangle.
    \\
\end{split}
\end{equation}
\textcolor{gray}{(challenge: the input to the tensor $\sum_{l \in [k]} \mEmiss_l \otimes \mTrans_{l} \otimes \mTrans_{l:}$ depends on the parameters.)}


\textcolor{RoyalBlue}{What if we assume $\|\cdot\|_1$ is matched?}
If the normalization term is matched, then
\begin{equation}
\begin{split}
    &\mEmiss \cdot (\mTrans\mEmiss^\top)_{i} \odot (\mTrans^\top\mEmiss^\top)_j
    = \tilde\mEmiss \odot (\tilde\mTrans \tilde\mEmiss^\top)_{i} \cdot (\tilde\mTrans^\top \tilde\mEmiss^\top)_j,
    ~\forall i, j
    \\
    \Rightarrow&~ \mEmiss\cdot (\mTrans\mEmiss^\top)_i \odot \1
        = \mEmiss\cdot (\mTrans\mEmiss^\top)_i
        = \tilde\mEmiss\cdot (\tilde\mTrans\tilde\mEmiss^\top)_i,
    ~\forall i,j
    \\
    \Rightarrow&~ \mEmiss\mTrans\mEmiss^\top = \tilde\mEmiss\tilde\mTrans\tilde\mEmiss^\top.
\end{split}
\end{equation}
A necessary condition is to satisfy the last equality,
i.e. $\tilde\mEmiss = \mEmiss\mR$, $\tilde\mTrans = \mR^{-1}\mTrans\mR$ for some invertible $\mR$.
However, this choice would not be able to match $\|\cdot\|_1$.


\begin{equation}
\begin{split}
    &\mEmiss \cdot (\mTrans\mEmiss^\top)_{i} \odot (\mTrans^\top\mEmiss^\top)_j
    = \sum_{l \in [k]} \mEmiss_l \cdot \langle \mTrans_l, \mEmiss_{i:}\rangle \cdot \langle \mTrans_{l:}, \mEmiss_{j:}\rangle 
    \\
    % =& \sum_{l \in [k]} \mEmiss_l \cdot \langle (\mTrans\mEmiss^\top)_i, \ve_l \rangle \cdot \langle (\mTrans^\top\mEmiss^\top)_j, \ve_l \rangle 
\end{split}
\end{equation}

% \input{COLT2022/not_used/hmm_2_13_attempts}


\textcolor{RoyalBlue}{Matching $\phi_{13}$ doesn't give identifiability}: 
to construct a counterexample, it suffices to choose symmetric $\mTrans, \tilde\mTrans$, doubly stochastic (up to scaling $\frac{k}{d}$) $\mEmiss,\tilde\mEmiss$, and $\mEmiss\mTrans = \tilde\mEmiss\tilde\mTrans$.
Then
\begin{equation}
\begin{split}
    \phi_{13}(x_1=i, x_3=j)
    = \frac{(\mEmiss\mTrans^\top)_{i:} \odot (\mEmiss\mTrans)_{j:}}{\|(\mEmiss\mTrans^\top)_{i:} \odot (\mEmiss\mTrans)_{j:}\|_1}
    = \frac{(\tilde\mEmiss\tilde\mTrans^\top)_{i:} \odot (\tilde\mEmiss\tilde\mTrans)_{j:}}{\|(\tilde\mEmiss\tilde\mTrans^\top)_{i:} \odot (\tilde\mEmiss\tilde\mTrans)_{j:}\|_1}
    = \tilde\phi_{13}(x_1=i, x_3=j).
\end{split}
\end{equation}
The following is a concrete counterexample: consider $d = k = 3$, and let $a = 0.8$,
\begin{equation}
\begin{split}
    &\mTrans = \begin{bmatrix}
        a & 1-a & 0 \\ 1-a & 0 & a \\ 0 & a & 1-a \\
    \end{bmatrix},
    ~\tilde\mTrans = \begin{bmatrix}
        a & 0 & 1-a \\ 0 & 1-a & a \\ 1-a & a & 0 \\
    \end{bmatrix},
    \mR = \tilde\mTrans \mTrans^{-1},
    \\
    &\mEmiss = \begin{bmatrix}
       0.4695323  & 0.40420827 & 0.12625944 \\
       0.27370492 & 0.40545776 & 0.32083732 \\
       0.25676278 & 0.19033397 & 0.55290324 \\
    \end{bmatrix},
    \\
    &\tilde\mEmiss = \mEmiss\mR^{-1}
        = \begin{bmatrix}
       0.52864941 & 0.30361077 & 0.16773982 \\
       0.30336755 & 0.4098252  & 0.28680725 \\
       0.16798304 & 0.28656402 & 0.54545293 \\
        \end{bmatrix}.
\end{split}
\end{equation}
We can also have $d = 4 > k=3$: let $\mTrans, \tilde\mTrans, \mR$ be the same as above, and let $\mEmiss, \tilde\mEmiss$ be:
{\small
\begin{equation*}
\begin{split}
    \mEmiss = \begin{bmatrix}
       0.36290765 & 0.33875795 & 0.0483344  \\
       0.27741051 & 0.27428275 & 0.19830674 \\
       0.13599324 & 0.23416529 & 0.37984147 \\
       0.22368861 & 0.152794   & 0.37351739 \\
    \end{bmatrix},
    \tilde\mEmiss = \begin{bmatrix}
       0.4280708  & 0.24382385 & 0.07810535 \\
       0.29470284 & 0.25018373 & 0.20511344 \\
       0.10992735 & 0.30164382 & 0.33842882 \\
       0.16729901 & 0.2043486  & 0.37835239 \\
    \end{bmatrix}.
\end{split}
\end{equation*}
}

\textcolor{RoyalBlue}{(Attempt; not yet successful) $\tilde\mEmiss = \mEmiss\mR^{-1}$, $\tilde\Phi_{13} = \mR\Phi_{13}$ for some $\mR$.}
Let's assume $\mTrans$ is symmetric so that we have 
\begin{equation}
\begin{split}
    \E[x_2|x_1=i, x_3=j] 
    = \sum_{h \in [k]} \mEmiss_h \cdot \underbrace{\frac{(\mEmiss\mTrans)_{i,h} (\mEmiss\mTrans)_{j,h}}{\sum_{\bar{h}}(\mEmiss\mTrans)_{i,\bar{h}} (\mEmiss\mTrans)_{j,\bar{h}}}}_{:= \phi_{13}(i,j)}
\end{split}
\end{equation}
One idea is to find some $\mR$ (invertible but not necessarily orthogonal) s.t. $\tilde\mEmiss = \mEmiss\mR^{-1}$.
Let $\Phi_{13} := [\phi_{13}(1,1), ..., \phi_{13}(d,d)] \in \R^{k \times d}$, and define $\tilde\Phi_{13}$ similarly.
Matching the optimal predictor means $\tilde\Phi_{13} = \mR\Phi_{13}$.

Denote $\mA := \tilde\mEmiss \tilde\mTrans$, then
\begin{equation}
\begin{split}
    \phi_{13}(i,i) = \frac{\mA_{i,:} \odot \mA_{i,:}}{\|\mA_{i,:} \odot \mA_{i,:}\|_1}
    \eqLabel{1}\Rightarrow \mA_{i,:} \propto \sqrt{\phi_{13}(i,i)}
    \Rightarrow \tilde\mTrans = \tilde\mEmiss^{-1}\mA.
\end{split}
\end{equation}
where step $\rnum{1}$ chooses the scaling of $\mA$ such that the columns sum up to 1.
We will have a counterexample if we can find $\mEmiss, \mTrans, \mR$ s.t. $\tilde\mTrans$ is symmetric (which implies doubly stochastic).
\textcolor{gray}{\textcolor{Orange}{todo}: find such a counterexample.}

\textcolor{gray}{what properties does $\Phi_{13}$ have for a doubly stochastic $\mTrans$?}


\textcolor{RoyalBlue}{Can we take a dummy $\hat{p}(x_1,x_3)$?}
Suppose we have a dummy distribution where $\hat{p}(x_1, x_3)$ is independent of a specific choice of parameters.
We would like to apply Kruskal on the following tensor:
\begin{equation}
\begin{split}
    \Tensor
    :=& \sum_{x_1,x_3} \hat{p}(x_1,x_3) x_1 \otimes x_3 \otimes \E[x_2|x_1,x_3]
    \\
    =& \sum_{h_2} \Big(\sum_{x_1,x_3} \underbrace{\hat{p}(x_1, x_3) p(h_2|x_1,x_3)}_{:= \hat{p}(x_1,x_3,h_2)} x_1 \otimes x_3 \Big) \otimes \E[x_2|h_2]
    \\
    =& \sum_{h_2} \hat{p}(h_1) \hat\E[x_1|h_2] \otimes \hat\E[x_3|h_2] \otimes \E[x_2|h_2].
\end{split}
\end{equation}
$\Tensor$ will have a unique decomposition if
1) we can find $\hat\mEmiss, \hat\mTrans$ that produce $\hat{p}(x_1, x_3, h_2)$,
and that
2) $\{\hat\E[x_1|h_2=i]: i\in[k]\}$ is of rank-$k$.

Let's first try $\hat{p}(x_1, x_3) = \frac{1}{d^2}$.
Then 
\begin{equation}
\begin{split}
    &\hat{p}(x_1=i, x_3=j, h_2=l)
    \\
    =&~ p(h_2=l|x_1=i,x_3=j) \cdot \hat{p}(x_1,x_3)
    = \frac{(\mEmiss\mTrans^\top)_{il} (\mEmiss\mTrans)_{jl}}{\sum_{l'} (\mEmiss\mTrans^\top)_{il'} (\mEmiss\mTrans)_{jl'}} \cdot \frac{1}{d^2}
    \\
    =&~ \hat{p}(x_1=i|h_2=l) \hat{p}(x_3=j|h_2=l) \hat{p}(h_2)
    = (\hat\mEmiss \hat\mTrans^\top)_{il} \cdot (\hat\mEmiss \hat\mTrans)_{jl} \cdot \hat{p}(h_2)
    \\
    \Rightarrow~& \sum_{l\in[k]} \hat{p}(x_1=i, x_3=j, h_2=l)
        = \frac{1}{d^2} 
        = \hat{p}(h_2) \langle (\hat{\mEmiss}\hat{\mTrans}^\top)_{i:}, (\hat{\mEmiss}\hat{\mTrans})_{j:} \rangle
    \\
    \Rightarrow~& \langle (\hat{\mEmiss}\hat{\mTrans}^\top)_{i:}, (\hat{\mEmiss}\hat{\mTrans})_{j:} \rangle = \frac{\hat{p}(h_2)}{d^2}
\end{split}
\end{equation}
If $\hat{\mTrans}$ is symmetric and $\hat{p}(h_2)$, then $\langle (\hat{\mEmiss}\hat{\mTrans})_{i:}, (\hat{\mEmiss}\hat{\mTrans})_{i:} \rangle = \|\hat\mEmiss \hat\mTrans\|_2 = \frac{1}{\sqrt{d}}$ while $\|\hat\mEmiss \hat\mTrans\|_1 = 1$,
hence $\hat\mEmiss \hat\mTrans = \frac{1}{d}\1$, and $\hat\mEmiss \hat\mTrans$ is of rank-1.
\textcolor{gray}{In fact $\mEmiss\mTrans$ has to be rank-1 just by the choice of $p(x_1,x_3)$:
\begin{equation}
\begin{split}
    &p(x_1=i, x_3=j)
    = \frac{1}{k}\sum_{l\in[k]} p(x_1=i|h_2=l) p(x_3=j|h_2=l)
    = \frac{\langle (\mEmiss\mTrans^\top)_{i:}, (\mEmiss\mTrans)_{j:} \rangle}{k}
    = \frac{1}{d^2}
    \\
    &\Rightarrow (\mEmiss\mTrans^\top)_{i:} = (\mEmiss\mTrans)_{j:}, ~\forall i, j \in [d].
\end{split}
\end{equation}
}

\textcolor{gray}{other choices of $\hat{p}(x_1,x_3), \hat{p}(h_2)$ and non-symmetric $\mTrans$?
May not help: we should keep $\hat{p}(h_2)$ uniform (\textcolor{Orange}{should we?}).
Then to match $p(x_1,x_3)$, $p(h_2|x_1,x_3)$, $p(h_2, x_1, x_3)$, it suffices to match $\mEmiss\mTrans$ and $\mEmiss\mTrans^\top$.}



\subsection{Gaussian case}

\textcolor{RoyalBlue}{Can we show that matching the predictor implies matching the posterior?}

If $f^{2|1,3}(x_1, x_3) = \tilde{f}^{2|1,3}(x_1, x_3)$,
then $\forall x_1, x_3 \in \R^d$,
\begin{equation}
\begin{split}
    \mMeans\phi_{13}(x_1, x_3) = \tilde\mMeans \tilde\phi_{13}(x_1, x_3)
    \Rightarrow \tilde\phi_{13}(x_1, x_3) = \underbrace{(\tilde\mMeans^\dagger \mMeans)}_{:= \mR} \phi_{13}(x_1,x_3).
\end{split}
\end{equation}
% 
We would like to match the Jacobian on both sides, i.e.
\begin{equation}
\begin{split}
    &\partial_{x_1} \tilde\phi_{13}(x_1, x_3)
    = \partial_{\tilde\phi(x_1)} \tilde\phi_{13}(x_1, x_3) \cdot \nabla_{x_1} \tilde\phi(x_1)
    \\
    =&~ \partial_{x_1} \mR\phi_{13}(x_1, x_3)
    = \mR \partial_{\phi(x_1)} \phi_{13}(x_1, x_3) \cdot \nabla_{x_1} \phi(x_1).
\end{split}
\end{equation}
% 
Denote $v := \phi(x_1)$, $u := \phi(x_3)$,
and denote $N := \sum_{j \in [k]} \langle \mTrans_j, u\rangle \langle \mTrans_j^\top, v\rangle$,
then for $l \in [k]$,
\begin{equation}
\begin{split}
    \partial_{v_l}[\phi_{13}(x_1, x_3)]_i
    =& \partial_{v_l} \left[\frac{\langle \mTrans_i, u\rangle \langle \mTrans_i^\top, v\rangle}
        {\sum_{j \in [k]} \langle \mTrans_j, u\rangle \langle \mTrans_j^\top, v\rangle}\right]
    = \partial_{v_l} \left[\frac{\langle \mTrans_i, u\rangle \sum_{l' \in [k]} \mTrans_{il'} v_{l'}}
        {\sum_{j\in[k]}\langle \mTrans_j, u\rangle \sum_{l' \in [k]} \mTrans_{jl'} v_{l'}}\right]
    \\
    =&~ \frac{\langle \mTrans_i, u\rangle \mTrans_{il} \cdot N
        - \big(\langle \mTrans_i, u\rangle \sum_{l'\in[k]} \mTrans_{il'} v_{l'}\big) \cdot \big(\sum_{j\in[k]} \mTrans_{jl} \langle \mTrans_j, u\rangle\big)}
        {N^2}
    \\
    =&~ \frac{\langle \mTrans_i, u\rangle}{N} \mTrans_{il} - [\phi_{13}(x_1, x_3)]_i \cdot \frac{\sum_{j\in[k]} \mTrans_{jl} \langle \mTrans_j, u\rangle}{N}
    \\
    =& \frac{\langle \mTrans_i, u\rangle}{N} \mTrans_{il} - [\phi_{13}(x_1, x_3)]_i \cdot \frac{\langle \mTrans^\top u, \mTrans_{l}\rangle}{N}
        \in \R
    \\
    \partial_{v_l} \phi_{13}(x_1, x_3)
        =&~ \diag\left(\frac{\mTrans^\top u}{N}\right) \mTrans_{l}
            - \frac{\langle \mTrans^\top u, \mTrans_{l}\rangle}{N} \cdot \phi_{13}(x_1, x_3)
        \in \R^k
    \\
    \partial_v \phi_{13}(x_1, x_3)
        =&~ \diag\left(\frac{\mTrans^\top u}{N}\right) \mTrans
        - \phi_{13}(x_1, x_3) \frac{u ^\top \mTrans \mTrans}{N}
\end{split}
\end{equation}
Hence we are matching 
\begin{equation}
\begin{split}
    &\mR\frac{\left[\diag\left(\mTrans^\top \phi(x_3)\right) - \phi_{13}(x_1, x_3)(\mTrans^\top \phi(x_3))^\top\right]}{\|\mTrans \phi(x_1) \odot \mTrans^\top\phi(x_3)\|_1}\mTrans
    \cdot \left[\diag(\phi(x_1)) - \phi(x_1)\phi(x_1)^\top\right] \Delta^\top
    \\
    =& \frac{\left[\diag\left(\tilde\mTrans^\top \tilde\phi(x_3)\right) - \mR \phi_{13}(x_1, x_3) \tilde\phi(x_3) \tilde\mTrans \right]}{\|\tilde\mTrans \tilde\phi(x_1) \odot \tilde\mTrans^\top \tilde\phi(x_3)\|_1}\tilde\mTrans 
    \cdot \left[\diag(\tilde\phi(x_1)) - \tilde\phi(x_1)\tilde\phi(x_1)^\top\right] \tilde\Delta^\top
\end{split}
\end{equation}
The $\left[\diag(\tilde\phi(x_1)) - \tilde\phi(x_1)\tilde\phi(x_1)^\top\right]$ suggests that when $\phi(x) \rightarrow \ei$, we also have $\tilde\phi(x) \rightarrow \ei$.
Let $\phi(x_3) \rightarrow \ei$, then
\begin{equation}
\begin{split}
    &\mR \left[\diag\left(\frac{\mTrans_{i:}}{\|\mTrans \phi(x_1) \odot \mTrans_{i:}\|_1}\right) - \frac{\mTrans\phi(x_1) \odot \mTrans_{i:}}{\|\mTrans \phi(x_1) \odot \mTrans_{i:}\|_1} \mTrans_{i:}^\top \right]\mTrans
        \cdot \left[\diag(\phi(x_1)) - \phi(x_1)\phi(x_1)^\top\right] \Delta^\top
    \\
    =& \left[\diag\left(\frac{\tilde\mTrans_{i:}}{\|\tilde\mTrans \tilde\phi(x_1) \odot \tilde\mTrans_{i:}\|_1}\right) - \mR \frac{\tilde\mTrans\tilde\phi(x_1) \odot \tilde\mTrans_{i:}}{\|\tilde\mTrans \tilde\phi(x_1) \odot \tilde\mTrans_{i:}\|_1}\tilde\mTrans_{i:}^\top \right]\tilde\mTrans
        \cdot \left[\diag(\tilde\phi(x_1)) - \tilde\phi(x_1)\tilde\phi(x_1)^\top\right] \tilde\Delta^\top
\end{split}
\end{equation}
\textcolor{orange}{todo: finish this}

\textcolor{RoyalBlue}{Does matching the posterior mean matching the parameters?}


\begin{equation}
\begin{split}
    \phi_{13}(x_1,x_3) = \frac{\mTrans\phi(x_1) \odot \mTrans^\top\phi(x_3)}{\|\mTrans\phi(x_1) \odot \mTrans^\top\phi(x_3)\|_1}
    = \frac{\tilde\mTrans\tilde\phi(x_1) \odot \tilde\mTrans^\top\tilde\phi(x_3)}{\|\tilde\mTrans\tilde\phi(x_1) \odot \tilde\mTrans^\top \tilde\phi(x_3)\|_1}
    = \tilde\phi_{13}(x_1, x_3)
\end{split}
\end{equation}

\textcolor{RoyalBlue}{If $\phi_{13} = \tilde\phi_{13}$ and the normalization is matched, then $\phi = \tilde\phi$.}

\textcolor{orange}{todo: prove that the normalization is the same}

Assume we have $\mTrans\phi(x_1) \odot \mTrans^\top\phi(x_3) = \tilde\mTrans\tilde\phi(x_1) \odot \tilde\mTrans^\top\tilde\phi(x_3)$, $\forall x_1,x_3$.
For any fixed $x_3$,
denote $\mS := \diag\left(\left[\frac{\langle \mTrans_i, \phi(x_3)\rangle}{\langle\tilde\mTrans_i, \tilde\phi(x_3)\rangle}\right]\right)$,
then 
\begin{equation}
\begin{split}
    &\mS \Delta(x) \Big(\diag(\phi(x)) - \phi(x)\phi(x)^\top\Big) \mTrans^\top 
    = \tilde\Delta(x)\Big(\diag(\tilde\phi(x)) - \tilde\phi(x)\tilde\phi(x)^\top\Big) \tilde\mTrans^\top, ~\forall x \in \R^d.
    \\
\end{split}
\end{equation}
Choose $x$ s.t. $\phi(x) \rightarrow \ei$, then the left hand side goes to 0, and the right hand side also goes to 0, which means $\tilde\phi(x)\rightarrow \ej$ for some $j \in [k]$ since $\tilde\Delta(x), \tilde\mTrans$ are both of rank $k$.
Let $x_3$ be such $x$, then 
\begin{equation}
\begin{split}
    &\mTrans\phi(x_1) \odot \mTrans_{i:}
    = \tilde\mTrans\tilde\phi(x_1) \odot \tilde\mTrans_{i:}, ~\forall x_1
    \Rightarrow~ \mTrans\phi(x_1) = \tilde\mTrans \tilde\phi(x_1), ~\forall x_1
    \Rightarrow \phi(x_1) = \mP\tilde\phi(x_1), ~\forall x_1.
\end{split}
\end{equation}



==> COLT2022/proof_HMM/draft_noJoint.tex <==
\subsection{\textcolor{Orange}{[in progress]} Fix the proofs}


% \textbf{Problem of the existing proof}: having the optimal predictors only means the conditional expectations are matched, which may not be sufficient.
% Take $x_2 \otimes x_3|x_1$ as an example.
% Previously we used a scaling $\weight(x_1)$ and defined a 3-tensor:
% \begin{equation}
% \begin{split}
%     \Tensor_\weight
%     := \sum_{x_1} \weight(x_1) x_1 \otimes \E_{\mEmiss,\mTrans}[x_2 \otimes x_3|x_1]
% \end{split}
% \end{equation}
% Suppose $\tilde\mEmiss, \tilde\mTrans$ satisfy $\E_{\mEmiss,\mTrans}[x_2\otimes x_3|x_1] = \E_{\tilde\mEmiss,\tilde\mTrans}[x_2 \otimes x_3|x_1]$.
% Taking $\weight(x_1) = P_{\mEmiss,\mTrans}(x_1)$ gives a rank-1 decomposition of
% \begin{equation}
% \begin{split}
%     \Tensor = \sum_{h_2} P(h_2) \E_{\mEmiss,\mTrans}[x_1|h_2] \otimes \E_{\mEmiss,\mTrans}[x_2|h_2] \otimes \E_{\mEmiss,\mTrans}[x_3|h_2].
% \end{split}
% \end{equation}
% However, taking $\weight(x_1) = P_{\tilde\mEmiss, \tilde\mTrans}(x_1)$ gives a different decomposition:
% \begin{equation}
% \begin{split}
%     \tilde\Tensor = \sum_{h_2} P(h_2) \E_{\tilde\mEmiss,\tilde\mTrans}[x_1|h_2] \otimes \E_{\tilde\mEmiss, \tilde\mTrans}[x_2|h_2] \otimes \E_{\tilde\mEmiss, \tilde\mTrans}[x_3|h_2].
% \end{split}
% \end{equation}
% Both $\Tensor, \tilde\Tensor$ have a unique decomposition, however these two decompositions can be different.



\paragraph{\textcolor{sky}{Case 3, $\E[x_2|x_1\otimes x_3]$}} (\textcolor{peach}{identifiable})
Suppose $\tilde\mEmiss, \tilde\mTrans$ form an optimal predictor $\E[x_2|x_1,x_3]$, and let $\tilde p(x_1, x_3)$ be the marginal distribution on $(x_1, x_3)$ according to $\tilde\mEmiss, \tilde\mTrans$, and let $\tilde{p}(h_2|x_1,x_3)$ be the posterior according to $\tilde\mEmiss, \tilde\mTrans$.
Consider the following tensor:
\begin{equation}
\begin{split}
    &\Tensor
    := \sum_{x_1, x_3} \tilde p(x_1,x_3) x_1 \otimes x_3 \otimes \tilde\E[x_2|x_1,x_3]
    \\
    =& \sum_{x_1, x_3} \tilde p(x_1,x_3) x_1 \otimes x_3 \otimes \tilde\E_{h_2|x_1,x_3}[\tilde\E[x_2|x_1,x_3,h_2]]
    \\
    =& \sum_{x_1, x_3} \tilde p(x_1,x_3) x_1 \otimes x_3 \otimes \sum_{h_2} \tilde{p}(h_2|x_1,x_3)\tilde\E[x_2|x_1,x_3,h_2]
    \\
    =& \sum_{x_1, x_3} \sum_{h_2} \tilde p(x_1,x_3) \tilde p(h_2|x_1, x_3) x_1 \otimes x_3 \otimes \tilde\E[x_2|x_1,x_3, h_2]
    \\
    =& \sum_{h_2} (\sum_{x_1, x_3} \tilde p(x_1,x_3) \tilde p(h_2|x_1,x_3) x_1 \otimes x_3) \otimes \tilde\E[x_2|h_2]
    \\
    =& \sum_{h_2} \tilde{p}(h_2) \tilde\E[x_1|h_2] \otimes \tilde\E[x_3|h_2] \otimes \tilde\E[x_2|h_2]
    \\
    =& \sum_{i\in[k]} \tilde{p}(i) (\tilde\mEmiss\tilde\mTrans^\top)_i \otimes (\tilde\mEmiss\tilde\mTrans)_i \otimes \tilde\mEmiss_i
\end{split}
\end{equation}
Applying Kruskal's theorem on this tensors recovers $\mEmiss$ and $\mEmiss\mTrans$.

On the other hand, since $\tilde\E[x_2|x_1,x_3] = \E[x_2|x_1,x_3]$, the same tensor above can also be written as 
\begin{equation}
\begin{split}
    &\Tensor
    = \sum_{x_1, x_3} \tilde p(x_1,x_3) x_1 \otimes x_3 \otimes \tilde\E[x_2|x_1,x_3]
    \\
    =& \sum_{x_1, x_3} \tilde p(x_1,x_3) x_1 \otimes x_3 \otimes \E[x_2|x_1,x_3]
    \\
    =& \sum_{x_1,x_3} \tilde{p}(x_1,x_3) x_1 \otimes x_3 \otimes \textcolor{Orange}{\sum_{h_2} p(h_2|x_1,x_3) \E[x_2|h_2]}
    \\
    \textcolor{red}{=}& \sum_{h_2} \tilde{p}(h_2) \tilde\E[x_1|h_2] \otimes \tilde\E[x_3|h_2] \otimes \E[x_2|h_2]
    = \sum_{i\in[k]} \tilde{p}(i) (\tilde\mEmiss\tilde\mTrans^\top)_i \otimes (\tilde\mEmiss\tilde\mTrans)_i \otimes \mEmiss_i,
\end{split}
\end{equation}
which means $\tilde\mEmiss = \mEmiss$.
\textcolor{gray}{\textcolor{red}{this is wrong}: the equality in red is problematic since the expression in Orange is scaled with $p(h_2|x_1,x_3)$ rather than $\tilde{p}(h_2|x_1,x_3)$.}

It remains to determine $\mTrans$.
The optimal predictor takes the form $\E[x_2|x_1, x_3] 
= \mEmiss \phi_{13}(x_1, x_3)$, where $\phi_{13}(x_1, x_3) = [P(h_2=i|x_1,x_3)]_{i \in [k]} \in \R^k$.
Matching the predictor with $\tilde\mEmiss = \mEmiss$ implies $\phi_{13}(x_1, x_3) = \tilde\phi_{13}(x_1, x_3)$.
Moreover, the marginal distribution for $x_3$ is also matched for the ground truth and the learned parameters, since the stationary distribution for the latent is uniform by Assumption \ref{assump:latent};
hence $p(x_3) = \mEmiss \frac{1}{k}\1 = \tilde{p}(x_3)$.
Then the posterior vector of $h_2$ given $x_1$, denoted as $P(h_2|x_1) \in \R^k$, is also matched, since 
\begin{equation}
\begin{split}
    P(h_2|x_1)
    =& \sum_{i \in [d]} p(x_3=\ei) P(h_2|x_1, \ei)
    = \sum_{i \in [d]} p(x_3=\ei) \phi_{13}(x_1, \ei)
    \\
    =& \sum_{i\in[d]} \tilde{p}(x_3 = \ei) \tilde\phi_{13}(x_1, \ei)
    = \tilde{P}(h_2|x_1).
\end{split}
\end{equation}
\textcolor{gray}{Note: matching the marginals also implies matching the following quantities:
\begin{equation}
\begin{split}
    P(x_2=i) 
    =& \sum_{h_1} P(h_1) P(x_2|h_1) = \frac{1}{k} \|(\mEmiss\mTrans)_{i:}\|_1 = \frac{1}{k} \|(\tilde\mEmiss\tilde\mTrans)_{i:}\|_1
    \\
    =& \sum_{h_2} P(h_2) P(x_2|h_1) = \frac{1}{k}\|\mEmiss_{i:}\|_1 = \frac{1}{k}\|\tilde\mEmiss_{i:}\|_1
    \\
    =& \sum_{h_3} P(h_3) P(x_2|h_3) = \frac{1}{k} \|(\mEmiss\mTrans^\top)_{i:}\|_1 = \frac{1}{k} \|(\tilde\mEmiss\tilde\mTrans^\top)_{i:}\|_1
\end{split}
\end{equation}
where the subscript $_{i:}$ means the $i_{th}$ row.
}


On the other hand, $P(h_2|x_1) = \mTrans\phi(x_1)$.
Considering all $d$ choices of $x_1$ gives:
\begin{equation}
\begin{split}
    &[P(h_2|e_1), P(h_2|e_2), ..., P(h_2|e_d)] = [\tilde{P}(h_2|e_1), \tilde{P}(h_2|e_2), ..., \tilde{P}(h_2|e_d)]
    \\
    \Rightarrow&~ \mTrans[\phi(e_1), \phi(e_2), ..., \phi(e_d)] = \tilde\mTrans[\phi(e_1), \phi(e_2), ..., \phi(e_d)]
    \\
    \Rightarrow&~ \mTrans \cdot \mEmiss^\top\diag([1/\|\mEmiss_i^\top\|_{i \in [d]}]) = \tilde\mTrans \cdot \mEmiss^\top\diag([1/\|\mEmiss_i^\top\|_{i \in [d]}])
    \\
    \Rightarrow&~ \mTrans = \tilde\mTrans,
\end{split}
\end{equation}
where the last step is because $\mEmiss^\top\diag([1/\|\mEmiss_i^\top\|_{i \in [d]}])$ is of rank $k$ by Assumption \ref{assump:discrete_full_rank}.

%% Comment out previous attempts
\input{COLT2022/not_used/hmm_2_13_attempts}


% \RestyleAlgo{ruled}
% %% This is needed if you want to add comments in
% %% your algorithm with \Comment
% \SetKwComment{Comment}{/* }{ */}
% \begin{algorithm}[hbt!]
% \KwData{$n \geq 0$}
% \KwResult{$y = x^n$}
% $y \gets 1$\;
% $X \gets x$\;
% $N \gets n$\;
% \While{$N \neq 0$}{
%   \eIf{$N$ is even}{
%     $X \gets X \times X$\;
%     $N \gets \frac{N}{2} $ \Comment*[r]{This is a comment}
%   }{\If{$N$ is odd}{
%       $y \gets y \times X$\;
%       $N \gets N - 1$\;
%     }
%   }
% }
% \caption{An algorithm with caption}\label{alg:two}
% \end{algorithm}


\vspace{1em}

For the Gaussian case \textcolor{Orange}{(in progress)}

\textcolor{RoyalBlue}{Can we show that matching the predictor implies matching the posterior?}

If $f^{2|1,3}(x_1, x_3) = \tilde{f}^{2|1,3}(x_1, x_3)$,
then $\forall x_1, x_3 \in \R^d$,
\begin{equation}
\begin{split}
    \mMeans\phi_{13}(x_1, x_3) = \tilde\mMeans \tilde\phi_{13}(x_1, x_3)
    \Rightarrow \tilde\phi_{13}(x_1, x_3) = \underbrace{(\tilde\mMeans^\dagger \mMeans)}_{:= \mR} \phi_{13}(x_1,x_3).
\end{split}
\end{equation}
% 
We would like to match the Jacobian on both sides, i.e.
\begin{equation}
\begin{split}
    &\partial_{x_1} \tilde\phi_{13}(x_1, x_3)
    = \partial_{\tilde\phi(x_1)} \tilde\phi_{13}(x_1, x_3) \cdot \nabla_{x_1} \tilde\phi(x_1)
    \\
    =&~ \partial_{x_1} \mR\phi_{13}(x_1, x_3)
    = \mR \partial_{\phi(x_1)} \phi_{13}(x_1, x_3) \cdot \nabla_{x_1} \phi(x_1).
\end{split}
\end{equation}
% 
Denote $v := \phi(x_1)$, $u := \phi(x_3)$,
and denote $N := \sum_{j \in [k]} \langle \mTrans_j, u\rangle \langle \mTrans_j^\top, v\rangle$,
then for $l \in [k]$,
\begin{equation}
\begin{split}
    \partial_{v_l}[\phi_{13}(x_1, x_3)]_i
    =& \partial_{v_l} \left[\frac{\langle \mTrans_i, u\rangle \langle \mTrans_i^\top, v\rangle}
        {\sum_{j \in [k]} \langle \mTrans_j, u\rangle \langle \mTrans_j^\top, v\rangle}\right]
    = \partial_{v_l} \left[\frac{\langle \mTrans_i, u\rangle \sum_{l' \in [k]} \mTrans_{il'} v_{l'}}
        {\sum_{j\in[k]}\langle \mTrans_j, u\rangle \sum_{l' \in [k]} \mTrans_{jl'} v_{l'}}\right]
    \\
    =&~ \frac{\langle \mTrans_i, u\rangle \mTrans_{il} \cdot N
        - \big(\langle \mTrans_i, u\rangle \sum_{l'\in[k]} \mTrans_{il'} v_{l'}\big) \cdot \big(\sum_{j\in[k]} \mTrans_{jl} \langle \mTrans_j, u\rangle\big)}
        {N^2}
    \\
    =&~ \frac{\langle \mTrans_i, u\rangle}{N} \mTrans_{il} - [\phi_{13}(x_1, x_3)]_i \cdot \frac{\sum_{j\in[k]} \mTrans_{jl} \langle \mTrans_j, u\rangle}{N}
    \\
    =& \frac{\langle \mTrans_i, u\rangle}{N} \mTrans_{il} - [\phi_{13}(x_1, x_3)]_i \cdot \frac{\langle \mTrans^\top u, \mTrans_{l}\rangle}{N}
        \in \R
    \\
    \partial_{v_l} \phi_{13}(x_1, x_3)
        =&~ \diag\left(\frac{\mTrans^\top u}{N}\right) \mTrans_{l}
            - \frac{\langle \mTrans^\top u, \mTrans_{l}\rangle}{N} \cdot \phi_{13}(x_1, x_3)
        \in \R^k
    \\
    \partial_v \phi_{13}(x_1, x_3)
        =&~ \diag\left(\frac{\mTrans^\top u}{N}\right) \mTrans
        - \phi_{13}(x_1, x_3) \frac{u ^\top \mTrans \mTrans}{N}
\end{split}
\end{equation}
Hence we are matching 
\begin{equation}
\begin{split}
    &\mR\frac{\left[\diag\left(\mTrans^\top \phi(x_3)\right) - \phi_{13}(x_1, x_3)(\mTrans^\top \phi(x_3))^\top\right]}{\|\mTrans \phi(x_1) \odot \mTrans^\top\phi(x_3)\|_1}\mTrans
    \cdot \left[\diag(\phi(x_1)) - \phi(x_1)\phi(x_1)^\top\right] \Delta^\top
    \\
    =& \frac{\left[\diag\left(\tilde\mTrans^\top \tilde\phi(x_3)\right) - \mR \phi_{13}(x_1, x_3) \tilde\phi(x_3) \tilde\mTrans \right]}{\|\tilde\mTrans \tilde\phi(x_1) \odot \tilde\mTrans^\top \tilde\phi(x_3)\|_1}\tilde\mTrans 
    \cdot \left[\diag(\tilde\phi(x_1)) - \tilde\phi(x_1)\tilde\phi(x_1)^\top\right] \tilde\Delta^\top
\end{split}
\end{equation}
The $\left[\diag(\tilde\phi(x_1)) - \tilde\phi(x_1)\tilde\phi(x_1)^\top\right]$ suggests that when $\phi(x) \rightarrow \ei$, we also have $\tilde\phi(x) \rightarrow \ei$.
Let $\phi(x_3) \rightarrow \ei$, then
\begin{equation}
\begin{split}
    &\mR \left[\diag\left(\frac{\mTrans_{i:}}{\|\mTrans \phi(x_1) \odot \mTrans_{i:}\|_1}\right) - \frac{\mTrans\phi(x_1) \odot \mTrans_{i:}}{\|\mTrans \phi(x_1) \odot \mTrans_{i:}\|_1} \mTrans_{i:}^\top \right]\mTrans
        \cdot \left[\diag(\phi(x_1)) - \phi(x_1)\phi(x_1)^\top\right] \Delta^\top
    \\
    =& \left[\diag\left(\frac{\tilde\mTrans_{i:}}{\|\tilde\mTrans \tilde\phi(x_1) \odot \tilde\mTrans_{i:}\|_1}\right) - \mR \frac{\tilde\mTrans\tilde\phi(x_1) \odot \tilde\mTrans_{i:}}{\|\tilde\mTrans \tilde\phi(x_1) \odot \tilde\mTrans_{i:}\|_1}\tilde\mTrans_{i:}^\top \right]\tilde\mTrans
        \cdot \left[\diag(\tilde\phi(x_1)) - \tilde\phi(x_1)\tilde\phi(x_1)^\top\right] \tilde\Delta^\top
\end{split}
\end{equation}


%% Comment out wrong proof (the 3-tensor was parameter-dependent)
% \input{COLT2022/not_used/gmm_2_13_wrong}

%% Comment out attempts with matching 
% \input{COLT2022/not_used/gmm_2_13_attempts_matchM}

%% Comment out attempt to find a counterexample
% \input{COLT2022/proof_HMM/attempt_case3_2_13}


\paragraph{\textcolor{sky}{Case 4, $\E[x_3|x_1\otimes x_2]$}} (\textcolor{Orange}{in progress})

The optimal predictor takes the form $\E[x_3|x_1,x_2] = \mEmiss\mTrans\phi_{12}(x_1,x_2)$, where $\phi_{12}(x_1,x_2)$ computes the posterior vectors of $h_2$:
\begin{equation}
\begin{split}
    &\phi_{12}(x_1, x_2)
    = [P(h_2=i|x_1, x_2)]_{i \in [k]}
    = \left[\frac{P(x_1|h_2=i) P(x_2|h_2=i)}{\sum_{j \in [k]} P(x_1|h_2=j) P(x_2|h_2=j)}\right]_{i \in [k]}
    \\
    =&~ \left[\frac{\langle \fll(x_1), \mTrans_i^\top\rangle \langle \fll(x_2), \ei\rangle}{\sum_{j\in[k]} \langle \fll(x_1), \mTrans_j^\top\rangle \langle \fll(x_2), \ej\rangle}\right]_{i \in [k]}
    = \left[\frac{\langle \phi(x_1), \mTrans_i^\top\rangle \langle \phi(x_2), \ei\rangle}{\sum_{j\in[k]} \langle \phi(x_1), \mTrans_j^\top\rangle \langle \phi(x_2), \ej\rangle}\right]_{i \in [k]}
    \\
    =&~ \frac{\mTrans^\top \fll(x_1) \odot \fll(x_2)}{\|\mTrans^\top \fll(x_1) \odot \fll(x_2)\|_1}
    = \frac{\mTrans^\top \phi(x_1) \odot \phi(x_2)}{\|\mTrans^\top \phi(x_1) \odot \phi(x_2)\|_1}.
\end{split}
\end{equation}
% 

%% Comment out: wrongly applied Kruskal: the constructed tensors are different.
% \input{COLT2022/not_used/hmm_3_12_wrong_Kruskal.tex}

\textcolor{RoyalBlue}{Can we have different singleton marginals, but the same conditional?}

For the discrete case, the probability vector $p(x_3|x_1=i,x_2=j) = \E[x_3|x_1=i, x_2=j] \in \R^{d}$.
Hence matching the predictors means:
\begin{equation}
\begin{split}
    &\E[x_3|x_1=i, x_2=j] = \tilde\E[x_3|x_1=i, x_2=j]
    \\
    \Rightarrow& p(x_3|x_1=i, x_2=j) = \tilde{p}(x_3|x_1=i, x_2=j)
    \\
    \Rightarrow& \underbrace{\frac{p(x_1=i, x_2=j|x_3=l)}{\sum_{l'\in[d]} p(x_1=i,x_2=j|x_3=l')}}_{:= V[i,j]}
        = \underbrace{\frac{\tilde{p}(x_1=i, x_2=j|x_3=l)}{\sum_{l'\in[d]} \tilde{p}(x_1=i, x_2=j|x_3=l')}}_{:= \tilde{V}[i,j]} \cdot \underbrace{\frac{\tilde{p}(x_3=l)}{p(x_3=l)}}_{:= r_l}
    \\
    \Rightarrow& \langle V[i,j], \1 \rangle = \langle \tilde{V}[i,j], r\rangle = 1, ~\forall i,j \in [d].
\end{split}
\end{equation}
We know that $r = \1$ is a valid solution,
and would like to show that $r = \1$ is the \textit{only} solution.
To do this, we would like to show that the set $\{\E[x_1=i, x_2=j|x_3] \in \R^d: i, j\in[d]\}$ spans a $(d-1)$-dimensional space.
Note that this is only possible for $d=k$, since the dimension of $\E[x_1=i,x_2=j|x_3]$ is limited by the latent dimension $k$:
\begin{equation}
\begin{split}
    &[\E[x_1=i,x_2=j|x_3]]_l
    = p(x_1=i, x_2=j|x_3=l)
    \\
    =& \sum_{m \in [k]} p(x_1=i|h_2=m) p(x_2=i|h_2=m) [\mTrans^\top \phi(x_3=l)]_m
    \\
    \propto&~ (\mEmiss_{i:})^\top \mTrans^\top \diag(\mTrans^\top \mEmiss_{l:}) \mEmiss_{j:}
    = \langle \mTrans^\top \mEmiss_{l:}, p(x_1=i, x_2=j|h_2= \cdot) \rangle
    \\
    \eqLabel{1}=&~ \Big\langle \mTrans^\top \mEmiss_{l:}, \frac{\phi_{12}(x_1=i, x_2=j) p(x_1=i, x_2=j)}{p(h_2)} \Big\rangle
    \\
    \propto&~ \langle \mTrans^\top\mEmiss_{l:}, \phi_{12}(x_1=i, x_2=j) \rangle 
    \propto \langle \mTrans^\top\mEmiss_{l:}, \mTrans\mEmiss_{i:} \odot \mEmiss_{j:} \rangle 
    \\
    \Rightarrow&~ \E[x_1=i,x_2=j|x_3] \propto \mEmiss\mTrans (\mTrans\mEmiss_{i:} \odot \mEmiss_{j:})
\end{split}
\end{equation}

\vspace{20em}

where step $\rnum{1}$ holds because $p(h_2)=\frac{1}{k}$ (otherwise the second expression would involve a diagonal scaling matrix.)

When $d=k$, we would like to see if the set $\{\mTrans\mEmiss_{i:} \odot \mEmiss_{j:}: i,j \in [d]\}$ is of dim $(d-1)$.
\textcolor{Orange}{(todo)}

Suppose this is true, then we have $r = \1$, and $p(x_3) = \tilde{p}(x_3)$.
Then
\begin{equation}
\begin{split}
    &p(x_3|x_1,x_2) = \frac{p(x_1,x_2|x_3) p(x_3)}{p(x_1,x_2)}
    = \frac{\tilde{p}(x_1,x_2|x_3) \tilde{p}(x_3)}{\tilde{p}(x_1,x_2)}
    = \tilde{p}(x_3|x_1,x_2)
    \\
    \Rightarrow& \frac{p(x_1,x_2|x_3)}{p(x_1,x_2)}
    = \frac{\tilde{p}(x_1,x_2|x_3)}{\tilde{p}(x_1,x_2)}
\end{split}
\end{equation}
\textcolor{gray}{If we can show that $p(x_1,x_2)$, $\tilde{p}(x_1,x_2)$ have to match, then $p(x_1,x_2|x_3) = \tilde{p}(x_1,x_2|x_3)$, i.e. back to Case 1 which is identifiable.}

\textcolor{RoyalBlue}{What does $p(x_1,x_2) = \tilde{p}(x_1,x_2)$ require / imply?}
\begin{equation}
\begin{split}
    &p(x_1=i,x_2=j)
    = \sum_{l\in[k]} p(x_1=i|h_1=l) p(x_2=j|h_1=l) p(h_1=l)
    \\
    =& \frac{1}{k}\sum_l p(x_1=i|h_1=l) p(x_2=j|h_1=l)
    = \frac{1}{k}\langle \mEmiss_{i:}, \mTrans^\top \mEmiss_{j:}\rangle
    = \frac{1}{k}\langle \tilde\mEmiss_{i:}, \tilde\mTrans^\top \tilde\mEmiss_{j:}\rangle
    \\
    \Rightarrow&~ \mEmiss\mTrans^\top \mEmiss^\top = \tilde\mEmiss \tilde\mTrans^\top \tilde\mEmiss^\top
\end{split}
\end{equation}

\textcolor{gray}{// can we get this from matching $p(x_3|x_1,x_2)$ and $p(x_3)$?}

If $\|\mTrans\mEmiss_{i:} \odot \mEmiss_{j:}\|_1 = \|\|\tilde\mTrans\tilde\mEmiss_{i:} \odot \tilde\mEmiss_{j:}\|_1$
\begin{equation}
\begin{split}
    p(x_3|x_1,x_2) = \mEmiss\mTrans \cdot \frac{\mTrans\mEmiss_{i:} \odot \mEmiss_{j:}}{\|\mTrans\mEmiss_{i:} \odot \mEmiss_{j:}\|}
    = \tilde\mEmiss \tilde\mTrans \cdot \frac{\tilde\mTrans\tilde\mEmiss_{i:} \odot \tilde\mEmiss_{j:}}{\|\tilde\mTrans\tilde\mEmiss_{i:} \odot \tilde\mEmiss_{j:}\|}
    = \tilde{p}(x_3 | x_1,x_2)
\end{split}
\end{equation}



\vspace{1em}
For \GHMM (\textcolor{Orange}{in progress}), the predictor is 
\begin{equation}
\begin{split}
    \E[x_3|x_1, x_2]
    = \mMeans\mTrans \phi_{12}(x_1,x_2)
    = \mMeans\mTrans \frac{\mTrans^\top \phi(x_1) \odot \phi(x_2)}{\|\mTrans^\top \phi(x_1) \odot \phi(x_2)\|_1}.
\end{split}
\end{equation}

Matching the predictors means $\tilde\phi_{12}(x_1,x_2) = \mR\phi_{12}(x_1,x_2)$ for $\mR := (\tilde\mMeans\tilde\mTrans)^\dagger \mMeans\mTrans$.
Equating the gradients on both sides gives:
\begin{equation}
\begin{split}
    &\mR \left[\diag\left(\frac{\phi(x_2)}{\|\mTrans \phi(x_1) \odot \phi(x_2)\|_1}\right) - \phi_{12}(x_1, x_2) \phi(x_2)^\top \right] \mTrans 
    \cdot \left[\diag(\phi(x_1)) - \phi(x_1)\phi(x_1)^\top\right] \Delta^\top
    \\
    =& \left[\diag\left(\frac{\tilde\phi(x_2)}{\|\tilde\mTrans \tilde\phi(x_1) \odot \tilde\phi(x_2)\|_1}\right) - \mR\phi_{12}(x_1, x_2) \tilde\phi(x_2)^\top \right] \tilde\mTrans
    \cdot \left[\diag(\tilde\phi(x_1)) - \tilde\phi(x_1)\tilde\phi(x_1)^\top\right] \tilde\Delta^\top
\end{split}
\end{equation}
The $\left[\diag(\tilde\phi(x_1)) - \tilde\phi(x_1)\tilde\phi(x_1)^\top\right]$ suggests that when $\phi(x) \rightarrow \ei$, we also have $\tilde\phi(x) \rightarrow \ei$.
Let $\phi(x_2) \rightarrow \ei$, then
\begin{equation}
\begin{split}
    &\mR \left[\diag\left(\ei\right) - \ei\ei^\top\right]\mTrans
        \cdot \left[\diag(\phi(x_1)) - \phi(x_1)\phi(x_1)^\top\right] \Delta^\top
        = 0
    \\
    &= \left[\diag\left(\ei\right) - \ei \ei^\top\mR^\top\right]\tilde\mTrans
        \cdot \left[\diag(\tilde\phi(x_1)) - \tilde\phi(x_1)\tilde\phi(x_1)^\top\right] \Delta^\top, ~\forall x_1
    \\
    \eqLabel{1}{\Rightarrow}&~ \diag\left(\ei\right) - \ei \ei^\top\mR^\top
        = \diag(\ei) - \ei \mR_i^\top 
        = 0
    \\
    \Rightarrow& \mR_i = \ei.
\end{split}
\end{equation}
\textcolor{Orange}{todo: double check step $\rnum{1}$.}

(Assuming the above is correct) Then $\mMeans\mTrans = \tilde\mMeans \tilde\mTrans$.
\textcolor{gray}{\textcolor{Orange}{todo}: what next? What does matching $\phi_{13}$ give us?}

% Let $x_c^{(i)}$ denote a vector s.t. $\lim_{c \rightarrow \infty} \tilde{\phi}(x_c^{(i)}) = \ei$.
% If we take $x_2 = x_\infty^{(i)}$, then 
% \begin{equation}
% \begin{split}
%     &\E[x_3|x_1, x_2]
%     = \mMeans\mTrans \frac{\mTrans^\top\phi(x_1) \odot \ei}{\|\mTrans^\top\phi(x_1) \odot \ei\|_1}
%     = \mMeans\mTrans \ei
%     = \tilde\mMeans \tilde\mTrans \frac{\tilde\mTrans^\top \tilde\phi(x_1) \odot \tilde\phi(x_\infty^{(i)})}{\|\tilde\mTrans^\top \tilde\phi(x_1) \odot \phi(x_\infty^{(i)})\|_1}
%     \\
%     % \Rightarrow \mMeans\mTrans = \tilde\mMeans \tilde\mTrans.
% \end{split}
% \end{equation}
% This means all vectors in the set $\{\tilde\mTrans^\top \tilde\phi(x_1) \odot \tilde\phi(x_\infty^{(i)}): x_1 \in \R^d\}$ are colinear.
% Since $\{\tilde\mTrans^\top \tilde\phi(x_1): x_1 \in \R^d\}$ can span $\R^k$ \textcolor{Orange}{(todo: show this)},
% it must be that $\tilde\phi(x_\infty^{(i)}) = \ej$ for some $j \in [k]$,
% hence $\mMeans\mTrans = \tilde\mMeans \tilde\mTrans$, and 
% \begin{equation}
% \begin{split}
%     \phi_{12}(x_1, x_2) = \tilde\phi_{12}(x_1, x_2)
% \end{split}
% \end{equation}
% \textcolor{gray}{could it be that this is identifiable?}

==> COLT2022/proof_HMM/jennrich_23_1.tex <==
We can use Jennrich's algorithm, provided that there exist $x_1,x_1'$ s.t. the element-wise division of $\mTrans\phi(x_1) / \mTrans\phi(x_1')$ has \textcolor{peach}{distinct entries}, as stated in the following assumption:
% (i.e. Assumption \ref{assump:discrete_distinct_diag}).
\vspace{-1em}
\begin{assumption}\label{assump:discrete_distinct_diag}
  Let $\mTrans$ denote the transition matrix, then there exist $x_1, x_1' \in \gX$ such that the diagonal matrix $\diag(\mTrans \phi(x_1)) \diag(\mTrans\phi(x_1'))^{-1}$ has distinct diagonal entries.
\end{assumption}
\vspace{-0.8em}
\textit{Remark}: For HMM, Assumption \ref{assump:discrete_distinct_diag} means there exist $i, j \in [k]$ such that $\frac{(\mTrans\mEmiss^\top)_i}{(\mTrans\mEmiss^\top)_j}$ has distinct entries, that is, $\frac{\langle \mTrans_h^\top, \mEmiss_i^\top \rangle}{\langle \mTrans_h^\top, \mEmiss_j^\top \rangle}$ is different for each $h \in [k]$.
% 
For \GHMM, this means there exist $x,x'$ s.t. $\frac{\mTrans\fll(x)}{\mTrans\fll(x')}$ has distinct entries.

Denote matrices $\mW_1 := \E[x_2 \otimes x_3 | x_1]$ and $\mW_2 := \E[x_2 \otimes x_3 | x_1']$, we have:
\begin{equation}
\begin{split}
  \mW_1 \mW_2^{-1}
  =& \mEmiss\mTrans \diag(\mTrans\phi(x_1)) \mEmiss^\top \mEmiss^{-\top} \diag(\mTrans\phi(x_1'))^{-1} (\mEmiss\mTrans)^{-1} 
  \\
  =& \mEmiss\mTrans \cdot \underbrace{\diag(\mTrans\phi(x_1))\diag(\mTrans\phi(x_1'))^{-1}}_{:= \mD_1} \cdot (\mEmiss\mTrans)^{-1}
  \\
  \mW_1^{-1} \mW_2
  =& \mEmiss^{-\top} \diag(\mTrans\phi(x_1))^{-1} (\mEmiss\mTrans)^{-1} \mEmiss\mTrans \diag(\mTrans\phi(x_1')) \mEmiss^\top
  \\
  =& \mEmiss^{-\top} \cdot \underbrace{\diag(\mTrans\phi(x_1))^{-1}\diag(\mTrans\phi(x_1'))}_{:= \mD_2} \cdot \mEmiss^\top
\end{split}
\end{equation}
Performing eigendecomposition on $\mW_\tOne \mW_\tTwo^{-1}$ and $\mW_{1}^{-1}\mW_2$ recovers the columns of $\mEmiss$ and $\mEmiss\mTrans$ up to column-wise permutation and scaling.
\textcolor{gray}{(note: if we use Assumption \ref{assump:discrete_distinct_diag}, then we do not need to reason about the form of $\phi$.)}

==> COLT2022/proof_HMM/proof_with_kruskal.tex <==
\subsubsection{Proof for identifiability from $x_{\tTwo} \otimes x_\tThr | x_{\tOne}$}

By the symmetry from the Markov property, the 6 permutations of $\{\tOne, \tTwo, \tThr\}$ can be summarized into two configurations: one is $\tOne < \tTwo < \tThr$, and the other is $\tOne < \tThr < \tTwo$.

\paragraph{Case I, $\tOne < \tTwo < \tThr$} 
The optimal predictor $f^{\tTwo,\tThr|\tOne}$ calculates $\E[x_{\tTwo} \otimes x_{\tThr} | x_{\tOne}]$, which takes the parametric form:
\begin{equation}
\begin{split}
&f^{\tTwo,\tThr|\tOne}(x_{\tOne})
  = \sum_{i, j\in[k]} P(h_{\tTwo}=i, h_{\tThr} = j| x_{\tOne}) \cdot \E[x_{\tTwo} \otimes x_{\tThr} | h_{\tTwo}, h_{\tThr}]
  \\
  =& \sum_{i} P(h_{\tTwo}=i| x_{\tOne}) \cdot \E[x_{\tTwo} | h_{\tTwo}] \otimes \big(\sum_{j} P(h_{\tThr} = j|h_{\tTwo}=i) \cdot \E[x_{\tThr} |h_{\tThr}]\big)
  \\
  =& \mEmiss\mTrans^{\tThr-\tTwo} \diag(\mTrans^{\tTwo-\tOne}\phi(x_{\tOne})) \mEmiss^\top
\end{split}
\end{equation}
When the learned predictor also has the above parametric form, identifying the parameters can be related to the uniqueness of tensor decomposition, by constructing a proper 3-tensor and applying Kruskal's theorem.
Let $\weight(x_\tOne)$ denote a weighting for $x_\tOne$, such as a distribution over $x_\tOne$,
and consider the following 3-tensor:
\begin{equation}
\begin{split}
  &\Tensor_\weight
  := \sum_{x_\tOne} \weight(x_\tOne) x_\tOne \otimes f^{\tTwo,\tThr|\tOne}(x_\tOne)
  \\
  =& \sum_{x_\tOne} \weight(x_\tOne) x_\tOne \otimes \sum_{i\in [k]} P(h_{\tTwo}=i|x_\tOne) \E[x_\tTwo|h_\tTwo=i] \otimes \E[x_\tThr|h_\tTwo=i]
  \\
  =& \sum_{i \in [k]} \sum_{x_\tOne} P(h_{\tTwo}=i|x_\tOne) \weight(x_\tOne) x_\tOne \otimes \E[x_\tTwo|h_\tTwo=i] \otimes \E[x_\tThr|h_\tTwo=i]
\end{split}
\end{equation}
Take $\weight(x_\tOne) = P(x_\tOne)$, then the first component involving $x_\tOne$ is 
\begin{equation}
\begin{split}
  &\sum_{x_\tOne} P(h_{\tTwo}=i|x_\tOne) P(x_\tOne) x_\tOne
  = P(h_\tTwo=i) \sum_{x_\tOne} P(x_\tOne|h_\tTwo=i) x_\tOne
  = \Pstat{\tTwo}{i} \E[x_\tOne|h_\tTwo=i].
\end{split}
\end{equation}
For $\E[x_\tOne|h_\tTwo]$, note that the transition matrix for the backward chain is $\mTrans^\top$, since  
\begin{equation*}
\begin{split}
  P(h_{t-1}=i|h_t=j) = \frac{P(h_t=j|h_{t-1}=i) \pi_{t-1}(i)}{\sum_{l \in [k]} P(h_{t}=j|h_{t-1}=l)\pi_{t-1}(l)}
  = \frac{\mTrans_{ji}}{\sum_{l\in[k]} \mTrans_{jl}}
  = \mTrans_{ji},
\end{split}
\end{equation*}
where the second equality uses $\pi_{t-1}$ is uniform, and the third equality uses the fact of $\mTrans$ is doubly stochastic, both by Assumption \ref{assump:latent}.
Hence 
\begin{equation}
\begin{split}
  &\Tensor_\weight 
  = \sum_{i \in [k]} \Pstat{\tTwo}{i} \E[x_{\tOne}|h_\tTwo=i] \otimes \E[x_{\tTwo}|h_\tTwo=i] \otimes \E[x_{\tThr}|h_\tTwo=i]
  \\
  =& \sum_{i \in [k]} \Pstat{\tTwo}{i} \big(\mEmiss(\mTrans^{\tTwo-\tOne})^\top\big)_i \otimes \mEmiss_i \otimes (\mEmiss\mTrans^{\tThr-\tTwo})_i.
\end{split}
\end{equation}
Each component in the above low-rank decomposition is of Kruskal rank $k$ by Assumption \ref{assump:discrete_full_rank}, hence columns of $\mEmiss, \mEmiss\mTrans^{\tThr-\tTwo}$ can be recovered up to a shared permutation and scaling.
Noting that columns of $\mEmiss$ need to sum up to 1, we can further remove the indeterminacy in scaling.
Therefore $\mEmiss, \textcolor{red}{\mTrans}$ are recovered up to a shared permutation.

\paragraph{Case II, $\tTwo < \tOne < \tThr$}
The optimal predictor $f^{\tTwo,\tThr|\tOne}$ has the parametric form
\begin{equation}
\begin{split}
  &f^{\tTwo,\tThr|\tOne}(x_{\tOne}) 
  = \E[x_\tTwo \otimes x_\tThr | x_\tOne]
  = \sum_{i \in [k]} P(h_{\tOne}=\ei|x_\tOne) \E[x_\tTwo|h_{\tOne}=\ei] \otimes \E[x_\tThr|h_\tOne=\ei] 
  \\
  =& \sum_{i \in [k]} [\phi(x_{\tOne})]_i \big(\mEmiss(\mTrans^{\tOne-\tTwo})^\top\big)_i \otimes (\mEmiss\mTrans^{\tThr-\tOne})_i
  = \mEmiss(\mTrans^{\tOne-\tTwo})^\top \diag(\phi(x_\tOne)) (\mTrans^{\tThr-\tOne})^\top \mEmiss^\top
\end{split}
\end{equation}
% 
Similar to Case I, we will construct a 3-tensor using outputs of the optimal predictor $f^{\tTwo,\tThr|\tOne}$, and apply Kruskal's theorem for identifiability.
Let $\weight(x_\tOne)$ be an arbitrary scaling for $x_\tOne$,
and consider the following 3-tensor defined with $\weight(x_{\tOne})$:
\begin{equation}
\begin{split}
  \Tensor_\weight
  := &\sum_{x_\tOne} \weight(x_{\tOne}) \E[x_{\tTwo} \otimes x_\tThr | x_\tOne] \otimes x_\tOne
  \\
  =& \sum_{x_\tOne} \weight(x_\tOne) \Big(\sum_{j\in[k]} \E[x_\tTwo \otimes x_\tThr | h_\tTwo] P(h_\tTwo|x_\tOne)\Big) \otimes x_\tOne
  \\
  =& \sum_{x_\tOne} \sum_{j\in[k]} \weight(x_\tOne)P(h_\tOne=j|x_\tOne) \E[x_\tTwo|h_\tOne=j] \otimes \E[x_\tThr | h_\tOne=j] \otimes x_\tOne
  \\
  =& \sum_{j\in[k]} \E[x_\tTwo|h_\tOne=j] \otimes \E[x_\tThr | h_\tOne=j] \otimes \sum_{x_\tOne} \weight(x_\tOne)P(h_\tOne|x_\tOne) x_\tOne
  \\
  =& \sum_{j\in[k]} (\mEmiss(\mTrans^\top)^{\tOne - \tTwo})_j \otimes (\mEmiss\mTrans^{\tThr-\tOne})_j \otimes \sum_{x_\tOne} \weight(x_\tOne)P(h_\tOne|x_\tOne) x_\tOne
\end{split}
\end{equation}
Take $\weight(x_\tOne) = P(x_\tOne)$, then the third component becomes
\begin{equation*}
\begin{split}
  &\sum_{i\in[d]} \weight(x_\tOne)P(h_\tOne=j|x_\tOne) x_\tOne
  = \sum_{i\in[d]} P(x_\tOne)P(h_\tOne=j|x_\tOne) x_\tOne
  \\
  =& P(h_\tOne=j) \sum_{i\in[d]} P(x_\tOne|h_\tOne=j) x_\tOne
  = P(h_\tOne=j) \E[x_\tOne|h_\tOne=j]
  = \Pstat{\tOne}{j} \mEmiss_j.
\end{split}
\end{equation*}
Hence $\Tensor_\weight = \sum_{j \in [k]} P(h_\tOne=j) (\mEmiss(\mTrans^\top)^{\tOne - \tTwo})_j \otimes (\mEmiss\mTrans^{\tThr-\tOne})_j \otimes \mEmiss_j$,
where all three components are of rank $k$ by Assumption \ref{assump:discrete_full_rank}.
% we have $\psi(h_\tTwo) = \sum_{i\in[d]} P(h_\tTwo, x_\tTwo) x_\tTwo = \pi(h_\tTwo) \E[x_\tTwo|h_\tTwo]$, which guarantees no pair of $j, j'$ makes $\psi(j), \psi(j')$ a scaling of each other.
Therefore Kruskal's theorem applies, and we can recover columns of $\mEmiss$ and $\mTrans^{\tThr-\tOne}$ up to a shared permutation, \textcolor{red}{hence also columns of $\mTrans$}.


\paragraph{An alternative proof for Case I}
\textcolor{Orange}{(a very minor remark)}
For Case I where the conditioned token is the first (or last) of the three tokens, we can use an alternative proof that does not require using all possible values of $x_\tOne$.
First, we make \textcolor{peach}{the following assumption}:
\vspace{-1em}
\begin{assumption}\label{assump:discrete_distinct_diag}
  Let $\mTrans$ denote the transition matrix, then there exist $x_1, x_1' \in \gX$ such that the diagonal matrix $\diag(\mTrans^t \phi(x_1)) \diag(\mTrans^t\phi(x_1'))^{-1}$ has distinct diagonal entries, for any power $t \in \N^+$.
\end{assumption}
% 
As before, the learned predictor is taken to have the correct parametric form.
Identifying the parameters boils down to the identifiability from the decomposition
\begin{equation}
\begin{split}
  \sum_{i} [\mTrans^{\tTwo-\tOne} \phi(x_{\tOne})]_i \cdot \mEmiss_i \otimes [\mEmiss\mTrans^{\tThr-\tTwo}]_i.
\end{split}
\end{equation}
% 
Note that this form is analogous to that of an eigendecomposition.
By \textcolor{peach}{Assumption \ref{assump:discrete_distinct_diag}},
 there exist $x_1, x_1'$ such that $\{[\mTrans^{\tThr-\tTwo} \phi(x_1)]_i /[\mTrans^{\tThr-\tTwo}\phi(x_1')]_i\}_{i \in [k]}$ has distinct values.
Define matrices $\mW_1 := \E[x_2 \otimes x_3 | x_1]$ and $\mW_2 := \E[x_2 \otimes x_3 | x_1']$, which are available from the optimal $f^{\tTwo,\tThr|\tOne}$, then:
\begin{equation}
\begin{split}
  \mW_1 \mW_2^{-1}
  =& \mEmiss\mTrans^{\tThr-\tTwo} \diag(\mTrans^{\tTwo-\tOne}\phi(x_1)) \mEmiss^\top \mEmiss^{-\top} \diag(\mTrans^{\tTwo-\tOne}\phi(x_1'))^{-1} (\mEmiss\mTrans^{\tThr-\tTwo})^{-1} 
  \\
  =& \mEmiss\mTrans^{\tThr-\tTwo} \cdot \underbrace{\diag(\mTrans^{\tTwo-\tOne}\phi(x_1))\diag(\mTrans^{\tTwo-\tOne}\phi(x_1'))^{-1}}_{:= \mD_1} \cdot (\mEmiss\mTrans^{\tThr-\tTwo})^{-1}
  \\
  \mW_1^{-1} \mW_2
  =& \mEmiss^{-\top} \diag(\mTrans^{\tTwo-\tOne}\phi(x_1))^{-1} (\mEmiss\mTrans^{\tThr-\tTwo})^{-1} \mEmiss\mTrans^{\tThr-\tTwo} \diag(\mTrans^{\tTwo-\tOne}\phi(x_1')) \mEmiss^\top
  \\
  =& \mEmiss^{-\top} \cdot \underbrace{\diag(\mTrans^{\tTwo-\tOne}\phi(x_1))^{-1}\diag(\mTrans^{\tTwo-\tOne}\phi(x_1'))}_{:= \mD_2} \cdot \mEmiss^\top
\end{split}
\end{equation}
Performing eigendecomposition on $\mW_\tOne \mW_\tTwo^{-1}$ and $\mW_{1}^{-1}\mW_2$ recovers the columns of $\mEmiss$ and $\mEmiss\mTrans^{\tTwo-\tOne}$ up to column-wise permutation and scaling. This permutation is shared, since the columns can be aligned noting that their corresponding eigenvalues are reciprocals of each other, given $\mD_1 \mD_2 = \mI$.
We can then recover $\mTrans^{\tTwo-\tOne}$, which removes the indeterminacy in scaling since the columns of \textcolor{red}{$\mTrans^{\tTwo -\tOne}$} need to sum up to 1.
Hence $\mEmiss, \mTrans$ can be recovered up to a shared permutation.

\subsubsection{Proof for identifiability from $x_{\tThr} | x_{\tOne} \otimes x_{\tTwo}$}

Similar to the previous task, using the Markov property and by symmetry, we only need to consider two configurations out of the six possible orderings of $\tOne, \tTwo, \tThr$: one is $\tOne < \tTwo < \tThr$, and the other is $\tOne < \tThr < \tTwo$.
The idea is to construct a proper 3-tensor for each case, on which we can apply Kruskal's theorem for identifiability.

\paragraph{Case I, $\tOne < \tTwo < \tThr$}:
The optimal predictor has the parametric form 
\begin{equation}
\begin{split}
  &f^{\tThr|\tOne,\tTwo}(x_\tOne, x_\tTwo)
  = \E[x_\tThr|x_\tOne, x_\tTwo]
  = \sum_{i\in[k]} \E[x_{\tThr}|h_\tTwo=i] P(h_\tTwo=i|x_\tOne, x_\tTwo)
  \\
  \eqLabel{1}=& \sum_{i \in [k]} (\mEmiss\mTrans^{\tThr-\tTwo})_i \cdot \frac{P(x_{\tOne}|h_{\tTwo}=i) P(x_{\tTwo}|h_{\tTwo}=i)}{\sum_{j \in [k]}P(x_{\tOne}|h_{\tTwo}=j) P(x_{\tTwo}|h_{\tTwo}=j)}
  \\
  =& \sum_{i \in [k]} (\mEmiss\mTrans^{\tThr-\tTwo})_i \cdot \frac{\big(\mEmiss(\mTrans^{\tTwo-\tOne})^\top\big)_{x_{\tOne},i} \mEmiss_{x_\tTwo, i}}{\sum_{j \in [k]} \big(\mEmiss(\mTrans^{\tTwo-\tOne})^\top\big)_{x_{\tOne},j} \mEmiss_{x_\tTwo, j}}
\end{split}
\end{equation}
where step $\rnum{1}$ uses Assumption \ref{assump:latent} that the latent distribution is stationary and uniform.

We now construct a 3-tensor using the optimal predictor.
Let $\eta(x_{\tOne}, x_{\tTwo})$ be some weighting on $(x_\tOne, x_\tTwo)$, and consider the following 3-tensor:
\begin{equation}
\begin{split}
  % &\E_\eta[x_{\tOne} \otimes x_{\tTwo} \otimes x_{\tThr}]
  &\Tensor_{\weight}
  = \sum_{x_{\tOne}, x_{\tTwo}} \weight(x_\tOne, x_\tTwo) x_\tOne \otimes x_\tTwo \otimes \E[x_\tThr | x_{\tOne}, x_{\tTwo}]
  \\
  =& \sum_{x_{\tOne}, x_{\tTwo}} \weight(x_{\tOne}, x_{\tTwo}) x_{\tOne} \otimes x_{\tTwo} \otimes \Big(\sum_{i\in[k]} P(h_{\tTwo}=\ei|x_{\tTwo}, x_{\tTwo}) \E[x_\tThr|h_{\tTwo}=\ei]\Big)
  \\
  =& \sum_{i \in [k]} \Big(\sum_{x_{\tOne}, x_{\tTwo}} P(h_{\tTwo}=\ei|x_{\tOne}, x_{\tTwo}) \weight(x_{\tOne}, x_{\tTwo}) x_{\tOne} \otimes x_{\tTwo}\Big) \otimes \E[x_\tThr|h_{\tTwo}=\ei].
  \\
\end{split}
\end{equation}
% 
Choose $\weight(x_{\tOne}, x_{\tTwo}) = P(x_{\tOne}, x_{\tTwo})$, then the 2-tensor defined with $x_\tOne, x_\tTwo$ is
\begin{equation}
\begin{split}
  &\sum_{x_{\tOne}, x_{\tTwo}} P(h_{\tTwo}=\ei|x_{\tOne}, x_{\tTwo}) P(x_{\tOne}, x_{\tTwo}) x_{\tOne} \otimes x_{\tTwo}
  \\
  =& P(h_{\tTwo}=\ei) \sum_{x_{\tOne}, x_{\tTwo}} P(x_{\tOne}|h_\tTwo=\ei) P(x_{\tTwo}|h_\tTwo=\ei) x_{\tOne} \otimes x_{\tTwo}
  \\
  =& P(h_{\tTwo}=\ei) \E[x_\tTwo|h_\tTwo=\ei] \otimes \E[x_\tOne|h_\tTwo=\ei]
  = \Pstat{\tTwo}{i} \cdot \big(\mEmiss(\mTrans^{\tTwo-\tOne})^\top\big)_i \otimes \mEmiss_i.
\end{split}
\end{equation}
Hence $\Tensor_\weight = \sum_{i\in[k]} \Pstat{\tTwo}{i} \big(\mEmiss(\mTrans^{\tTwo-\tOne})^\top\big)_i \otimes \mEmiss_i \otimes (\mEmiss\mTrans^{\tThr-\tTwo})_i$.
Each component has Kruskal rank $k$ by Assumption \ref{assump:discrete_full_rank}, therefore we can recover columns of $\mEmiss$, $\mEmiss\mTrans^{\tau_2}$, and \textcolor{red}{hence also $\mTrans$}.


\paragraph{Case II, $\tOne < \tThr < \tTwo$}:
% we can write $\tOne, \tTwo, \tThr$ as $t - \tau_1, \tTwo, t$ instead, for $t = \tThr$, and $\tau_1, \tau_2 > 0$, $\tau_1 < t$.
The optimal predictor is 
\begin{equation}
\begin{split}
  &f^{\tThr|\tOne,\tTwo}(x_\tOne, x_\tTwo)
  = \sum_{i \in [k]} \E[x_\tThr|h_{\tThr}=i] P(h_{\tThr}=i|x_\tOne, x_\tTwo)
  \\
  \eqLabel{1}=& \sum_{i \in [k]} \mEmiss_i \cdot \frac{P(x_{\tOne}|h_{\tThr}=i) P(x_{\tTwo}|h_{\tThr}=i)}{\sum_{j \in [k]}P(x_{\tOne}|h_{\tThr}=j) P(x_{\tTwo}|h_{\tThr}=j)}
  \\
  =& \sum_{i \in [k]} \mEmiss_i \cdot \frac{\big(\mEmiss(\mTrans^{\tThr-\tOne})^\top\big)_{x_{\tOne},i} (\mEmiss \mTrans^{\tTwo-\tThr})_{x_\tTwo, i}}{\sum_{j \in [k]} \big(\mEmiss(\mTrans^{\tThr-\tOne})^\top\big)_{x_{\tOne},j} (\mEmiss \mTrans^{\tTwo-\tThr})_{x_\tTwo, j}}
\end{split}
\end{equation}
where step $\rnum{1}$ uses Assumption \ref{assump:latent} that the latent distribution is stationary and uniform.

We construct a 3-tensor for applying the Kruskal's theorem. 
Let $\weight(x_{\tOne}, x_{\tTwo})$ denote an arbitrary distribution on $(x_{\tOne}, x_{\tTwo})$, and consider the following 3-tensor:
\begin{equation}
\begin{split}
  &\Tensor_\weight
  = \sum_{x_{\tOne}, x_{\tTwo}} \weight(x_{\tOne}, x_{\tTwo}) \E[x_\tThr | x_{\tOne} \otimes x_{\tTwo}] \otimes x_{\tOne} \otimes x_{\tTwo}
  \\
  =& \sum_{x_{\tOne}, x_{\tTwo}} \sum_{i\in[k]} \E[x_\tThr|h_\tThr=i] \otimes \big(P(h_\tThr=i | x_{\tOne}, x_{\tTwo}) \weight(x_{\tOne}, x_{\tTwo}) x_{\tOne} \otimes x_{\tTwo} \big)
  \\
  =& \sum_{i \in [k]} \E[x_\tThr|h_\tThr=i] \otimes \Big( \sum_{x_{\tOne}, x_{\tTwo}} P(h_\tThr=i | x_{\tOne}, x_{\tTwo}) \weight(x_{\tOne}, x_{\tTwo}) x_{\tOne} \otimes x_{\tTwo} \Big)
\end{split}
\end{equation}
Choose $\weight(x_{\tOne}, x_{\tTwo}) = P(x_{\tOne}, x_{\tTwo})$, then the 2-tensor involving $x_\tOne, x_\tTwo$ is
\begin{equation}
\begin{split}
    &\sum_{x_{\tOne}, x_{\tTwo}} P(h_\tThr=i | x_{\tOne}, x_{\tTwo}) P(x_{\tOne}, x_{\tTwo}) x_{\tOne} \otimes x_{\tTwo}
  = \sum_{x_{\tOne}, x_{\tTwo}} P(h_{\tThr}=i, x_{\tOne}, x_{\tTwo}) \otimes x_{\tOne} \otimes x_{\tTwo}
  \\
  =& P(h_\tThr=i) \E[x_{\tOne}|h_\tThr=i] \otimes \E[x_{\tTwo}|h_\tThr=i] 
  = \Pstat{\tThr}{i} \big(\mEmiss(\mTrans^{\tThr-\tOne})^\top\big)_{i} \otimes \big(\mEmiss\mTrans^{\tTwo-\tThr}\big)_{i}
\end{split}
\end{equation}
Hence $\Tensor_\weight = \sum_{i \in [k]} \Pstat{\tThr}{i} \mEmiss_i \otimes \big(\mEmiss(\mTrans^{\tThr-\tOne})^\top\big)_{i} \otimes \big(\mEmiss\mTrans^{\tTwo-\tThr}\big)_{i}$, where each component is of Kruskal rank $k$ by Assumption \ref{assump:discrete_full_rank}.
Therefore the columns of $\mEmiss,\mTrans^{\tTwo-\tThr}$ are recovered, and \textcolor{red}{hence also $\mTrans$}.


==> imports/author_notes.tex <==
\include{defs}
\def\shownotes{1}  %set 1 to show author notes
\ifnum\shownotes=1
\newcommand{\authnote}[2]{{$\ll$\textsf{\footnotesize #1 notes: #2}$\gg$}}
\else
\newcommand{\authnote}[2]{}
\fi
\newcommand{\Anote}[1]{{\color{Rouge}\authnote{Andrej}{{#1}}}}
\newcommand{\Bnote}[1]{{\color{Orange}\authnote{Bingbin}{{#1}}}}
\newcommand{\dhcomment}[1]{{\color{Emerald}\authnote{Daniel}{{#1}}}}
\newcommand{\Dnote}[1]{{\color{Emerald}\authnote{Daniel}{{#1}}}}
\newcommand{\Pnote}[1]{{\color{Cerulean}\authnote{Pradeep}{{#1}}}}
\newcommand{\Q}[1]{{\color{red}{Q: }{{#1}}}}
\newcommand{\TODO}[1]{{\color{red}{TODO: }{{#1}}}}

==> imports/colors.tex <==
%% NOTE: remove these color definitions before submitting
%% to make sure all comments are addressed.

\definecolor{RoyalBlue}{RGB}{0,100,170}
\definecolor{OliveGreen}{RGB}{30,140,30}
\definecolor{peach}{rgb}{1, 0.56, 0.56}
\definecolor{midgray}{RGB}{150,150,150}
\definecolor{grass}{RGB}{120, 190, 50}
\definecolor{sky}{RGB}{50,150,250}
\definecolor{Orange}{RGB}{250,150,50}
\definecolor{Cerulean}{RGB}{80,150,220}
\definecolor{Rouge}{RGB}{250,95,95}


\definecolor{ColorDef}{RGB}{80, 180, 150}

%% The following colors are defined for draft only;
%% Remove these definitions before submitting the final draft.
\definecolor{draftGray}{RGB}{150,150,150}


==> imports/packages_colt.tex <==
\usepackage{amsmath}
\usepackage{amssymb}
% \usepackage{amsthm}
\usepackage{bm}
\usepackage[ruled]{algorithm2e}
% \usepackage{mathtools}
\usepackage{graphicx}
% \usepackage{bm,bbm}

% \usepackage{listings}
% \usepackage[dvipsnames]{xcolor}
% \usepackage{xcolor}
% \usepackage[colorlinks = true,
%             linkcolor = blue,
%             urlcolor  = blue,
%             citecolor = blue,
%             anchorcolor = blue]{hyperref}
% \usepackage{geometry}
\usepackage{enumitem}
\usepackage{url}
% \usepackage{algorithmic}
% \usepackage{fullpage}
% \usepackage{geometry}
% \geometry{
% %  total={170mm,257mm},
% left=20mm,
% top=20mm,
% bottom=20mm,
% }
% 
\usepackage{caption}
% \usepackage{subcaption}

% \usepackage[hang,flushmargin]{footmisc}
\usepackage[bottom]{footmisc}
\usepackage{natbib}
\usepackage{romannum}
\def \rnum#1{(\romannum{#1})}
\def \eqLabel#1{\overset{(\romannum{#1})}}

\usepackage{xspace}

% for breaking long citations into new lines
\usepackage{breakcites}
\usepackage{breakurl}




==> math/commands_colt.tex <==
\renewcommand{\Pr}{\mathop{\bf Pr\/}}               
% \newcommand{\E}{\mathop{\bf E\/}}
\newcommand{\Ex}{\mathop{\bf E\/}}
\newcommand{\Es}[1]{\mathop{\bf E\/}_{{\substack{\#1}}}}            
% \newcommand{\Var}{\mathop{\bf Var\/}}
% \newcommand{\Cov}{\mathop{\bf Cov\/}}
\newcommand{\stddev}{\mathop{\bf stddev\/}}
\newcommand{\littlesum}{\mathop{{\textstyle \sum}}}
% \newcommand{\R}{\mathbb R}
\newcommand{\C}{\mathbb C}
\newcommand{\N}{\mathbb N}
\newcommand{\Z}{\mathbb Z}
\newcommand{\F}{\mathbb F}
\newcommand{\W}{\mathbb W}
\newcommand{\I}{\mathbbm{1}}


% \newtheorem{theorem}{Theorem}
\newtheorem*{namedtheorem}{\theoremname}
\newcommand{\theoremname}{testing}
\newenvironment{named}[1]{ \renewcommand{\theoremname}{\#1} \begin{namedtheorem}} {\end{namedtheorem}}
\newtheorem{thm}[theorem]{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem*{lemma*}{Lemma}
\newtheorem{lem}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{clm}[theorem]{Claim}
\newtheorem*{claim*}{Claim}
% \newtheorem{proposition}[theorem]{Proposition}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{res}{Restriction}
\newtheorem{observation}{Observation}
% \newtheorem{corollary}[theorem]{Corollary}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{question}[theorem]{Question}
\newtheorem{cons}{Constraints}
% \newtheorem{conjecture}{Conjecture}
\newtheorem*{question*}{Question}
\newtheorem{vars}{Variables}
\newtheorem{conds}{Condition}
% \theoremstyle{definition}
% \newtheorem{definition}{Definition}
\newtheorem{definition*}{Definition}
\newtheorem{defn}[theorem]{Definition}
% \newtheorem{remark}[theorem]{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem{rem}[theorem]{Remark}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{notn}[theorem]{Notation}
% \theoremstyle{plain}
\newtheorem{Alg}{Algorithm}
\newtheorem{assumption}{Assumption}


\newcommand{\defeq}{\stackrel{\small \mathrm{def}}{=}}



==> math/format.tex <==
%% Note: need \usepackage{bm}

%%%%% NEW MATH DEFINITIONS %%%%%

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\def \P {\mathbb{P}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.


% mathrm terms
% \newcommand{\poly}{\mathrm{poly}}
% \newcommand{\polylog}{\mathrm{polylog}}
% \newcommand{\size}{\mathrm{size}}

